An approach to Physics Based Single Photon Vision System Design

The design of the camera and optical measurement is a crucial part of optimizing machine vision systems. However, camera designs are usually optimized to produce human-interpretable images. Moreover, camera optimization typically makes the assumption of additive noise, while modern optical imaging systems are mainly affected by photon noise which is not additive. Previous studies have highlighted the fundamental effect of the noise model on the outcome of the design process in the context of coded single-pixel and compressed sensing cameras. In addition to the exact noise model, the nature of the data encountered and the vision task fundamentally affect the optimal hardware design. This means that a camera or compressed sensing code that is optimal for capturing images is almost certainly not optimal for any downstream vision task. In this work, we used a simple end-to-end model on a single-pixel camera to study the effects of the noise model for different vision tasks. We demonstrate the importance of incorporating non-linear noise features in optimizing even the simplest vision systems.

==> hardware_pca_onn/Main/authorship.tex <==
\makeatletter
\newcommand{\linebreakand}{%
  \end{@IEEEauthorhalign}
  \hfill\mbox{}\par
  \mbox{}\hfill\begin{@IEEEauthorhalign}
}
\makeatother

\IEEEoverridecommandlockouts

\author{
\IEEEauthorblockN{Yizhou Lu}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: ylu289@wisc.edu}
\and
\IEEEauthorblockN{Trevor Seets}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: seets@wisc.edu}
\and
\IEEEauthorblockN{Ehsan Ahmadi}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: eahmadi2@wisc.edu}

% \and
\linebreakand 
\IEEEauthorblockN{Felipe Gutierrez-Barragan}
\IEEEauthorblockA{Department of Computer Sciences\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: fgutierrez3@wisc.edu}
\and
\IEEEauthorblockN{Andreas Velten \thanks{\IEEEauthorrefmark{4} Andreas Velten is corresponding author.}}
\IEEEauthorblockA{Department of Biostatistics and Medical Informatics\\
Department of Electrical and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: velten@wisc.edu}
}

==> hardware_pca_onn/Main/authorship_example.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}

==> hardware_pca_onn/Main/custom_sty_edit.tex <==
% re-define the equation environment
\let\oldequation\equation%
\let\endoldequation\endequation%
% \renewenvironment{equation}%
%   {\linenomath\oldequation}{\endoldequation\endlinenomath}%
\expandafter\let\expandafter\oldequationstar\csname equation*\endcsname%
\expandafter\let\expandafter\endoldequationstar\csname endequation*\endcsname%
\renewenvironment{equation*}%
  {\linenomath\oldequationstar}{\endoldequationstar\endlinenomath}%
  

\newcommand{\B}{\boldsymbol}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IZ}{\mathbb{Z}}

\newcommand{\diag}{\text{diag}}

\usepackage{subcaption}

\newcommand{\totphoton}{\mathfrak{N}}
\newcommand{\photon}{\mathfrak{n}}
% \def\totphoton{\left(\rho\tau\right)}

\newcommand{\totexposure}{\tau} %total expo time
\newcommand{\exposure}{\mathfrak{t}} %expo time for each mask
\newcommand{\flux}{\rho} %photons per second



\newcommand{\Xalign}[1]{\begin{aligned}#1\end{aligned}}

\newcommand{\Xequa}[1]{\begin{equation}\Xalign{#1}\end{equation}}




% \def\Xhide#1{\iffalse#1\fi}
\def\Xhide#1{}

\def\noisy#1{\tilde{#1}}
\def\AGN{\mathcal{N}}
\def\Poisson{\mathcal{P}}
\def\Poisson{\mathrm{Poisson}}

% \usepackage{svg}
\usepackage{graphicx} % include PDF figures
\def\Xpolish#1#2{#2}


\def\bnote#1{\textcolor{blue}{#1}}
\def\rnote#1{\textcolor{red} {#1}}
\def\ynote#1{\textcolor{orange}{#1}}
\def\enote#1{\textcolor{violet}{#1}}
\def\YLnote{\rnote}
\def\FGnote#1{\textcolor{brown}{#1}}

\def\ynote#1{\color{orange} #1 \color{black}}
\def\AVnote{\ynote}
\def\TSnote{\bnote}

\def\Bingnote#1{\color{purple} \textit{{#1}} \color{black}}
% \usepackage{pifont}
% \def\checkednote#1{\ding{51} #1}
% \usepackage{soul}
% \usepackage[normalem]{ulem}
% \usepackage{ulem, lipsum}
% \newcommand\xoutpars[1]{\let\helpcmd\xout\parhelp#1\par\relax\relax}
% \newcommand\soutpars[1]{\let\helpcmd\sout\parhelp#1\par\relax\relax}
% \long\def\parhelp#1\par#2\relax{%
%   \helpcmd{#1}\ifx\relax#2\else\par\parhelp#2\relax\fi%
% }

\usepackage[normalem]{ulem}
\def\checkednote#1{\sout{#1}}

%%%%%%network plot
\usepackage{tikz}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary {shapes.misc}
\usepackage{caption}
\usepackage{amsmath,amsfonts}

%%
% \usepackage{slashbox}

%%%% before submit: uncomment the following, OR changing the value of \peerreview in output.tex 
\ifpeerreview
    % \linenumbers\linenumbersep 15pt\relax    
    \def\checkednote#1{} % remove comments
    \def\YLnote{}
\else
    % \linenumbers \linenumbersep 15pt\relax  
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> hardware_pca_onn/Main/to_do.tex <==
add result Figures

add teaser figure

iterate on the intro

small example with 4 pixels

use Low freq Hadamard

==> hardware_pca_onn/sections/1_intro/1_intro.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

% Coding is a fundamental technique used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance. For applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging, coding enables a low dimensional sensor to sample in a \textbf{complete} measurement space.
% %an $n$-dimension measurement space.
% Due to its range of applications, coding schemes have been investigated thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise. It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under the AGN. This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 

% In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.

% Coding is a widely-used technique in computational imaging (CI) that aims to improve image quality and reduce the dimensionality of the measurement space \cite{cossairt2012does}. It has been shown to be effective in a variety of applications, including single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging. These techniques rely on coding to allow low-dimensional sensors to sample a complete measurement space. While coding schemes have been widely studied, most research has focused on low noise scenarios or additive Gaussian noise models. This is due to the fact that additive Gaussian noise, which is introduced by imperfections in cameras and sensors, is easy to model both analytically and computationally as it is a signal-independent linear noise.

\IEEEPARstart{A}{}n imaging device performs a projection from a high-dimensional scene space onto a lower-dimensional reconstruction space. The need for the projection stems partially from a need to reduce and interpret the data, either as a human-interpretable image or as some form of pattern yielding actionable information about the scene. In addition, especially when imaging with visible light, a projection reduces the information to an amount that can be digitized by a camera sensor and processed. Camera sensors are two-dimensional and capture the absolute value squared of the light wave averaged over pixels in space, time, wavelength, and polarization. The projection onto a sensor prior to digitization is thus a fundamental and essential component of any imaging and vision device for physical and computational reasons. One quite general way to model this projection process is through what is commonly referred to as coding or multiplexing. 

\Xhide{\bnote{insert an eqn about the symbols mentioned below}}

Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. \YLnote{The \textbf{single-pixel-imaging} technique is considered as a typical example of this model.} Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x}
    \end{aligned}
\end{equation}
, where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is a set of sensing masks\Xhide{or in other words, weighing design (WD) \cite{harwit1979hadamard} \bnote{not sure if language from 1979 is useful. I have not heard of weighing design},} linearly projecting the field of view onto the sensor pixels, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured \YLnote{flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts.


A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does}\Xhide{\bnote{Define coding here?}} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.

%\rnote{Coding is accomplished by blocking photons over time or space, and more details about the scene can be preserved consequently \cite{raskar2009computational}}. In addition to increasing light throughput, coding can reduce the dimensionality of the measurement space, which is a common metric for the performance of a CI method. Coding allows low-dimensional sensors to sample a complete measurement space in applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging.

% \bnote{This paragraph reads choppily. Many of the sentences could be blended together/ reorganized to be smoother. Potentially combine this with the following paragraph.} While coding schemes have been extensively researched, the mathematical foundation is based on low noise scenarios or Additive Gaussian noise (AGN) models. This is because the AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurements in noisy cameras and sensors, and is easy to analyze and compute analytically as it is signal-independent and linearly additive.

Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 

Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation~\ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not effective under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson}.

\YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
%Previous research has shown that coding behaves differently under Poisson noise compared to AGN \cite{duarte2008CS, harwit1979hadamard, neifeld2003FSI}. Existing coding and computational imaging techniques may not be applicable to these sensors, which makes developing new coding techniques a crucial task. 

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{In this project, we use the popular a single pixel camera design to analyze and design effecive coding models under Poisson noise. Similar to the conclusion of Cossairt et al., Harwid et. al., and Swift et. al., and Willett et. al. we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $M$ \YLnote{\cite{cossairt2012does, harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}.
We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. We propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. 
%This is opposed to compressive sensing strategies, where data is projected into a sparse basis after capture. SS coding strategies can provide a significant improvement on downstream tasks such as correlation analysis and classification in the presence of Poisson noise.
This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of noise on downstream analyses.}

% However, as optical imaging technologies improve, readout noise is decreasing and Poisson noise, due to the quantized nature of light, is becoming more dominant in measured imaging data \bnote{Mention the sensors that make this capable here? By combining with the previous paragraph it could also be made more clear the Poisson noise breaks the underlying assumptions of coding derivations. Mention that the signal-dependent property of Poisson noise is a key factor in why these proofs break down.} \rnote{For instance, Single-photon Avalanche Diode (SPAD) and Photon Multiplier Tube (PMT) are two typical sensors}. Poisson noise is a fundamental physical property of light and arises from the discrete nature of light. An optical signal is composed of discrete photons that can not be arbitrarily divided across codes. Therefore, in state-of-the-art and future sensors measuring visible light, it is important to consider measurement and processing techniques under Poisson noise.

% Previous research has shown that coding behaves substantially differently under Poisson noise compared to the AGN \cite{duarte2008CS}, which is particularly significant in emerging single-photon sensors that only experience Poisson noise. \bnote{Talk more about why Poisson noise is hard to code here.} \rnote{Coding is challenging in this case as it is impossible to remove the Poisson noise without eliminating some of the signal \cite{harwit1979hadamard}}. This means that existing coding and computational imaging techniques may not be applicable to single-photon or "few-photon" sensitive sensors (such as most state-of-the-art CMOS and machine vision cameras) where readout noise is on the order of just a few photons \cite{harwit1979hadamard}.

Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network.
\end{itemize}

While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.

% \bnote{Should we add the example 4-pixel problem and a teaser figure here?}\ynote{I think that makes most sense in the context of compressed sensing. We could add it to the discussion or leave it for the talk.}

\iffalse
\textbf{New paper story:}
\begin{enumerate}
    \item Coding is one of the fundamental techniques used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance.\bnote{Insert definition of computational imaging, probably similar to the one of \cite{cossairt2012does}}.
    \item 
    Coding is important in any application where an n dimensional measurement space is sampled with a sensor or dimensionality $<$ n. It is relevant in single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, polarization imaging, computational imaging, and compressed sensing.
    \item Due to its range of applications coding schemes have been explored thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. 
    \item As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. \item In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise.
    \item It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under AGN.
    % \item For example, recent work explored the regimes where coding/computational imaging can lead to improved performance \cite{cossairt2012does}. The conclusion of their analysis was that coding/computational imaging can improve performance in scenarios where the dominant noise source is due to Gaussian noise often associated to read-out noise. However, when the dominant noise source is Poisson noise, due to the random arrival of photons, the performance gains are negligible. In other words: In a Poisson noise limited measurement, the best "code" is the trivial "pinhole" code, where each sample is scanned on it's own. 
    % \item Beccas paper.
    \item This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 
    \item In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. 
    \item Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.
\end{enumerate}
\fi

\iffalse
\subsection{Outline (for planning only)}
Definition of coding, sensor dimensionality, measurement dimensionality

definition of signal reconstruction, imaging, and pattern recognition

\bnote{Single-pixel imaging.} 

\bnote{Compressive sensing} Compressive sensing has enabled the design of single-pixel imaging systems that are able to reconstruct images from very few measurements. 
These systems are useful in applications where it is expensive to have pixel arrays that sample the full image in parallel. 
For example in low-light applications, PMTs are commonly used, and it is expensive to build arrays of PMTs.

Additionally, compressive sensing can also be applied to other imaging modalities such as hyper-spectral imaging,  fluorescence imaging etc... 

\bnote{Signal reconstruction under Poisson noise.}\ynote{same as before. Shouldn't talk about comprehensive sensing here. Everything we have talked about before is about signal reconstruction} The most efficient compressive sensing systems have been implemented for signal reconstruction under Gaussaian noise. 
Unfortunately, compressive sensing in the presence of Poisson noise does not benefit from the same low-sample complexity \cite{raginsky2011performance}.
This is due to XXX


\bnote{Signal reconstruction amplifies (\rnote{may not necessarily}) noise so we should skip it.} 
Signal reconstruction, however, is often an intermediate step. 
The final goal is often to execute a high-level task such as classification or segmentation.
To this end, current computer vision systems extract features from the reconstructed signal and use these features to accomplish the task at hand.
In this paper, we find that in a single-pixel imaging system under Poisson noise, it is sub-optimal to reconstruct from compressive measurements and then extract features.
This is because the signal reconstruction step amplifies noise.

\bnote{Task Specific Masks vs General Masks}
Should we adapt our masks based on our objective (pattern recognition task, image reconstruction domain, different types of signals)? The conventional wisdom for AGN is that that doesn't help much. 

Now we need to do analysis:
define toy problems, discuss performance for simple adaptive masks
conclusion: with Poisson noise signal reconstruction makes no sense. But pattern recognition works with an adapted mask set.

How do we find the masks:
PCA, ONN

\bnote{Optical neural nets to the rescue.} 
Inspired by recent trends in optical neural networks, we propose a single-pixel vision system for low-light applications. 
By capturing image features directly we avoid amplifying noise

\bnote{How to design these masks.} 

Discussion:
end to end computational imaging with adaptive asks works under Poisson noise.

This provides an additional motivation for proposed optical ANNs or ANNs with optical layers. Such an architecture allows me to choose where in the design I want to add the Poisson noise.

Possibly: Quantum mechanics interpretation.
\fi

==> hardware_pca_onn/sections/1_intro/1_intro_2023_11_30.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi



\IEEEPARstart{I}{}n imaging devices, a crucial step involves projecting information from a high-dimensional scene space onto a lower-dimensional reconstruction space. This projection serves the dual purpose of data reduction for human interpretation and the extraction of actionable patterns pertaining to the scene. Information from a 3D scene involving color, timing, polarization, and phase has to be encoded on a 2 dimensional image sensor. This process, often termed coding or multiplexing, is a fundamental and essential aspect of both physical and computational considerations in imaging and vision devices.

Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. The \textbf{single-pixel-camera} is considered as a typical example of this model. Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view (FOV), $\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts.

In this work we will study the performance of this camera for different choices of $\B{M}$ under different noise models. The single pixel camera is intended specifically as a toy model that exhibits the more general dimensional reduction problem experienced by all imaging devices. Our goal is to design $\B{M}$ such that it allows us to extract desired information from the scene when combined with digital processing. In other words, we seek to design an end to end vision system and consider both the physical and the digital part of the design. While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.


%A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.



% Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 
Coding schemes, often developed under signal independent Additive Gaussian Noise (AGN), provide a mathematically tractable framework. While AGN is suitable to model certain types of noise introduced by the measurement device, it does not correctly model Poisson noise which is signal-dependent. In almost all modern cameras and sensors, however, Poisson noise is predominant, especially in advanced sensors like Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}.  This necessitates a reevaluation of coding strategies tailored to this noise type.

% Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation \ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not recommended under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Poisson noise, a fundamental property of light, arises due to the discrete nature of light measurements. Unlike the assumptions of the linear model in Eq.  \ref{eqn:NoiselessMeasurement}, it's impossible to distribute a photon measurement across all open pixels in a mask. Consequently, the measurements $\B{y}$ called for by the equation are unattainable by linear reconstruction approaches. This renders coding and compressed sensing approaches, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. The optimal code, denoted as $\B{M}_P$, for measurements limited by real Poisson noise must converge to $\B{M}_G$ applicable to the optimal code under Additive Gaussian Noise (AGN) or under no noise as the number of measured photons tends toward infinity. However, it is crucial to highlight that, as demonstrated below, $\B{M}_P$ does not necessarily exhibit similarity to $\B{M}_G$ for any finite number of photons.

\AVnote{\checkednote{The optimal code $\B{M}_P$ for a real Poisson noise limited measurement has to approach the $\B{M}_G$ for a noise-less measurement or one under AGN as the number of measured photons goes to infinity. Crucially, however, as we will show below $\B{M}_P$ does not become similar to $\B{M}_G$ for any finite number of photons.}}

% \YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
\Xhide{
\Xpolish{In most of the papers, people optimize the algorithms on reconstruction but keep using random coding \cite{goyal2016performance}. Some other work, such as Feature Specific Imaging (FSI) does optimize the sensing matrices based on some learn-able priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, but how to optimize masks under Poisson noise remains an unsolved problem \cite{neifeld2014optimizing}. Meanwhile, some attempts on matrix optimization based on minimal mutual coherence are not based on Poisson noise model itself \cite{mordechay2014matrixRIP} and is proved defective in this paper.}
{
\AVnote{this seems like it belongs into related work}
In many papers, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}  \YLnote{need more here}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methids explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}
}

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{In this project, we use the popular single pixel camera design to analyze and design effective coding models under Poisson noise. Similar to the conclusion of Cossairt et al., Harwid et. al., and Swift et. al., and Willett et. al. we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $\B{M}$ \YLnote{\cite{cossairt2012does, harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}.
We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. We propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of noise on downstream analyses.}



Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel cameras.}
\end{itemize}

\Xpolish{While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.}
{
Our work, although rooted in compressed sensing principles applicable to regularized image reconstruction, specifically addresses two extreme scenarios. The first involves non-compressible data with full-rank measurements, reconstructed without regularization. Conversely, we examine highly compressible data in image classification, projecting images into a minimal feature space where the impact of Poisson noise becomes particularly evident.}
\AVnote{\checkednote{Add a figure showing different vision tasks with different compressibilities}}





==> hardware_pca_onn/sections/1_intro/1_intro_2024_01_03.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi



\YLnote{poisson is not considered before. we developed a simple vision system to address that and compare the noise models impacts}
\YLnote{https://ieeexplore.ieee.org/document/6637874, https://www.nature.com/articles/srep41435.pdf, https://compphotolab.northwestern.edu/wordpress/wp-content/uploads/2015/04/BeatHadamard.pdf}

\IEEEPARstart{T}{}he projection of \checkednote{information} information from a high-dimensional scene space involving color, timing, polarization, and phase onto a lower-dimensional reconstruction space is crucial step in any imaging and vision device. This projection serves the dual purpose of data reduction to fit the limited number of values that can be digitized and processed by the hardware and the extraction of actionable patterns. This process, often termed coding or multiplexing, is a fundamental and essential aspect of both physical and computational considerations in imaging and vision devices. 
In this project, the primary objective is to optimize coding schemes, with a particular emphasis on selecting the appropriate noise model.

\Xhide{Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. }
The \textbf{single-pixel-camera} \Xpolish{demonstrated}{shown} in Fig. \ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}. Supposing the image representation of the field of view (FOV) $\B{x} \in \IR^{N \times 1}$ consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ \Xpolish{projections}{measurements, whose photon counts are denoted as $\B{y} \in \IR^{m \times 1}$}, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where \Xhide{$\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, }$\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel\Xhide{, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts }\cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light from $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-rank, \Xpolish{this model accurately characterizes conventional single-pixel imaging scenarios}{the \Xpolish{FOV}{$\B{x}$} can be reconstructed by $\B{M}^{-1}\B{y}$}. However, even when $m < N$, \Xhide{the model remains effective through the integration of regularization techniques, specifically }{we can still recover the \Xpolish{FOV}{$\B{x}$} via} compressed sensing.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct Measurement Strategy: Raster Scan}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational Imaging (CI) Strategy: Basis Scan}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

In this work we will study the performance of this camera for different choices of $\B{M}$ under different noise models. \Xhide{The single pixel camera is intended specifically as a toy model that exhibits the more general dimensional reduction problem experienced by all imaging devices. Our goal is to design $\B{M}$ such that it allows us to extract desired information from the scene when combined with digital processing. In other words, we seek to design an end to end vision system and consider both the physical and the digital part of the design. }While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.


%A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.



% Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 
Coding schemes, often developed under signal independent Additive Gaussian Noise (AGN), provide a mathematically tractable framework. While AGN is suitable to model certain types of noise introduced by the measurement device, it does not correctly model Poisson noise\YLnote{\Xhide{even after quantization }\cite{yang2015poisson}}\Xhide{ which is signal-dependent and not avoidable via better sensor fabrication techniques. \Xhide{In almost all modern cameras and sensors, however, Poisson noise is predominant, especially in advanced sensors like Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}.  }This necessitates a reevaluation of coding strategies tailored to this noise type}.

% Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation \ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not recommended under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Poisson noise, a fundamental property of light, arises due to the discrete and random nature of light measurements. \AVnote{\checkednote{ This sentence doesn't seem to make sense Jan 18, 2024 9:41 AM}}\YLnote{\Xpolish{Unlike the assumptions of the linear model in Eq.  \ref{eqn:NoiselessMeasurement},}{Different from AGN, Poisson noise is discrete}} and it is impossible to distribute a photon measurement across all open pixels in a mask. Consequently, linear reconstruction approaches based on the measurements $\B{y}$ called for by the \YLnote{\Xpolish{quation}{Eq.  \ref{eqn:NoiselessMeasurement}}} are \Xpolish{\Xpolish{unattainable}{unsatisfactory}}{unattainable}\Xhide{ by linear reconstruction approaches}. This renders coding and compressed sensing approaches\YLnote{\checkednote{more about  compressed sensing}}, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. \Xhide{The optimal code, denoted as $\B{M}_P$, for measurements limited by real Poisson noise must converge to $\B{M}_G$ applicable to the optimal code under Additive Gaussian Noise (AGN) or under no noise as the number of measured photons tends toward infinity. However, it is crucial to highlight that, as demonstrated below, $\B{M}_P$ does not necessarily exhibit similarity to $\B{M}_G$ for any finite number of photons.}

\AVnote{\checkednote{The optimal code $\B{M}_P$ for a real Poisson noise limited measurement has to approach the $\B{M}_G$ for a noise-less measurement or one under AGN as the number of measured photons goes to infinity. Crucially, however, as we will show below $\B{M}_P$ does not become similar to $\B{M}_G$ for any finite number of photons.}}

% \YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
\Xhide{
\Xpolish{In most of the papers, people optimize the algorithms on reconstruction but keep using random coding \cite{goyal2016performance}. Some other work, such as Feature Specific Imaging (FSI) does optimize the sensing matrices based on some learn-able priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, but how to optimize masks under Poisson noise remains an unsolved problem \cite{neifeld2014optimizing}. Meanwhile, some attempts on matrix optimization based on minimal mutual coherence are not based on Poisson noise model itself \cite{mordechay2014matrixRIP} and is proved defective in this paper.}
{
\AVnote{this seems like it belongs into related work}
In many papers, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}  \YLnote{need more here}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methids explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}
}


\Xhide{\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{\Xhide{In this project, we use the popular single pixel camera design to analyze and design effective coding models under Poisson noise. } Therefore, we propose a coding methodology called \textbf{Selective Sensing} (SS) \Xpolish{that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time}{specifically optimized for Poissonian data}. This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of Poisson noise on downstream analyses.}
}%hide old versions
\AVnote{\checkednote{velten: This still comes out of nowhere. So far we have mostly talked about image reconstruction and reconstructing and image x. Now we talk about a vision problem and character recognition.
Maybe Figire 1 should have another component after x that is the output of the vision system or the pattern. That could also be an image. Or we have to say that x is not necessarily and image but could be something else.
Jan 18, 2024 9:50 AM}}
\YLnote{Alternatively, we propose a coding methodology called \textbf{Selective Sensing} (SS) specifically optimized for Poissonian data acquisition. SS focuses on the retention of the key information from some prior knowledge and reducing the impact of Poisson noise for the downstream computer vision tasks, e.g. classification, instead of general reconstruction of $\B{x}$. Its classification performance most closely approaches the theoretical upper limit among all imaging strategies.
}





Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $\B{M}$ {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extracting the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel cameras.}
\end{itemize}

\Xhide{\Xpolish{While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.}
{
Our work, although rooted in compressed sensing principles applicable to regularized image reconstruction, specifically addresses two extreme scenarios. The first involves non-compressible data with full-rank measurements, reconstructed without regularization. Conversely, we examine highly compressible data in image classification, projecting images into a minimal feature space where the impact of Poisson noise becomes particularly evident.}
\AVnote{\checkednote{Add a figure showing different vision tasks with different compressibilities}}}





==> hardware_pca_onn/sections/1_intro/1_intro_2024_03_01.tex <==
% \IEEEPARstart{T}{}

\Xpolish{Optical coding, or multiplexing, is a common technology in computational imaging (CI) as it is believed to be able to acquire a better SNR with greater light throughput \cite{mitra2014can}. However, the recovery of the image also depends on the conditioning of coding matrices as a non-optimal coding matrix can even degrade the vision system's recovery performance \cite{mitra2014can}.}{
\IEEEPARstart{O}{}ptical coding, also known as multiplexing, is a prevalent technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput \cite{mitra2014can}. The successful recovery of images, however, also depends on the conditioning of the coding matrices. Suboptimal coding matrices have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes is intricately linked to the characteristics of noise, a facet that has not been extensively emphasized previously. Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents Poisson noise \cite{yang2015poisson} arising intrinsically due to the discrete and random nature of light measurements. The optimization behaviors of coding manifest notable distinctions under low-light conditions where Gaussian noise dominates and high-light conditions where Poisson noise prevails \cite{mitra2014can}, suggesting coding and compressed sensing approaches, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. In this project, the primary objective is to optimize coding schemes, with a particular emphasis on selecting the appropriate noise model.
}



The \textbf{single-pixel-camera} \Xpolish{demonstrated}{shown} in Fig. \ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}. Supposing the image representation of the field of view (FOV) $\B{x} \in \IR^{N \times 1}$ consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ \Xpolish{projections}{measurements, whose photon counts are denoted as $\B{y} \in \IR^{m \times 1}$}, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where \Xhide{$\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, }$\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel\Xhide{, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts }\cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light from $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-rank, \Xpolish{this model accurately characterizes conventional single-pixel imaging scenarios}{the \Xpolish{FOV}{$\B{x}$} can be reconstructed by $\B{M}^{-1}\B{y}$}. However, even when $m < N$, \Xhide{the model remains effective through the integration of regularization techniques, specifically }{we can still recover the \Xpolish{FOV}{$\B{x}$} via} compressed sensing.

==> hardware_pca_onn/sections/1_intro/1_intro_2024_03_02.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi


\IEEEPARstart{O}{}ptical coding, also known as multiplexing, is a \Xpolish{prevalent}{popular} technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput thank point by point measurements\cite{mitra2014can}. The recovery quality of images, however, also depends on the conditioning of the coding matrices \cite{mitra2014can}. Suboptimal coding matrices have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes is intricately linked to the characteristics of noise, a facet that has not been extensively emphasized previously. Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents Poisson noise \cite{yang2015poisson} arising intrinsically due to the discrete and random nature of light measurements. The optimization behaviors of coding manifest notable distinctions under low-light conditions where Gaussian noise dominates and high-light conditions where Poisson noise prevails \cite{mitra2014can}, suggesting coding and compressed sensing approaches designed for effectiveness under the AGN or noiseless conditions unsuitable under Poisson noise. Existing literature strongly discourages their utilization in such situations \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. \YLnote{This issue was first identified by Mitra et al \cite{mitra2014can} but has not received significant attention.} \Xpolish{As Mitra et al. highlighted, a data-driven prior can significantly improve the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}, the cost function based on L2 error metric lacks fundamental perceptual information \cite{mitra2014can}. In this project, the primary objectives is to better identify the role of data-driven prior in computer vision tasks on a more meaningful metric, and further fix the limitations when learning that prior in provious models.}{
As emphasized by Mitra et al., leveraging a data-driven prior can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. However, the cost function based on the L2 error metric lacks essential perceptual information \cite{mitra2014can}. Our study aims to illustrating why AGN is not suitable for optimizing coding under Poisson noise by direct comparison, elucidating the nuanced impact of a data-driven prior on computer vision tasks using more meaningful metrics, and addressing limitations encountered in previous models during the learning \Xhide{process }of such priors and the optimization of coding schemes.
}

\Bingnote{{Clarity and Focus: Ensure the introduction clearly states the problem and the proposed solution. It should succinctly explain why Poisson noise is significant and how it affects imaging systems.}}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct Measurement Strategy: Raster Scan}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational Imaging (CI) Strategy: Basis Scan}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

The \textbf{single-pixel-camera} \Xpolish{demonstrated}{shown} in Fig. \ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}, and serves as the primary example in this project. \YLnote{It employs a rapid single-pixel detector in conjunction with a Digital Micromirror Device (DMD) to sequentially multiplex a sensing matrix by modulating various patterns on the DMD \cite{mitra2014can}.} Supposing the image representation of the field of view (FOV) $\B{x} \in \IR^{N \times 1}$ consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ \Xpolish{projections}{measurements, whose photon counts are denoted as $\B{y} \in \IR^{m \times 1}$}, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where \Xhide{$\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, }$\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the \Xpolish{FOV}{$\B{x}$} onto the sensor pixel\Xhide{, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts }\cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light from $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-rank, \Xpolish{this model accurately characterizes conventional single-pixel imaging scenarios}{the \Xpolish{FOV}{$\B{x}$} can be reconstructed by $\B{M}^{-1}\B{y}$}. However, even when $m < N$, \Xhide{the model remains effective through the integration of regularization techniques, specifically }{we can still recover the \Xpolish{FOV}{$\B{x}$} via} compressed sensing. \YLnote{While Hadamard matrices are considered effective for $\B{M}$, their suitability diminishes in the presence of data-dependent noise \cite{mitra2014can, harwit1979hadamard}.} In this work, we will study the performance of this camera for different choices of $\B{M}$ under different noise models. While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.

\Bingnote{Provide a brief background on existing coding schemes and their limitations with Poisson noise. This sets the stage for the importance of your work.}

Our contributions are as listed.
\begin{itemize} 
% \item We analyze the performance of coding techniques for  using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise individually, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding \YLnote{using Hadamard and random matrices} provides no benefit over a trivial raster scanning approach under Poisson noise using an identity matrix as $\B{M}$  {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits \Xpolish{to those seen in compressed sensing and computational imaging}{in classification rate which is more perceptually meaningful metric} can be seen if appropriate adjustments to the measurement matrices are made. 
\item We assert that coding can yield substantial performance improvements under Poisson noise \textit{only} when codes used in hardware capture are optimized specifically for downstream vision tasks, which extend beyond naive image reconstruction to include promising classification.
\item \Xpolish{We propose the methodology of selective sensing (SS) which includes coding methods selectively extracting the data-driven priors and can be directly combined with models for downstream tasks.}{We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.}
\item We provide a model to \Xpolish{create masks optimized}{optimize $\B{M}$} for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel vision systems.} 
Addressing the limitations identified by Mitra et al. \cite{mitra2014can}, this model presents the following advantages.
    \begin{itemize}
        \item The optimization of coding relies on the gradient descent algorithm, leading to the determination of a globally optimal matrix $\B{M}$ rather than its greedy approximation.
        \item Noise is incorporated during the training process to simulate real-world conditions, deviating from the assumption of a one-dimensional affine noise model.
        \item The training process is accelerated and computationally more efficient due to the binary constraint being addressed even in real experiments. Additionally, the prior is learned from the entirety of the light fields and spectral data, rather than from patches.
        \item The contribution of a data-driven prior to performance enhancement is more accurately discerned when evaluating this model using the classification rate, a metric that holds superior interpretability in terms of visual perceptual meaning compared to the reconstruction error.
    \end{itemize}
\end{itemize}


==> hardware_pca_onn/sections/1_intro/1_intro_2024_04_01.tex <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi


\IEEEPARstart{O}{}ptical coding, also known as multiplexing, is a popular technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. If ignoring the noise, coding is represented as 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector, $\B{M}$ is the sensing matrix, and $\B{y}$ is the measured vector. Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$. The recovery quality of $\B{x}$, however, also depends on the conditioning of the $\B{M}$ besides the light throughput \cite{mitra2014can}. Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents Poisson noise \cite{yang2015poisson} arising intrinsically due to the discrete and random nature of photon measurements. The optimization behaviors of coding manifest notable distinctions under low-light conditions where Gaussian noise dominates and high-light conditions where Poisson noise prevails \cite{mitra2014can}, suggesting coding and compressed sensing approaches designed for effectiveness under the AGN or noiseless conditions unsuitable under Poisson noise. It has been shown that in that case without the use of priors for regularization, coding does not provide an improvement over a simple sequential scan \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. 
Mitra et. al. \cite{mitra2014can} develop a data driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. \YLnote{An important conclusion is that if the signal exhibits sparsity and thereby  compressibility, signal optimized coding can improve recovery performance under Poisson noise and the amount of improvement is directly related to the comprehensibility of the measured data. However, recovery is typically not the ultimate goal for modern vision systems.} Furthermore, the cost function based on the L2 error metric in that project lacks essential perceptual information \cite{mitra2014can}. \YLnote{Since vision tasks, such as classification, operate in embeddings created from images their data should be inherently more compressible than their upstream imaging tasks. Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.} To show this, our study implements a simple end to end vision system that can be optimized  under different noise assumptions. We illustrate why AGN is not suitable for optimizing coding under Poisson noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when only photon noise is present.
% }

% If the signal is sparse and compressible, it is possible to have a better recovery performance under Poisson noise. However, recovery is usually not the final objective for modern vision systems. Vision tasks, such as classification, usually present greater compressibility than their upstream imaging tasks. If the signal compressibility is the answer, we should skip the intermediate imaging step and directly code for better feature extracting for next vision tasks to attain the best compressibility and therefore, better performances under Poisson noise.

Our contributions are as listed.
\begin{itemize} 
% \item We analyze the performance of coding techniques for  using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise individually, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding \YLnote{using Hadamard and random matrices} provides no benefit over a trivial raster scanning approach under Poisson noise using an identity matrix\Xhide{ as $\B{M}$} {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is highly compressible, substantial improvements in classification rate can be seen if appropriate adjustments to the measurement matrices are made. In these scenarios the compressive vision system performance approaches the performance of a non-coded camera.
\item We assert that coding can yield substantial performance improvements under Poisson noise \textit{only} when codes used in hardware capture are optimized specifically for downstream vision tasks.
\item \Xpolish{We propose the methodology of selective sensing (SS) which includes coding methods selectively extracting the data-driven priors and can be directly combined with models for downstream tasks.}{We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.}
\item We provide a model to \Xpolish{create masks optimized}{optimize $\B{M}$} for Poisson noise using neural network model. \YLnote{We find optimized measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel vision systems.} 
Addressing the limitations identified by Mitra et al. \cite{mitra2014can}, this model presents the following advantages.
    \begin{itemize}
        \item The optimization of coding relies on the gradient descent algorithm, leading to the determination of a globally optimal $\B{M}$ rather than its greedy approximation.
        \item Noise is incorporated during the training process to simulate real-world conditions, deviating from the assumption of a one-dimensional affine noise model.
        \item The training process is accelerated and computationally more efficient due to the binary constraint being addressed even in real experiments. Additionally, the prior is learned from the entirety of the light fields and spectral data, rather than from patches.
        \item The contribution of a data-driven prior to performance enhancement is more accurately discerned when evaluating this model using the classification rate, a metric that holds superior interpretability in terms of visual perceptual meaning compared to the reconstruction error.
    \end{itemize}
\end{itemize}


==> hardware_pca_onn/sections/1_intro/1_intro_2024_04_11.tex <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

\AVnote{\checkednote{Lets try to make the text about machine vision system optimization. Could start with: While we have the ability to mass produce optical components of increasing complexity, creation of human interpretable imaging by closely following the optics of the human eye is still the design principle of most vision hardware. We use a single pixel camera relying on optical coding as a test bed system to optimize. This system can produce images, but allows great freedom to perform alternative measurements while being easily described mathematically.}}

% \YLnote{\IEEEPARstart{D}{}espite advances in mass-producing complex optical components, most vision systems still follow the template of human vision where the optics create a two dimensional image that is then digitized and processed. A more general imaging system that has been extensively studied is the single-pixel camera that relies on masks to perform coded measurements from which images are computed. This setup also offers flexibility for alternative measurements, with straightforward mathematical descriptions.} 


% While we have the ability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely follows the optics of the human eye to create human-interpretable imaging. However, the more generalized vision systems can also perform alternative measurement which can be easily described in mathematical ways and is more perceptually meaningful than just producing images. We use a single-pixel camera, which can be seen as a system in this kind,  relying on masks to perform coded measurements as a test bed for hardware optimization.

% can depend on direct measurement with visual perception as well. We use a single-pixel camera relying on masks to perform coded measurements from which images are computed as a test bed to optimize, as it not only can produce images but also allows great freedom to perform alternative measurements while being easily described mathematically.

\IEEEPARstart{W}{}hile we possess the capability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely mimics the optics of the human eye to create human-interpretable imaging. However, more generalized vision systems can also perform alternative coded measurements that are not only easily described mathematically but also potentially more perceptually meaningful than merely producing images. We employ a single-pixel camera as a test bed for hardware optimization, which exemplifies such a system, relying on masks to conduct optically-coded measurements. 

% Optical coding, also known as multiplexing, is a popular technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. If ignoring the noise, coding is represented as 
%  \begin{equation}
%     \label{eqn:NoiselessMeasurement}
%     \begin{aligned}
%         \B{y} &=  \B{M x} ,
%     \end{aligned}
% \end{equation}
% where $\B{x}$ is the signal vector, $\B{M}$ is the sensing matrix, and $\B{y}$ is the measured vector. 

% Maybe: For optical coding or multiplexing an image is prjoected onto a mask and only light transmitted to the mask is collected by a single large sensor pixel. A measurement consists of a set of measurements expressed as a vector y with a set of masks. The vectiruzed masks form the rows of the measurement matrix M.

% Optical coding, or multiplexing, is a popular technology projecting an image onto a mask and collecting the light transmitting it by a large senor pixel. It potentially achieves enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. A measurement consists of a set of measurements expressed as a vector $\B{y}$ with a set of masks vectorized as the rows of the measurement matrix $\B{M}$. If ignoring the noise, coding is represented as 

Optical coding, or multiplexing, is a popular technology that projects an image onto a mask and collects the light transmitted through it using a large sensor pixel. It potentially achieves an enhanced signal-to-noise ratio (SNR) and greater light throughput compared to point-by-point measurements \cite{mitra2014can}. A measurement vector $\B{y}$ consists of a set of measured photon counts, with the corresponding masks vectorized as the rows of the sensing matrix $\B{M}$. Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 

Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$. The recovery quality of $\B{x}$, however, also depends on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}. Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 
%---- delete
\iffalse
{
Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. 
However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents \Xpolish{Poisson noise arising intrinsically due to the discrete and random nature of photon measurements}{\YLnote{\Xpolish{photon noise which arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables despite that it is indeed super-Possionian. However, we continue to use the term "Poisson noise" to maintain consistency with the terminology commonly found in the literature.}{Photon noise arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables, even though it is actually super-Poissonian. However, we continue to use the term "Poisson noise" to maintain consistency with the terminology commonly found in the literature.}}} \AVnote{\checkednote{Lets call it photon noise. Photon noise is more complex and Poisson distribution is just an approximation. Then we can explain later that the key feature to model is the fact that the variance depends on the mean.}}\cite{yang2015poisson}Past works usually distinguish between low-light regimes, where AGN introduced by imperfect sensors dominates, and bright-light regimes, where the physical photon noise dominates \cite{mitra2014can}. With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel. This reduction is significant enough that photon noise becomes the primary noise factor in the vast majority of imaging applications. }
\fi
%----
\YLnote{
Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN) which arises from imperfect sensors and is introduced from the low-light regimes in many past works, offer a mathematically tractable framework. With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel. This reduction is significant enough that photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise is intrinsically signal-dependent \cite{cossairt2012does} and usually approximated by Poisson noise, even though it is actually \textbf{super-Poissonian} \cite{mandel1959fluctuations}. 
% In this work, we focus on its signal-dependent feature and propose 
% arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables. 
}
\YLnote{Unfortunately, the effects of changing the noise model are not subtle as designs that are optimal under AGN conditions often fail to approximate optimal designs under photon noise.
%
The intensity dependence of photon noise renders the camera a nonlinear system, necessitating nonlinear optimization methods. Linear optics are only truly linear in the limit of infinite photons, where quantum noise vanishes. Consequently, the linear approximation frequently used is not applicable at finite light levels.}\AVnote{\checkednote{Add here: Unfortunately, the effect of changing the noise model are not subtle. Designs optimal under AGN are usually not even approximations of optimal designs under photon noise. In fact, the intensity dependence of the noise turns the camera into a nonlinear system requiring nonlinear optimization approaches. Linear optics are only truly linear at the infinite photon limit where quantum noise disappears. The linear approximation commonly used is not applicable at any finite light level. }} 
\AVnote{\checkednote{ While this issue affects any camera optic it has been studied extensively in the context of single pixel and compressed sensing cameras that rely on coding. For example, it has been shown, that while a single pixel camera provides performance advantages under AGN, in the case of  Poisson noise that more closely resembles photon noise, coding does not ....}}  \YLnote{\Xpolish{It has been shown that in that case without the use of priors for regularization, coding does not provide an improvement over a simple sequential scan}{ While this issue impacts all camera optics, it has been extensively studied in the context of single-pixel and compressed sensing cameras that rely on coding techniques. }
For instance, although single-pixel cameras demonstrate performance advantages under AGN, coding does not offer improvements over a simple sequential scan when dealing with \Xpolish{Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}, which more closely resembles photon noise.}{photon noise, or Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.}
}
{
Mitra et al. \cite{mitra2014can} develop a data driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. \YLnote{An important conclusion is that if the signal exhibits sparsity and thereby  compressibility, signal optimized coding can improve recovery performance under signal-dependent noise and the amount of improvement is directly related to the comprehensibility of the measured data. However, recovery is typically not the ultimate goal for modern vision systems.}
}{
\YLnote{Since vision tasks, such as classification, operate in embeddings created from images their data should be inherently more compressible than their upstream imaging tasks. Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.} To show this, our study implements a simple end to end vision system that can be optimized  under different noise assumptions. We illustrate why AGN is not suitable for optimizing coding under \Xpolish{Poisson}{photon} noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }photon noise is present.
}

Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. \YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}
\item \Xpolish{We provide a model to {optimize $\B{M}$} for Poisson noise using neural network model. This model is end to end vision model with classification as the performance metric}{
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

==> hardware_pca_onn/sections/1_intro/1_intro_2024_08_18.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

% Coding is a fundamental technique used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance. For applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging, coding enables a low dimensional sensor to sample in a \textbf{complete} measurement space.
% %an $n$-dimension measurement space.
% Due to its range of applications, coding schemes have been investigated thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise. It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under the AGN. This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 

% In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.

% Coding is a widely-used technique in computational imaging (CI) that aims to improve image quality and reduce the dimensionality of the measurement space \cite{cossairt2012does}. It has been shown to be effective in a variety of applications, including single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging. These techniques rely on coding to allow low-dimensional sensors to sample a complete measurement space. While coding schemes have been widely studied, most research has focused on low noise scenarios or additive Gaussian noise models. This is due to the fact that additive Gaussian noise, which is introduced by imperfections in cameras and sensors, is easy to model both analytically and computationally as it is a signal-independent linear noise.

\IEEEPARstart{A}{}n imaging device performs a projection from a high-dimensional scene space onto a lower-dimensional reconstruction space. The need for the projection stems partially from a need to reduce and interpret the data, either as a human-interpretable image or as some form of pattern yielding actionable information about the scene. In addition, especially when imaging with visible light, a projection reduces the information to an amount that can be digitized by a camera sensor and processed. Camera sensors are two-dimensional and capture the absolute value squared of the light wave averaged over pixels in space, time, wavelength, and polarization. The projection onto a sensor prior to digitization is thus a fundamental and essential component of any imaging and vision device for physical and computational reasons. One quite general way to model this projection process is through what is commonly referred to as coding or multiplexing. 

\Xhide{\bnote{insert an eqn about the symbols mentioned below}}

Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. \YLnote{The \textbf{single-pixel-imaging} technique is considered as a typical example of this model.} Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x}
    \end{aligned}
\end{equation}
, where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is a set of sensing masks\Xhide{or in other words, weighing design (WD) \cite{harwit1979hadamard} \bnote{not sure if language from 1979 is useful. I have not heard of weighing design},} linearly projecting the field of view onto the sensor pixels, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured \YLnote{flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts.


A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does}\Xhide{\bnote{Define coding here?}} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.

%\rnote{Coding is accomplished by blocking photons over time or space, and more details about the scene can be preserved consequently \cite{raskar2009computational}}. In addition to increasing light throughput, coding can reduce the dimensionality of the measurement space, which is a common metric for the performance of a CI method. Coding allows low-dimensional sensors to sample a complete measurement space in applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging.

% \bnote{This paragraph reads choppily. Many of the sentences could be blended together/ reorganized to be smoother. Potentially combine this with the following paragraph.} While coding schemes have been extensively researched, the mathematical foundation is based on low noise scenarios or Additive Gaussian noise (AGN) models. This is because the AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurements in noisy cameras and sensors, and is easy to analyze and compute analytically as it is signal-independent and linearly additive.

Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 

Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation~\ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not effective under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson}.

\YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
%Previous research has shown that coding behaves differently under Poisson noise compared to AGN \cite{duarte2008CS, harwit1979hadamard, neifeld2003FSI}. Existing coding and computational imaging techniques may not be applicable to these sensors, which makes developing new coding techniques a crucial task. 

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{In this project, we use the popular a single pixel camera design to analyze and design effecive coding models under Poisson noise. Similar to the conclusion of Cossairt et al., Harwid et. al., and Swift et. al., and Willett et. al. we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $M$ \YLnote{\cite{cossairt2012does, harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}.
We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. We propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. 
%This is opposed to compressive sensing strategies, where data is projected into a sparse basis after capture. SS coding strategies can provide a significant improvement on downstream tasks such as correlation analysis and classification in the presence of Poisson noise.
This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of noise on downstream analyses.}

% However, as optical imaging technologies improve, readout noise is decreasing and Poisson noise, due to the quantized nature of light, is becoming more dominant in measured imaging data \bnote{Mention the sensors that make this capable here? By combining with the previous paragraph it could also be made more clear the Poisson noise breaks the underlying assumptions of coding derivations. Mention that the signal-dependent property of Poisson noise is a key factor in why these proofs break down.} \rnote{For instance, Single-photon Avalanche Diode (SPAD) and Photon Multiplier Tube (PMT) are two typical sensors}. Poisson noise is a fundamental physical property of light and arises from the discrete nature of light. An optical signal is composed of discrete photons that can not be arbitrarily divided across codes. Therefore, in state-of-the-art and future sensors measuring visible light, it is important to consider measurement and processing techniques under Poisson noise.

% Previous research has shown that coding behaves substantially differently under Poisson noise compared to the AGN \cite{duarte2008CS}, which is particularly significant in emerging single-photon sensors that only experience Poisson noise. \bnote{Talk more about why Poisson noise is hard to code here.} \rnote{Coding is challenging in this case as it is impossible to remove the Poisson noise without eliminating some of the signal \cite{harwit1979hadamard}}. This means that existing coding and computational imaging techniques may not be applicable to single-photon or "few-photon" sensitive sensors (such as most state-of-the-art CMOS and machine vision cameras) where readout noise is on the order of just a few photons \cite{harwit1979hadamard}.

Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network.
\end{itemize}

While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.

% \bnote{Should we add the example 4-pixel problem and a teaser figure here?}\ynote{I think that makes most sense in the context of compressed sensing. We could add it to the discussion or leave it for the talk.}

\iffalse
\textbf{New paper story:}
\begin{enumerate}
    \item Coding is one of the fundamental techniques used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance.\bnote{Insert definition of computational imaging, probably similar to the one of \cite{cossairt2012does}}.
    \item 
    Coding is important in any application where an n dimensional measurement space is sampled with a sensor or dimensionality $<$ n. It is relevant in single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, polarization imaging, computational imaging, and compressed sensing.
    \item Due to its range of applications coding schemes have been explored thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. 
    \item As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. \item In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise.
    \item It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under AGN.
    % \item For example, recent work explored the regimes where coding/computational imaging can lead to improved performance \cite{cossairt2012does}. The conclusion of their analysis was that coding/computational imaging can improve performance in scenarios where the dominant noise source is due to Gaussian noise often associated to read-out noise. However, when the dominant noise source is Poisson noise, due to the random arrival of photons, the performance gains are negligible. In other words: In a Poisson noise limited measurement, the best "code" is the trivial "pinhole" code, where each sample is scanned on it's own. 
    % \item Beccas paper.
    \item This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 
    \item In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. 
    \item Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.
\end{enumerate}
\fi

\iffalse
\subsection{Outline (for planning only)}
Definition of coding, sensor dimensionality, measurement dimensionality

definition of signal reconstruction, imaging, and pattern recognition

\bnote{Single-pixel imaging.} 

\bnote{Compressive sensing} Compressive sensing has enabled the design of single-pixel imaging systems that are able to reconstruct images from very few measurements. 
These systems are useful in applications where it is expensive to have pixel arrays that sample the full image in parallel. 
For example in low-light applications, PMTs are commonly used, and it is expensive to build arrays of PMTs.

Additionally, compressive sensing can also be applied to other imaging modalities such as hyper-spectral imaging,  fluorescence imaging etc... 

\bnote{Signal reconstruction under Poisson noise.}\ynote{same as before. Shouldn't talk about comprehensive sensing here. Everything we have talked about before is about signal reconstruction} The most efficient compressive sensing systems have been implemented for signal reconstruction under Gaussaian noise. 
Unfortunately, compressive sensing in the presence of Poisson noise does not benefit from the same low-sample complexity \cite{raginsky2011performance}.
This is due to XXX


\bnote{Signal reconstruction amplifies (\rnote{may not necessarily}) noise so we should skip it.} 
Signal reconstruction, however, is often an intermediate step. 
The final goal is often to execute a high-level task such as classification or segmentation.
To this end, current computer vision systems extract features from the reconstructed signal and use these features to accomplish the task at hand.
In this paper, we find that in a single-pixel imaging system under Poisson noise, it is sub-optimal to reconstruct from compressive measurements and then extract features.
This is because the signal reconstruction step amplifies noise.

\bnote{Task Specific Masks vs General Masks}
Should we adapt our masks based on our objective (pattern recognition task, image reconstruction domain, different types of signals)? The conventional wisdom for AGN is that that doesn't help much. 

Now we need to do analysis:
define toy problems, discuss performance for simple adaptive masks
conclusion: with Poisson noise signal reconstruction makes no sense. But pattern recognition works with an adapted mask set.

How do we find the masks:
PCA, ONN

\bnote{Optical neural nets to the rescue.} 
Inspired by recent trends in optical neural networks, we propose a single-pixel vision system for low-light applications. 
By capturing image features directly we avoid amplifying noise

\bnote{How to design these masks.} 

Discussion:
end to end computational imaging with adaptive asks works under Poisson noise.

This provides an additional motivation for proposed optical ANNs or ANNs with optical layers. Such an architecture allows me to choose where in the design I want to add the Poisson noise.

Possibly: Quantum mechanics interpretation.
\fi

==> hardware_pca_onn/sections/1_intro/1_intro_2024_09_29.tex <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

\IEEEPARstart{W}{}hile we possess the capability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely mimics the optics of the human eye to create human-interpretable imaging where the lens projects an image that is then post-processed to extract patterns.
More generalized vision systems can perform many alternative measurements that are potentially more perceptually meaningful than merely producing images. Designing such a system requires co-designing hardware and digital processing with the correct noise model.
To explore the design, we employ a single-pixel camera as a toy model for joint vision system optimization. 

The single pixel camera uses the concept of optical coding, or multiplexing, which involves projecting an image onto a mask and collecting the transmitted light with a large sensor pixel.
% We employ a single-pixel camera as a test bed for hardware optimization, which exemplifies such a system, relying on masks to conduct optically-coded measurements.
% Optical coding, or multiplexing, is a popular technology that projects an image onto a mask and collects the light transmitted through it using a large sensor pixel. 
The system can potentially achieve an enhanced signal-to-noise ratio (SNR) and greater light throughput by coding compared to point-by-point measurements \cite{mitra2014can}.
In this context, a measurement vector $\B{y}$ is formed from a set of measured photon counts, with the corresponding masks vectorized as the rows of the sensing matrix $\B{M}$.
Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 

Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$.
The recovery quality of $\B{x}$, however, also depends on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}.
Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. %The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 

% \subsection*{Transitioning from Gaussian to Photon Noise Models}
Code design is often performed under the assumption of signal-independent Additive Gaussian Noise (AGN) which arises from imperfect sensors.
With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel.
This reduction is significant enough that non-additive photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise follows a Super Poissonian distribution~\cite{mandel1959fluctuations}. For passive cameras operated with incoherent ambient light the noise can usually be approximated as Poissonian.

% \subsection*{Inapplicability of Gaussian Noise for Poisson Mask Optimization}
The transition from AGN to more realistic photon noise  fundamentally alters the designs of vision systems.
%Linear optics are only truly linear in the limit of infinite photons, where quantum noise vanishes.
%The intensity dependence of photon noise renders the camera a nonlinear system, necessitating nonlinear optimization methods. 
%Consequently, the linear approximation frequently used for AGN is not applicable at finite light levels.
%While this issue impacts all camera optics, it has been extensively studied in the context of single-pixel and compressed sensing cameras that rely on coding techniques. 
For instance, although single-pixel cameras with random masks provide performance advantages under AGN, but do not offer improvements over a simple sequential scan when dealing with  Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Furthermore, the optimal coding designs under AGN conditions fail to deliver optimal performance under photon noise. 

In response to this challenge, Mitra et al. \cite{mitra2014can} develop a data-driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can} by designing measurements specifically targeting sparsity or compressibility in the data. 
%An important conclusion from their work is that if the signal exhibits sparsity and thereby compressibility, signal optimized coding can improve recovery performance under signal-dependent noise and the amount of improvement is directly related to the comprehensibility of the measured data. 

However, image recovery is typically not the ultimate goal for modern vision systems.
Since vision tasks, such as classification, operate in embeddings created from images, their data should be inherently more compressible than their upstream imaging tasks allowing for more effective measurement designs. 
%Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.
To show this, our study implements a simple end-to-end vision system that can be optimized  under different noise assumptions. 
We illustrate why AGN is not suitable for optimizing coding under \Xpolish{Poisson}{photon} noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }photon noise is present.


Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively for \YLnote{various downstream tasks.} \Xhide{\YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}}
\item {
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\item {
% \textbf{We train the model under the physically accurate signal-dependent photon noise, as opposed to its approximated version of Poisson noise, to enhance the robustness of our model.}
% We extend Poisson noise to an alternative approximation that places greater emphasis on signal-dependency property, using the reparameterization trick to effectively trace the gradient and train the model to be near optimal when tested under Poisson noise.
We extend Poisson noise to an alternative approximation that prioritizes the signal-dependency property, using the reparameterization trick to effectively trace the gradient and train the model to achieve near-optimal performance when evaluated under Poisson noise conditions.
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

==> hardware_pca_onn/sections/2_related/2_related.tex <==
% \bnote{Don't use the paper start unless it is the large first letter unless it the paper start.... }Multiplexing \bnote{multiplexing has not been mentioned yet. stick with either coding or multiplexing.} %is a method that 

\bnote{Few projects optimize masks for Poisson noise}
\bnote{list how they find the masks for Poisson}


In single-pixel imaging, coding allows the capture of a two-dimensional image with a single-pixel sensor. \bnote{\checkednote{ not constrained to single independent noise just probed for that case.}} Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal} in systems with only additive gaussian noise.
\Xhide{ \bnote{Combine these two sentences?} However, under Poisson noise a trivial raster scan, where one pixel of the mask opens at a time provides the best performance even though it transmits only a small fraction of the light \cite{wuttig2005optimal, harwit1979hadamard, cossairt2012does}.} \checkednote{Previous studies have shown that there is an upper limit to the performance gain of Hadamard multiplexing when Poisson noise is present.} However, incorporating task-specific priors can be beneficial for reconstructions \cite{cossairt2012does, harwit1979hadamard}. \ynote{do these papers really show this? That seems like it is our contribution} \Xhide{\bnote{We are citing mostly just the cossairt2012 paper for all these claims, can we add more citations to the different claims?}. \ynote{Cossairt takes these results from the hadamard transform optics book. We should cite that.}}

% but it is still unclear how to surpass this limit on photon counting systems where Poisson noise is predominant. 



Priors are usually used to enhance the image quality \cite{cossairt2012does, nayer2009prior, Levin2007prior} but the extent of this improvement depends on prior types and masks\Xhide{\ynote{what is imaging coding??}}\cite{cossairt2012does}. Compressed sensing, which utilizes sparsity priors, is a proposed method for improving the reconstruction performance \Xhide{of photon counting systems~\rnote{Is this true?? This seems to be contradicting beccas paper.}}\cite{duarte2008CS}. Nevertheless, the performance attainable under Poisson noise is bounded, significantly lower than under additive gaussina noise, and is heavily influenced by the number of measurements taken and thereby the resolution of the reconstructed image\cite{willet2009CSPoisson}. As such, compressed sensing is a far more challenging task when the measured data are Poisson distributed \cite{willet2009CSPoisson}. Coding strategies and theoretical frameworks developed for additive Gaussian noise are not necessarily usable under Poisson noise.

\Xpolish{While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}. \Xhide{\ynote}{In many cases the most meaningful way to quantify the quality of the collected imaging data is to apply it to a downstream vision task.} Therefore, we explore 
% alternative metrics that better capture the perceptual features and 
optimal masks for feature specific imaging \cite{neifeld2003dual}. \Xhide{\rnote{FSI doesn't work under Poisson \cite{neifeld2003dual}}}
One inspiring solution is the task-specific imaging via Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training}. Wang et al. \cite{nature2022ONN}\Xhide{\ynote{citation}} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. }
{While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation \cite{davenport2007smashed}. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}. Therefore, we explore 
% alternative metrics that better capture the perceptual features and 
optimal masks for feature specific imaging \cite{neifeld2003dual}. The principal component analysis (PCA) is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. Another inspiring solution is the task-specific imaging via end-to-end optimization such as Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training}. 
\YLnote{This idea was usually implemented without considering Poisson noise \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training} or training under Poisson noise \cite{tseng2021differentiable, diamond2021dirty, rego2022deep}. Rego et. al froze the sensing matrix as a pinhole without optimizing it.}
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. }
% Wang et al. reported a successful implementation of a neural networks model on optical device for handwritten numbers classification with limited photon budget \cite{nature2022ONN}, which gives a inspiring example in searching task-specific optimal coding scheme for the CI with the assistance of AI .
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked from a set of hyper-parameter combinations \cite{nature2022ONN}. } 


% \rnote{Our contribution}





% Raginsky et al proved the 

%see
%http://vigir.missouri.edu/~gdesouza/Research/Conference_CDs/IEEE_CVPR_2007/data/papers/0194.pdf

==> hardware_pca_onn/sections/2_related/2_related_revised.tex <==
\textbf{Single Pixel Imaging}. In single-pixel imaging, coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal} in systems with only additive gaussian noise.

\textbf{Imaging Priors}. Priors are usually used to enhance the image quality \cite{cossairt2012does, nayer2009prior, Levin2007prior} but the extent of this improvement depends on prior types and masks \cite{cossairt2012does}. 

\textbf{Compressed Sensing}. Compressed sensing, which utilizes sparsity priors, is a proposed method for improving the reconstruction performance \Xhide{of photon counting systems~\rnote{Is this true?? This seems to be contradicting beccas paper.}}\cite{duarte2008CS}. Nevertheless, the performance attainable under Poisson noise is bounded, significantly lower than under additive gaussina noise, and is heavily influenced by the number of measurements taken and thereby the resolution of the reconstructed image\cite{willet2009CSPoisson}. As such, compressed sensing is a far more challenging task when the measured data are Poisson distributed \cite{willet2009CSPoisson}. Coding strategies and theoretical frameworks developed for additive Gaussian noise are not necessarily usable under Poisson noise.

\textbf{Non-reconstruction classification}. While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation \cite{davenport2007smashed}. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}.

% \textbf{Metric for imaging}. \YLnote{MSE is not a good metric}

\textbf{Principal Component Analysis}. The principal component analysis (PCA) aims to extract significant features in another orthogonal space \cite{abdi2010PCA}. It is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}.

\textbf{End-to-End optimization}. This method refers to training hardware and software networks for image processing pipelines \cite{diamond2021dirty, zhang2021deep}. \Xhide{One typical archetecture is Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training, caulfield1989ONN}.} \YLnote{In many previous projects, this idea was usually implemented without considering Poisson noise \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training} or without optimizing masks under Poisson noise \cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN}. Rego et al. froze the sensing matrix as a pinhole without optimizing it \cite{rego2022deep}}
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. 
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked from a set of hyper-parameter combinations \cite{nature2022ONN}. } 

==> hardware_pca_onn/sections/2_related/2_related_revised_2.tex <==

\textbf{Coding under Poisson noise}. In coded imaging, \Xhide{coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. }Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal, mitra2014can} in systems with only AGN, though this conclusion doesn't hold for Poisson noise \cite{mitra2014can}. \Xpolish{However, when Poisson noise is predominant, we should not use any coding \cite{harwit1979hadamard, cossairt2012does}. When the noise is Poisson distributed, coding with sparse priors such as compresses sensing are not recommended \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}.}
{In many recent projects, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance, gibson2020single, liutkus2014imaging, candes2008introduction}\YLnote{\checkednote{need more here}}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson,  willett2011poisson, vanden2019various}.\Xhide{ While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methods explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}.} \YLnote{Wuttig, Ratner, et al. \cite{wuttig2005optimal, ratner2007optimal} introduced Poisson noise-aware optimization techniques for multiplexing matrices, outperforming Hadamard in the presence of moderate signal-dependent noise. However, their analysis neglects data priors, leading to suboptimal matrices for greater Poisson noise \cite{mitra2014can}.} Additionally, attempts at matrix optimization focusing on minimal mutual coherence \cite{mordechay2014matrixRIP} lack a foundation in the Poisson noise model, as highlighted in this study.}



% \textbf{Task Specific Imaging}


\textbf{Feature Specific Imaging}. Feature-specific imaging (FSI) is a type of imaging system \Xpolish{that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it}{where sensing matrix $\B{M}$ incorporates linear features of expected data} \cite{neifeld2003FSI, neifeld2003dual}. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}. This technique can be viewed as a variant of compressed sensing, wherein the sensing matrix is determined based on prior information \cite{neifeld2014optimizing}. Nevertheless, \Xpolish{its performance and implications under Poisson noise conditions remain relatively unexplored in the existing literature, warranting further discussion and investigation}{\YLnote{current state-of-the-art} FSI is explicitly designed for AGN rather than Poisson noise\cite{neifeld2014optimizing}}. \YLnote{FSI can be regarded as a technique that leverages data driven priors, and Mitra et al. have asserted that employing data driven priors can enhance image recovery under Poisson noise \cite{mitra2014can}. Therefore, in our work, we underscore the promising prospects of extending feature-specific concepts to a broad spectrum of vision tasks under Poisson noise.}


\textbf{End-to-end optimization}. This method \Xpolish{refers to training hardware and software networks for image processing pipelines}{jointly optimizes camera design and digital signal processing to achieve optimal overall performance} \cite{diamond2021dirty, zhang2021deep, jacome2023middle}. \YLnote{In many previous projects, this idea was usually implemented \Xpolish{without considering Poisson noise}{without considering Poisson noise in cost functions} \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training, jacome2023middle, gibson2020single} or without optimizing masks \Xpolish{under Poisson noise during training}{with gradient incorporating Poisson distribution} \cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN, gibson2020single, xu2020compressed}. Rego et. al froze the sensing matrix as a pinhole without optimizing it \cite{rego2022deep}}.
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes\Xhide{ in CI}. 
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked among a set of \Xpolish{hyper-parameter combinations}{different initialization seeds} \cite{nature2022ONN}. %supplementary note 13
Xu et al. \cite{xu2020compressed} examined the robustness of the proposed neural networks model to Poisson noise; however, the training process does not explicitly incorporate the gradients affected by Poisson noise.} Our contribution is developing a noise-\Xpolish{included}{aware} training approach within a neural network model to find the globally optimal masks under Poisson noise.

% \textcolor{blue}{Add section on feature specific imaging}



\iffalse

\YLnote{For the feature specific imaging, here are some paper to cite}

\YLnote{yizhou notes start}
\textbf{Mark A. Neifeld and Premchandra Shankar, "Feature-specific imaging," Appl. Opt. 42, 3379-3389 (2003)} Feature-specific imaging is a type of imaging system that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features.  Poisson noise when the mean and variance of the photon count are equal. The paper shows that feature-specific imaging does not provide any advantage over conventional imaging in the presence of shot noise, because the shot-noise-limited SNR is inherent in the irradiance collected by the instrument and does not depend on the energy incident on any particular detector. Therefore, we can infer that feature-specific imaging would not work well with Poisson noise either, unless the mean and variance of the photon count are very different. \YLnote{However, that is where we come up with hardware PCA. We can then further reduce the text by citing Neifeld for the PCA part. }

\textbf{Abhijit Mahalanobis and Mark Neifeld, "Optimizing measurements for feature-specific compressive sensing," Appl. Opt. 53, 6108-6118 (2014)} "Although our analysis assumes that the noise is independent of the signal, this is not the case when Poisson noise is present. While a formal treatment of the effects of signal-dependent noise is beyond the scope of the paper, we compare the behavior of optimized masks to the normalized PCA in signal-dependent noise." It also has imcomplete future work "Other types of noise models will also be considered, such as signal-dependent shot noise." It seems it hasn't been studied after this paper. We could say that our contribution is designing a method to extend feature specific imaging in poisson noise model.

\YLnote{Interesting conclusions listed below}  

"FSI is a form of CS in which the measurement kernels are not random, but are based on prior knowledge of the information we are interested in sensing. Working in this FSI framework, we have developed a methodology for designing a set of masks that satisfy the photon constraint and are optimum for making measurements that minimize the reconstruction MSE in the presence of noise. "

"Of course, the primary reason for CS is to make fewer measurements than the number of pixels in the reconstructed image, and to collect the information more efficiently than a conventional image. One might intuitively expect that utilizing more features (or measurements) in the reconstruction process will yield a smaller reconstruction error. We demonstrated, however, that the photon constraint limits the number of masks that can be used at a particular SNR to reduce the reconstruction MSE. In noisy conditions, the MSE initially decreases as the number of measurements is increased, but then increases when measurements that contain more noise than signal information are included." \YLnote{It aligns with Rebecca's work.}

\textbf{W. Van den Broek, B. W. Reed, A. Béché, A. Velazco, J. Verbeeck and C. T. Koch, "Various Compressed Sensing Setups Evaluated Against Shannon Sampling Under Constraint of Constant Illumination," in IEEE Transactions on Computational Imaging, vol. 5, no. 3, pp. 502-514, Sept. 2019, doi: 10.1109/TCI.2019.2894950.}  show that for the investigated sensing matrices and in the absence of read-out noise, i.e. with only Poisson noise present, compressed sensing does not raise the amount of Fisher information in the recordings above that of a Shannon sampled signal.





\YLnote{yizhou notes end}

\ynote{andreas notes start}
Other refrerences:
M. Mordechay and Y. Y. Schechner, "Matrix optimization for poisson compressed sensing," 2014 IEEE Global Conference on Signal and Information Processing (GlobalSIP), Atlanta, GA, USA, 2014, pp. 684-688, doi: 10.1109/GlobalSIP.2014.7032205.
“Considering that the measurements are noisy, it is important to
avoid energy loss, since measurements with low energy have low
signal-to-noise ratio (SNR).”
We prove this assumption wrong in this paper ... \YLnote{ONN reconstruction}

Photon-noise: is a single-pixel camera better than point scanning? A signal-to-noise ratio analysis for Hadamard and Cosine positive modulation, Camille Scotté, Frédéric Galland1 and Hervé Rigneault
Published 7 June 2023 • © 2023 The Author(s). Published by IOP Publishing Ltd
Journal of Physics: Photonics, Volume 5, Number 3 Citation Camille Scotté et al 2023 J. Phys. Photonics 5 035003 DOI 10.1088/2515-7647/acc70b
Looking at SNR for different codes. Mostly confirms prior results. Finds that snr is improved for brightest pixels, but degraded for others. \YLnote{Only $x_i \ge k \bar{x} = \frac{k\sum_{j=1}^N x_j}{N}$ can get improved. $k$ is usually $2, 4, 16$, which means only bright pixels get reconstruction gain. E.g. cosmophotography. For normal images, that usually means the general performance degrades!}

D. Shin, J. H. Shapiro and V. K. Goyal, "Performance Analysis of Low-Flux Least-Squares Single-Pixel Imaging," in IEEE Signal Processing Letters, vol. 23, no. 12, pp. 1756-1760, Dec. 2016, doi: 10.1109/LSP.2016.2617329.
Finds bounds for noise. Probably agrees with paper above.
This is very interesting. AT very low rates the non negativity constraint can improve our estimate for multiplexing so it may become better than poisson. The paper doesn’t prove that it is better. Just says the proof for the general case is not valid and shows an experiment where an improvement is shown. Could we use the same constraint in convex optimization? What does this say about other constrained or regularized optimizations?
\ynote{andreas notes end}


\iffalse
better arrangement
coding under Poisson: mention hadamard book, ollie and becca's paper show that coding under Poiss is not ideal
mask optimization: people optimize the masks under wrong noise model, we proposed a better way for Poiss 

\fi


\YLnote{In summary, we can have a list of literature by their category
\begin{enumerate}
    \item Open more pixels doesn't help under Poisson noise (no compression): \cite{harwit1979hadamard, neifeld2003FSI, cossairt2012does, scotte2022photon_noise}
    \item Regularization doesn't help (usually comes with compression):
    \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}. Their suggestion is to use fewer measurements as more measurements give rise to a greater reconstruction error upper bound. BTW, ONN are can have many measurements with low rank, which doesn't contradict to this conclusion.
    \item Feature specific imaging is designed for gaussian noise especially. It is a good way for feature preserving and reconstruction. No follow-up about the poisson. That is why we start this project.
    \item When doing a classification task, we give some higher compression by labelling. E.g, gender recognition. We only need one mask to tell the gender in the most ideal case. \textbf{It will be good to find some paper directly saying this.} As the data can be highly compressible, we can avoid dense measurements, and thus have lower error bound. Reconstruction is just a linear operation, so it doesn't matter a lot if we use Rebecca's conclusion about the upper bound, even though it is for reconstruction. 
        \begin{itemize}
        \item Think about reconstructing an image about the night sky. After using TV \textbf{re-binning}, we have two colors, black for background, and white for stars. It can be treated as a classification task as well! That is why rebecca proposed some algorithms with TV stuff: to minimize the possible amount of measurements.
    \end{itemize}
    Neifeld uses features learned from training data to do reocnstruction, that is how our idea of directly classification comes from. If we want to apply the ONN for reconstruction, it may be useful to read "RecDNN: deep neural network for image reconstruction from limited view projection data"
\end{enumerate}
}
\fi


\AVnote{\checkednote{Regularization, CS, might help but noise bounds are very unfavorable (cite becca). \\ In most of the papers, people optimize the algorithm. In only very few people try to optimize the masks. No paper where masks are optimize with poisson noise. \\ In this paper we are looking at how to optimize the measurement under poisson noise. \\ We find that optimizing the measurement can have profound improvements to the performance of single pixel vision approaching the perfonance of ideal mutipixel cameras in particular for Poisson noise dominated signals like visible light. }}




==> hardware_pca_onn/sections/3_background/model_implementation_old.tex <==
\Xhide{Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ masks\Xhide{\bnote{We have not introduced the language mask yet.}}, 
  the single-pixel-sensing process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x}
    \end{aligned}
\end{equation}
, where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is the sensing masks\Xhide{or in other words, weighing design (WD) \cite{harwit1979hadamard} \bnote{not sure if language from 1979 is useful. I have not heard of weighing design},} linearly projecting the field of view, and $\B{y} \in \IR^{m \times 1}$ is the corresponding photon counts \cite{willet2009CSPoisson}.}

\Xpolish{
As a typical CI technique, the mathematical foundation of single pixel imaging follows the equation \ref{eqn:NoiselessMeasurement}. However, the different choices of the sensing matrix $\B{M}$ give rise to different coding types (strategies) introduced later. However, $\B{M}$ yields to two constraints when physically implemented. 
}{
As a representative technique in the CI, the mathematical underpinning of single-pixel camera is encapsulated by Eq. \ref{eqn:NoiselessMeasurement}. The diverse selections of the sensing matrix $\B{M}$ lead to distinct coding strategies, as elaborated upon subsequently. \Xhide{Nonetheless, the physical realization of $\B{M}$ introduces two inherent constraints.}
}
\YLnote{Not a good place for this}
\begin{enumerate}
    \item\label{constraint:photonNumber} \textbf{Flux-preserving} \cite{willet2009CSPoisson}\Xhide{\bnote{Y: Should I use the same term as Rebecca?}}. The single-pixel camera model involves the allocation of available photons among masks, as discussed in \cite{neifeld2003dual}. It is important to ensure that the mask basis $\B{M}$ does not produce additional photons through improper entries \cite{neifeld2003dual}. Mathematically, $\sup \sum_{i=1}^m M_{ij} = 1, \forall j \in \{1,2,\dots,N\}$ \cite{neifeld2003dual}.\Xhide{\bnote{Include what an improper entry is!} \bnote{A: this is not something we need to mention here. its obvious that the measurements have to be normalized correctly}}
    \item\label{constraint:negativeEntry} \textbf{Positivity-preserving} \cite{willet2009CSPoisson}. It is not possible to physically implement negative values for the masks $\B{M}$, as demonstrated in \cite{neifeld2003dual, willet2009CSPoisson}. 
\end{enumerate}

\AVnote{the rest of this section can be removed. the figure should stay}
\YLnote{The sensing matrix $\B{M}$ can be generated using either computational or non-computational imaging methods (i.e. Raster scan). The key difference between the two is that computational imaging involves additional steps of optical coding and computational decoding to capture and process the image \cite{cossairt2012does}, while non-computational method, i.e. Raster scan, involves measuring each pixel sequentially \cite{duarte2008CS}. In the case of Raster scan, $\B{M} = \B{I}$, which is an identity matrix. In contrast, computational methods measure a combination of pixels simultaneously and can be further classified based on the type of masks used. For example, Hadamard matrices composed of $\pm 1$ have been shown to be the optimal coding strategy for reconstruction under the AGN \cite{harwit1979hadamard}. A useful feature of computational methods is their compressibility. If the signal is sparse in the subspace of $\B{M}$, it is likely that only a few vectors of $\B{M}$ are needed.}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct measurement scheme (Raster scan)}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational imaging scheme (Basis scan)}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{ Single-Pixel imaging methods. $\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

\YLnote{It is better to intro this at the end of this section or \textbf{move it to methods}}
\Xpolish{
Another problem to be investigated is the noise. To compare measurements, we assume that each measurement is performed using the same amount of light at the camera aperture and over the same total time.
}{
Another critical issue for investigation is noise level. In order to establish meaningful comparisons between measurements, it is assumed that each measurement is conducted under consistent conditions, including uniform light intensity at the camera aperture and an equal duration of exposure.
}

==> hardware_pca_onn/sections/3_background/model_implementation_old_2024_04_11.tex <==
% \YLnote{1. What are sensing matrix 2. their types 3. limitations}
\Xhide{As a representative technique in the CI, the mathematical underpinning of single-pixel camera is encapsulated by Eq. \ref{eqn:NoiselessMeasurement}. The diverse selections of the sensing matrix $\B{M}$ lead to distinct coding strategies, as elaborated upon subsequently. }

\YLnote{\Xpolish{\AVnote{ChatGPT problem}In the realm of the Computational Imaging (CI), the foundational equation for single pixel imaging is encapsulated in Eq. \ref{eqn:NoiselessMeasurement}}{Eq. \ref{eqn:NoiselessMeasurement} is the foundational equation for single pixel imaging}}. \Xpolish{The diverse array of choices for the sensing matrix $\B{M}$ engenders two basic coding strategies, as expounded in Fig \ref{fig:SinglePixelImaging}. However, the process of discerning an optimal $\B{M}$, whether drawn from random matrices or Hadamard matrices, hinges on multifaceted considerations. In the present study, we advocate the notion that the selection of an ideal $\B{M}$ should be contingent upon the requisite prior information pertinent to the tasks at hand. Herein, we delineate various coding types along with their corresponding optimal applications for reference and guidance.}{Based on it, we distinguish different types of $\B{M}$ below for reference and guidance.}

\iffalse
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct measurement strategy (Raster scan)}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational imaging strategy (Basis scan)}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}
\fi
% As a typical CI technique, the mathematical foundation of single pixel imaging follows the equation \ref{eqn:NoiselessMeasurement}. However, the different choices of the sensing matrix $\B{M}$ give rise to different coding types (strategies) introduced later. However, how to select a good $\B{M}$ from random matrices to Hadamard matrices for the Basis scan depends on many factors. In this project, we proposed that the optimal $\B{M}$ should be selected based on the required prior information of tasks we want to complete. The coding types and the most suitable task of each type are listed below for reference.

\subsubsection{Coding Types}

\begin{itemize}
    \item \textbf{Raster scan} entails a pixel-wise scanning approach where photon counts for all pixels are sequentially measured \cite{gibson2020single}. Mathematically, the sensing matrix $\B{M} = \B{I}$, an identity matrix.      
    
    \item \textbf{Impulse imaging} entails an ideal camera that simultaneously captures \Xpolish{complete hyper-spectral data}{all elements in the measurements, $\B{y}$}. A prominent instance is a pixel array. When the field of view $\B{x}$ consists of $N$ pixels, the sensing matrix assumes the form $\B{M} = N\B{I}$ where $\B{I}$ is an identity matrix. Each pixel receives $N$ times the exposure in comparison to the raster scan scenario. This technique sets a benchmark akin to a gold standard, serving as an upper limit for the CI performance and an indicator of the noise level for comparison.
    
    \Xhide{\item \textbf{Non-Selective Codes} \Xpolish{are codes that are not adjusted to the specific sparsity of the dataset. Any general code not generated using the statistics of a representative training set is included in this group. This includes many codes used in practice today, such as Hadmard patterns and Rademacher Random codes. We also include truncated Hadamard patterns that are popular in compressed sensing. A truncated Hadamard code uses a random subset of the full Hadamard basis.
    }{encompass coding schemes that lack adaptation to the inherent sparsity of a given dataset. Codes falling within this category are not crafted based on the statistical attributes of a representative training set. This classification encompasses a range of widely used codes, such as Hadamard patterns and Rademacher Random codes\Xhide{, which do not leverage the specific characteristics of the dataset}. This grouping also extends to truncated Hadamard patterns\Xpolish{, a popular choice in compressed sensing, which employ random subsets of complete Hadamard basis.}{ which employ low frequency components of complete Hadamard basis.}
    }
    }%change to a newer and simpler one
    \item \YLnote{\textbf{Non-Selective Codes} refer to coding schemes that uncorrelated with the inherent \Xpolish{sparsity}{compressibility} or statistical attributes of a specific dataset. Examples include widely used codes like Hadamard patterns and Rademacher Random codes. This category also includes truncated Hadamard patterns that use low-frequency components of the complete Hadamard basis.}

    
    \item \textbf{Selective Codes}
    \Xpolish{In this work we show that for single photon cameras, codes need to be specifically selected to measure sparse representations of the data. To achieve this we employ PCA codes and ONN generated codes. The principal component analysis (PCA) is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. In this project, the most significant components are computed from the training data and implemented as the hardware masks. Measured photon counts $\B{y}$ are then be feed to a classifier for model optimization. The optical neural networks (ONN) method is like a fully-connected neural networks model but its first layer is used to simulate the sensing matrix $\B{M}$. By properly applying the physical constraints on the first layer, it is possible for this model to find optimal sensing matrix for a given task.}
    {\Xpolish{.In this study, we elucidate the necessity for the tailored selection of codes in}{encompass coding schemes selectively \YLnote{\Xpolish{incorporating the context of single pixel cameras}{learn the significant features from training data}}} to effectively capture sparse data representations. \Xpolish{To address this, we harness both PCA codes and ONN-generated codes. Principal Component Analysis (PCA) serves as a classical technique for analyzing and classifying multispectral data correspondences \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. Specifically, we compute the most significant components from training data and implement them as hardware masks within this project. The recorded photon counts, $\B{y}$, are subsequently fed into a classifier to optimize the model. The Optical Neural Networks (ONN) approach mirrors a fully-connected neural network model, yet with its first hidden layer simulating the sensing matrix $\B{M}$. By adeptly applying physical constraints to this foundational layer, the model becomes capable of determining the optimal sensing matrix for a designated task.}{When under AGN, FSI finds data specific codes through Principal Component Analysis (PCA).}
    }
    
\end{itemize}

\subsubsection{Vision Tasks}
% \paragraph{Null Prior Reconstruction/No Compression}
% \paragraph{Imaging: Weak Prior/Some compression}
% \paragraph{Classification: Strong Prior/Strong compression}
\iffalse
\begin{itemize}
    \item Classic imaging: null-prior/no compression. In this task, the rank of $\B{M}$ is required to be $N$, the number of pixels in the FOV. Therefore, there is no compression when conduct measurements. This case is universal and doesn't require any prior knowledge of the FOV. It can be found in some scenarios such as raster scan. When there is no noise, we can also use full rank Hadamard to reconstruct the FOV. The coding types commonly seen in this kind of tasks are raster scan and non-selective codes.
    \item Image Processing and the Computational Imaging: weak-prior/some compression. This idea comes from some prior knowledge such as signals are sparse in some linear space and noise is concentrated in high frequency domain. One example is the JPEG format of pictures. If we only measure the FOV with low frequency components of the Hadamard matrices, we are working on this task. This type can be found in scenarios such as compressed sensing and image compression. The coding type commonly seen in this kind of tasks is non-selective codes.
    \item Computer vision: strong-prior/much compression. Usually we switch to downstream computer vision tasks such as classification after reconstruct the FOV. However, it is possible to directly capture the principal features by $\B{M}$ if some of its components are similar to the FOV. In this kind of tasks, only a few measurements are needed if we have a strong prior from training data. The coding type involved in this kind of tasks is selective codes.
\end{itemize}
\fi

\begin{itemize}
    \item Signal Reconstruction (Null-prior/No Compression):
    In tasks involving classic imaging, a null-prior is assumed, and there is no compression during measurements. The rank of the measurement matrix $\B{M}$ is required to be equal to $N$, the number of pixels in the \Xpolish{FOV}{$\B{x}$}\Xpolish{. This scenario, such as in raster scan applications, is universal and does not necessitate prior knowledge of the FOV. Full-rank Hadamard matrices can be employed for reconstruction in noise-free situations. Common coding types for this task include raster scan and non-selective codes.}{ and no prior or bias should be introduced through $\B{M}$.}
    \Xhide{
    \item Image Reconstruction and Computational Imaging (Weak-prior/Some Compression):
    In this kind of tasks, a weak-prior assumption is made\Xhide{, allowing for some compression during measurements}. This idea is based on prior knowledge, such as signals being sparse in some linear space, with noise concentrated in the high-frequency domain. \Xpolish{An example is the JPEG format. If only the low-frequency components of Hadamard matrices are measured for reconstructing the FOV, this task is engaged. Non-selective codes are typically used for this purpose.}{One example in this category is compressed sensing.}    
    }%hide and update to newer one below    
    \YLnote{\item Computational Imaging (Weak-prior/Some Compression): In this kind of tasks, a weak-prior assumption is made. This idea is based on prior knowledge, such as signals being sparse in some linear space, with noise concentrated in the high-frequency domain. One example in this category is compressed sensing.
    }\AVnote{\checkednote{We are not doing any imge reconstruction any more Jan 18, 2024 10:40 AM}}
    \item Classification (Strong-prior/Much Compression):
    \Xpolish{Tasks related to computer vision}{Many computer vision tasks} involve a strong prior, enabling substantial compression during measurements. \YLnote{\Xpolish{After reconstructing the \Xpolish{FOV}{$\B{x}$}, the process often transitions to downstream computer vision tasks like classification. Alternatively, direct}{Directly}} capture of principal features by $\B{M}$ is possible if some of its components resemble the \Xpolish{FOV}{$\B{x}$}. In these tasks, a few measurements are often sufficient with a strong prior derived from training data. \Xpolish{Selective codes are commonly employed in this context.}{Our focus is to optimize codes in this scenario.}
\end{itemize}

==> hardware_pca_onn/sections/4_methods/constraint_implement.tex <==
\subsection{Constraints Implementation}

\Xpolish{This section introduces our methods for the optical implementations for the model. To construct a valid model, the Flux-preserving and Positivity-preserving constraints has been satisfied by the following techniques.}
{In this section, we outline our methods for implementing the model optically. In order to ensure that our model is valid, we have implemented techniques that satisfy both the Flux-preserving and Positivity-preserving constraints. By using these techniques, we can ensure that the model accurately represents the underlying physical processes and produces results that are both reliable and interpretable.}

\subsubsection{Photon Distribution Factor} \label{sssection:PDF}
\Xhide{\bnote{A: This section shouldn't be here}}

\Xpolish{The optimization of $\B{M}$ can be challenging, as it is subject to constraint \ref{constraint:photonNumber}.\Xhide{ Specifically, $\B{M}$ must belong to a subset $S$ of $\IR^{m \times N}$, which can vary depending on the specific case \bnote{<- not sure why this sentence is here}. To address this issue \bnote{the issue of belonging to a subset?}, } Here, we propose using a scale factor as a solution. This allows us to select any values for $\B{M}$ without being limited by the constraint \ref{constraint:photonNumber}\Xhide{\bnote{It would be nice to name the constraints}}. The Photon Distribution Factor, $\lambda$, is thus introduced to ensure compliance with constraint \ref{constraint:photonNumber}. As a scale factor, it is calculated as \Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m v_k}},\Xhide{ \bnote{this should be in an equation line}} where $\flux$ represents the number of photons per second projected onto the DMD, $\totexposure$ is the total exposure time for all masks, $N$ represents the number of pixels, and $v_k$ represents the greatest value of the $k_\text{th}$ mask. The maximum value $v_k$ is selected as its corresponding pixel is open for longer than any other one in the $k_\text{th}$ mask, and the exposure time of this mask depends solely on $v_k$. Furthermore, the total exposure time $\totexposure$ is proportional to $\sum_{k=1}^m v_k$ and the total number of photons from the field of view is $\totexposure \sum_{i=1}^N \frac{\flux}{N} x_i$.  }
{Optimizing $\B{M}$ subject to constraint \ref{constraint:photonNumber} can be challenging. To overcome this limitation, we propose the use of a scale factor, known as the Photon Distribution Factor $\lambda$, which allows us to select any values for $\B{M}$ without violating constraint \ref{constraint:photonNumber}. The Photon Distribution Factor is calculated as \Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m v_k}}, where $\flux$ is the number of photons per second projected onto the DMD, $\totexposure$ is the total exposure time for all masks, $N$ is the number of pixels, and $v_k$ is the greatest value of the $k_\text{th}$ mask. The maximum value $v_k$ is chosen as its corresponding pixel is open for longer than any other pixel in the $k_\text{th}$ mask, and the exposure time of this mask depends solely on $v_k$. Moreover, the total exposure time $\totexposure$ is proportional to $\sum_{k=1}^m v_k$, while the total number of photons from the field of view is $\totexposure \sum_{i=1}^N \frac{\flux}{N} x_i$.}

\Xhide{\rnote{Maybe in appendix} \bnote{ Could just state the first and last lines of the math and move the proof to the appendix but still state this ensures constraint one is true}
% Suppose we use an arbitrary matrix $\{\B{a}_1, \dots, \B{a}_m \} \in \IR^{N \times m}$ for measurement, the total number of photons detected is
When an arbitrary measurement matrix, $\{\B{a}_1, \dots, \B{a}_m \} \in \IR^{N \times m}$, is used, the total number of detected photons can be expressed as $\sum_{i=1}^m \lambda \B{a}_i^\top \B{x}$ and the following inequality always holds:
\begin{equation}
\begin{aligned}
    \sum_{i=1}^m \lambda \B{a}_i^\top \B{x} &\le \sum_{i=1}^m \lambda \sum_{j=1}^N v_i x_j\\
    &= \sum_{i=1}^m \sum_{j=1}^N \frac{\flux \totexposure}{N \sum_{k=1}^m v_k} v_i x_j \\
    &= \frac{\flux \totexposure}{N} \sum_{j=1}^N x_j  \frac{\sum_{i=1}^m v_i}{\sum_{k=1}^m v_k} \\
    &= \totexposure \sum_{j=1}^N \frac{\flux}{N} x_j
\end{aligned}.
\end{equation}
% Therefore, by the Photon Distribution Factor, the constraint \ref{constraint:photonNumber} is never violated.
}

\Xpolish{By utilizing the Photon Distribution Factor, constraint \ref{constraint:photonNumber} is guaranteed to be never violated. Then we can re-formulate model in Equation \ref{eqn:NoiselessMeasurement} as the following equation
 \begin{equation} \label{eqn:NoisyMeasurement}
    \begin{aligned}
        \tilde{\B{y}} &=  \frac{1}{\lambda}f_r(\lambda \B{ M x})
    \end{aligned}
\end{equation}
, where $f_r$ generates random numbers with expectation $\lambda \B{ M x}$ to simulate the noise and gives rise to the measurement with noise \bnote{Be consistent with language throughout the text. "noisy-version-measurement" is probably not the best name} $\tilde{\B{y}}$.}
{By utilizing the Photon Distribution Factor, we can guarantee that constraint \ref{constraint:photonNumber} is never violated. With this in mind, we can re-formulate the model in Equation \ref{eqn:NoiselessMeasurement} into the following equation,
\Xequa{\tilde{\B{y}} &=  \frac{1}{\lambda}f_r(\lambda \B{ M x})}.
Here, $f_r$ generates random numbers with an expected value of $\lambda \B{ M x}$ to simulate noise and produce a measurement with noise, denoted as $\tilde{\B{y}}$.}

\subsubsection{Dual-Rail Technique for Negative Entries}\label{sssection:DualBranch}
\Xpolish{\Xhide{\ynote{this could be part of a methods section later on or go to the supplement. Shouldn't be here.}\bnote{Consistent language "Rail" or "Branch" or "Path"} }
The dual-rail technique is introduced for constraint \ref{constraint:negativeEntry} \cite{neifeld2003dual}. In it\Xhide{ \bnote{ might be better to call it a "technique"}}, one measurement needs two complementary branches where one measures with all positive entries, $\B{M}^+$, and the other measures with all negative entries, $\B{M}^-$ \cite{neifeld2003dual}. }
{To satisfy constraint \ref{constraint:negativeEntry}, the dual-rail technique \cite{neifeld2003dual} employs two complementary measurement branches: one measures with all positive entries, denoted as $\B{M}^+$, while the other measures with all negative entries, denoted as $\B{M}^-$. By doing so, the dual-rail technique effectively converts the constraint on negative entries to a constraint on the difference between the measurements made by the two branches.}

\begin{figure}[h]
    \centering
    % \includesvg[width=0.9\linewidth]{\homedir/figures/Methods/Dual_rail.svg}
    \includegraphics[width=0.9\linewidth]{\homedir/figures/Methods/Dual_rail.pdf}
    \caption{Dual-Rail technique}
    \label{fig:Dual-Rail Technique}
\end{figure}


\Xpolish{\bnote{Many of these equations should be on their own line for readability and to reference them later. We have 11 pages so we can do this easily.}
To create the two branches, the mask $\B{M}$ should be split into $\B{M}^+ = \max(\B{M}, 0)$ and $\B{M}^- = \max(-\B{M}, 0)$. The superscripts of the parameters indicate the branches they belong to. Intuitively, we have $\lambda \tilde{\B{y}} = \lambda \tilde{\B{y}}^+ - \lambda \tilde{\B{y}}^-$ where $\tilde{\B{y}}^+$ and $\tilde{\B{y}}^-$ are photon counts with noise measured by $\B{M}^+$ and $\B{M}^-$ respectively. The two-rail trick also changes the expression of the  Photon Distribution Factor. In the case that each branch has a PMT, 
\Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m |v_k|}}
where $|\cdot|$ takes the absolute value. In the case of using only one PMT, it is worth noting that the Photon Distribution Factor changes to 
\Xequa{\lambda = \frac{\flux \totexposure}{N (\sum_{k=1}^m v_k^+ + \sum_{k=1}^m v_k^-)}}
as one PMT measures with $\B{M}_k^+$ and $\B{M}_k^-$ in turn to accomplish measuring $\B{M}_{k}$. \iffalse as there are approximately two times of measurements. \fi \rnote{figure}All the parameters in this updated Photon Distribution Factor are of the same meaning as in section \ref{sssection:PDF}.}{To implement the two branches, we split the mask $\B{M}$ into two components: $\B{M}^+ = \max(\B{M}, 0)$ and $\B{M}^- = \max(-\B{M}, 0)$, with the superscripts indicating the respective branches. This enables us to express $\lambda \tilde{\B{y}}$ as the difference between the photon counts with noise measured by $\B{M}^+$ and $\B{M}^-$, denoted $\lambda \tilde{\B{y}}^+$ and $\lambda \tilde{\B{y}}^-$, respectively. Notably, the two-rail approach also modifies the expression for the Photon Distribution Factor. In the case that each branch has a PMT, 
\Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m |v_k|}}, 
where $|\cdot|$ takes the absolute value. In the case of using only one PMT, it is worth noting that the Photon Distribution Factor changes to 
\Xequa{\lambda = \frac{\flux \totexposure}{N (\sum_{k=1}^m v_k^+ + \sum_{k=1}^m v_k^-)}},
since one PMT measures with both $\B{M}_k^+$ and $\B{M}_k^-$ sequentially to obtain the measurement result for $\B{M}_{k}$. All the parameters in this updated Photon Distribution Factor are of the same meaning as in section \ref{sssection:PDF}, and $v_k^+$ and $v_k^-$ stand for the maximum values of $\B{M}^+$ and $\B{M}^-$ respectively. 
} 

==> hardware_pca_onn/sections/4_methods/model_validation_2024_04_11.tex <==
\subsection{Model Validation}

% In this section, we start with a theoretical investigation on the reconstruction performances of null-prior strategies. Then the reconstruction and classification performances of all strategies and fairly compared by simulations and experiments. 

\Xhide{
\Xpolish{To validate the ONN model is correct, we begin with a theoretical derivation of the null-prior reconstruction. Afterwards, we test our ONN model by reconstructing random signals under two noise models and see what the optimized masks converge to at last.}
{
\Xpolish{To affirm the correctness of the ONN model, we initiate the validation process with a theoretical derivation of the null-prior reconstruction. Subsequently, we conduct empirical testing of the ONN model by reconstructing random signals under two distinct noise models. This experimental approach allows us to observe the convergence of optimized masks, providing empirical evidence for the validity and efficacy of the ONN model.}{To validate the proposed ONN model, we apply it to a signal reconstruction task with a \YLnote{\Xpolish{mathematically provable foundation}{mathematical proof}}. In the subsequent section, we undertake a theoretical derivation of error propagation resulting from both AGN and Poisson noise. \Xpolish{Notably, this section doesn't find the optimal masks $\B{M}$, but focuses on the comparison under Poisson noise between the identity matrix and the Hadamard matrix which has been proved to surpass the former under AGN.}{While optimal masks $\B{M}$ are not determined in this context, we concentrate on disproving the superiority which has been previously proven under AGN of the Hadamard matrix over the identity matrix under Poisson noise.}}
}
}%Hide
\YLnote{
\Xpolish{To validate the proposed ONN model, we apply it to a non-compressible signal reconstruction task. We focus on comparing Hadamard and Raster coding, and proving which is the better under different noise conditions. In the subsequent sections, we undertake a theoretical derivation of error propagation resulting from both AGN and Poisson noise, and test if our ONN model can justify the conclusion.
}{
To validate the proposed ONN model, we apply it to non-compressible signal reconstruction tasks where the correct solution is known. We compare Hadamard and Raster coding under both AGN and Poisson noise conditions. In subsequent sections, we derive the theoretical error propagation caused by both AGN and Poisson noise, assessing the ONN model's ability to substantiate our findings.
}
}
\AVnote{\checkednote{This section still doesn't clearly state what we do and why. Cand te just say we train masks to reconstruct non -compressible signals? Jan 18, 2024 10:58 AM}}
\AVnote{\checkednote{Need to be more specific what we show. I think we select two patterns, raster and hadamart, and prove which is better for non-compressible data. Then we see if the ONN finds similar masks. Jan 18, 2024 11:08 AM}}

\subsubsection{Theoretical Treatment for Null-Prior Reconstruction }

% \textcolor{blue}{This section could be taken out.}
\YLnote{In our study, the FOV comprises albedo and illumination. To streamline the discussion and formulas and avoid unnecessary complexity, we did not previously mention illumination. The illumination level for each pixel in a measurement, denoted as $\lambda$, influences noise magnitude. We reformulate the model as $\lambda \B{y} = \lambda \B{Mx}$, where $\B{x} \in [0,1]^{N \times 1}$ now represents the albedo which is our objective for reconstruction.}
Define $\B{I}$ as the identity matrix and $\totphoton = \rho \tau$ as the total number of photons from the source. Given the noisy photon counts $\tilde{\B{y}}$ and the full-rank mask basis $\B{M}$, we can reconstruct the field of view $\tilde{\B{x}} = \B{M}^{-1} \tilde{\B{y}}$.
Based on Parseval's identity, the covariance matrix of a vector $\B{b}$ is $\B{\Sigma}_{\B{b}\B{b}} = c^2 \sigma^2 \B{I}$ if $\B{b} = \B{W a}$ where $\B{\Sigma}_{\B{a}\B{a}} = \sigma^2 \B{I}$ and 
% $\B{W}$ is $c$ times an orthonormal matrix
$\B{W} \B{W}^\top = c^2 \B{I}$. 
For RS, we have $\lambda = \frac{\totphoton}{N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{I}\B{x}, \sigma^2 \B{I})$. Thus, the reconstructed \Xpolish{field of view}{$\B{x}$} is 
\begin{equation}
    \label{eqn:RS_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{\sigma^2 N^4}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{H}\B{x}, 2\sigma^2 \B{I})$ where the factor of $2$ arises from the dual rail trick mentioned in section \Xpolish{\ref{sssection:DualBranch}}{\ref{ssection:constraints}}. For $\B{H}^{-1}$, $c = \sqrt{\frac{1}{N}}$. The reconstructed field of view is 
\begin{equation}
    \label{eqn:HB_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{8 \sigma^2 N^3}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
% Therefore, when considering the AWGN model, using the Hadamard matrix can improve the SNR of the reconstructed field of view when $N$ is large.
Therefore, using the Hadamard matrix in the AWGN model can improve the signal-to-noise ratio (SNR) of the reconstructed field of view when the number of elements, $N$, is large. 

When the noise is Poisson distributed, the covariance matrix of the noisy photon counts depends on the choice of $\B{M}$. Suppose $\sigma_j$ is the standard deviation of $\lambda \tilde{y}_j$, the $j_\text{th}$ measured noisy photon counts. For the RS, we have $\sigma_j^2 = \lambda x_j$ and $\lambda = \frac{\totphoton}{N^2}$. The covariance matrix of the reconstructed field of view is thus 
\begin{equation}
    \label{eqn:RS_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{N^2}{\totphoton}\diag\{x_1, x_2, \cdots, x_N\}
    \end{aligned}.
\end{equation}
% For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$ by the Skellam Distribution in section \ref{sssection:DualBranch}. Since Hadamard matrices only includes $\pm 1$ entries, we further have $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$ and the covariance matrix  

In the case of the HB, we can express the rate parameter $\lambda$ as $\lambda = \frac{\totphoton}{2N^2}$, as demonstrated in section \ref{ssection:constraints} using the Skellam distribution. Additionally, we can express the variance of each element in the sum as $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$. As Hadamard matrices only contain entries of $\pm 1$, this reduces to $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$. Using this information, we can construct the covariance matrix
\begin{equation}
    \label{eqn:HB_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{2N \sum_{k=1}^N x_k}{\totphoton}  \B{I}
    \end{aligned}.
\end{equation}
% Therefore, the mean squared error (MSE) of HB is 2 times that of RS under Poisson noise. This factor of 2 arises from the dual branch trick. In other words, HB can never exceed RS in reconstruction error even when measuring with 2 PMTs simultaneously.
The results of our analysis reveal that the mean squared error (MSE) of the HB method is twice that of the RS method when the noise is Poisson distributed. \Xpolish{This difference is attributed to the dual branch trick utilized in the HB method. Despite the use of two PMTs in the HB method, it is unable to surpass the reconstruction error of the RS method. These findings demonstrate the limitations of the HB method in comparison to the RS method under Poisson noise conditions.}{\Xpolish{In other words, the}{The} HB outperforms the RS when the observed measurements $\B{y}$ are Gaussian distributed. This superiority doesn't hold under Poisson noise.} Given that many algorithms rely on AGN model, their conclusions may not hold if the optimal masks differ under Poisson noise. 

\Xhide{
\begin{figure}[ht]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Reconstruction under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_reconstruction.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_reconstruction.pdf}
        \label{fig:gaussian_reconstruction}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering        
        \caption{Reconstruction under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_reconstruction.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_reconstruction.pdf}
        \label{fig:poisson_reconstruction}
    \end{subfigure}
    \caption{Reconstruction errors on simulated data. RS: Raster basis. HB: Hadamard basis. II: Impulse imaging. BR: Binary random basis. (\subref{fig:gaussian_reconstruction}) RS is always worse than HB for all noise levels under Gaussian noise. (\subref{fig:gaussian_reconstruction}) HB is no better than RS under Poisson noise.
    }
    \label{fig:simulated_reconstruction}
\end{figure}
}





\Xhide{The first question to be answered is if the ONN can find the (approximately) optimal masks. To get the benchmark, we compared the reconstruction performance w.r.t the mean squared error between the raw and reconstructed images $\|\noisy{\B{x}} - \B{x}\|_2^2$ where $\noisy{\B{x}} = \B{M}^{-1} \noisy{\B{y}}$. Fig. \ref{fig:simulated_reconstruction} shows that Hadamard Basis is less preferred under Poisson noise but more optimal under the AGN compared with the Raster Basis.}

\Xhide{
\YLnote{\checkednote{This para needs polish}}
\Xpolish{We already saw the ONN had the best classification performance on the simulated data and its masks are optimal, it is still unclear if the ONN masks under the AGN and Poisson noise are similar. Since many algorithms are based on the AGN model, the conclusions drawn from them may be problematic if the optimal masks are different under the Poisson noise model. One simple approach is to let the ONN optimize the masks for a reconstruction task under different noise models. Therefore, we built a new ONN model which has $m = N$ masks. Its scanner took the raw images vectors $\B{x}$, and output $N$-element measured photon count vectors under some noise model, $\noisy{\B{y}}$. Its classifier is a single-layer network taking $N$-element vectors $\noisy{\B{y}}$ and outputting $N$-element vectors $\noisy{\B{x}}$. The objective is to minimize the MSE between the input images and the output vectors, or $\|\noisy{\B{x}} - \B{x}\|_2^2$. In noiseless cases, the classifier is equivalent to $\B{M}^{-1}$ if $\B{M}$ is the masks in the scanner.}
{ 
The primary question to address is whether the ONN has the ability to identify \Xpolish{noise specific optimized masks}{the derivation above}. We established a benchmark by comparing the reconstruction performance in terms of the MSE between the original and reconstructed images, denoted by $\|\noisy{\B{x}} - \B{x}\|_2^2$, where $\noisy{\B{x}} = \B{M}^{-1} \noisy{\B{y}}$. The reconstructed images were obtained using the Hadamard basis and Raster basis under Poisson noise and AGN models respectively. The outcomes, depicted in Fig. \ref{fig:simulated_reconstruction} where the x-axis is the log-scaled MSE of impulse imaging with different exposure times, indicate that the Hadamard basis is less effective in the presence of Poisson noise, while it is more effective under AGN model when compared to the Raster basis. Given that many algorithms rely on AGN model, their conclusions may not hold if the optimal masks differ under Poisson noise. \ynote{\checkednote{the following text does not belong in the results section}}\Xhide{ To address this, we propose a simple approach of optimizing the ONN masks for a reconstruction task under different noise models. To achieve this, we developed a new ONN model with $m = N$ masks. The scanner takes raw image vectors $\B{x}$ and outputs $N$-element measured photon count vectors under a chosen noise model, $\noisy{\B{y}}$. The classifier is a single-layer network that takes $\noisy{\B{y}}$ as input and outputs $\noisy{\B{x}}$, also an $N$-element vector. The objective is to minimize the MSE between the input images and the output vectors, $\|\noisy{\B{x}} - \B{x}\|_2^2$. In noiseless cases, the classifier is equivalent to $\B{M}^{-1}$, where $\B{M}$ is the masks used in the scanner.}
}
}

\subsubsection{ONN Non-compressible Signal Reconstruction}  
\TSnote{confusing}

\Xpolish{Before the ONN model is employed, the primary question to address is whether the ONN has the ability to identify \Xpolish{noise specific optimized masks}{the derivation above}. To \Xpolish{make this reconstruction task less specific and more general}{generate non-compressible data}, the input data vectors $\B{x}$ were reshaped from 8 by 8 random patterns. In different epochs of training, the $\B{x}$ was re-generated randomly. This simulation is conducted with a great noise level as the total number of photons is about $1 \times 10^3$. The masks $\B{M}$ were initialized with an $N \times N$ identical matrix and were optimized until this model reported constant losses.}
{Before the employment of the ONN model, the primary question to address is whether the ONN has the ability to identify \Xpolish{noise specific optimized masks}{the derivation above}. 
Given the universality of reconstruction algorithms, it is imperative that the input data vector $\B{x}$, \YLnote{the albedo in this study}, \Xpolish{exhibits non-compressibility}{is not compressible}.
\Xpolish{{To \Xpolish{make this reconstruction task less specific and more general}{generate non-compressible data}, we reshape the input data vectors $\B{x}$ from $10^5$ random 8 by 8 patterns, increasing their generality. W}{Therefore, w}e randomly sample \YLnote{\Xhide{10 times}}from the uniform distribution $U(0,1)$ to generate \Xhide{10 groups of }inputs \YLnote{$\B{x}$} and it is regenerated several times during the optimization, introducing \YLnote{\Xpolish{additional variability \AVnote{added to what?}}{extra randomization and less compressibility}}}{\YLnote{
Hence, we generate {$\B{x}$} by randomly sampling from the uniform distribution $U(0,1)$. Throughout the optimization process, these inputs are regenerated 10 times, thereby introducing additional randomization and reducing compressibility}}. The simulations are conducted \Xhide{under \YLnote{\Xpolish{significant noise}{a low-light condition}}, }with a total of $1 \times 10^2$ photons. We initialize the masks $\B{M}$ with an $N \times N$ identity matrix and a $\{0,1\}$ Hadamard matrix respectively, and optimize them until the model reports constant losses.}

\Xpolish{The first 6 masks optimized by the ONN are shown in figure \ref{fig:recon_masks}. From it, we can see that the ONN model has very different behaviors under the AGN and the Poisson noise. For the AGN, it tended to open more pixels to increase the light throughput, while it adhered to the RS mode for the Poisson noise. The figure \ref{fig:masks_value_dist} gives a more thorough visualization of the optimized masks by showing their entries' distributions. The x-axis is the values in the masks and the y-axis is the total number of entries in a certain range. This result is consistent with the classification results in the last section, where the RS is mediocre under the AGN but much better under the Poisson noise.}
{Fig. \ref{fig:recon_masks} displays the first 6 optimized masks \YLnote{from both initial matrices} generated by the ONN model \YLnote{\Xpolish{. A notable observation is that the model exhibits distinct behavior patterns under the AGN and Poisson noise}{ under both AGN and Poisson noise}}. Specifically, it tends to open more pixels to enhance light throughput under AGN, but adheres to the RS mode under the Poisson noise. Fig. \ref{fig:masks_value_dist} provides a more detailed visualization of the optimized masks by presenting the distribution of their entries. The x-axis represents the values in the masks, while the y-axis shows the total number of entries within a specific range. This observation aligns with the reconstruction results\Xhide{classification results presented in the previous section}, where the RS performed modestly under AGN but considerably better under the Poisson noise. \Xpolish{The rationale behind this is that re-projection from a captured basis into a basis of sparsity does not yield the same recovery quality under Poisson noise that is provides for AGN. To obtain a performance benefit over the trivial point scanning method, or RS, it is essential that the data is sparse and is captured in a sparse basis. Since random patterns are not sparse, the best scanning strategy is the point scanning, which matches our results.}{}  Gradients incorporating these two noise models during the training process lead the mask optimization along very different directions. From this example we can see that it is not appropriate to design a coding system under AGN and then apply it to Poisson noise data.}

\begin{figure}[ht]  
\begin{subfigure}{\linewidth}
\caption{First 6 ONN Optimized Masks}
\footnotesize	
\centering
\begin{tabular}{>{\centering\arraybackslash}p{0.15\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}}
{Initial matrix} &  Gaussian & Poisson\\
\hline
Identity & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.pdf} \\
\hline
Hadamard & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks_Hadamard.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks_Hadamard.pdf} \\
\end{tabular}
\normalsize

\label{fig:recon_masks}
\end{subfigure}
\begin{subfigure}{\linewidth}
\caption{Value Distributions of ONN Optimized Masks}
\footnotesize
\centering
\begin{tabular}{>{\centering\arraybackslash}p{0.15\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}}
{Initial matrix} &  Gaussian & Poisson\\
\hline
Identity & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian_Raster.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_poisson_Raster.pdf} \\
\hline
Hadamard & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian_Hadamard.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_Poisson_Hadamard.pdf} \\
\end{tabular}
\normalsize
\label{fig:masks_value_dist}
\end{subfigure}
\caption{\Xpolish{Optimizations on $\B{M}$ initialized with identity and Hadamard matrices are studied under the AGN and Poisson noise. $\B{M}$ prefers coding strategies under the AGN but favors the raster scan strategy under the Poisson noise regardless of the initialized matrices.}
{
\Xhide{(\subref{fig:recon_masks}) }Optimizations on the matrix $\B{M}$, initialized with identity and Hadamard matrices, are explored under both AGN and Poisson noise. While $\B{M}$ demonstrates a preference for strategies with higher light throuput under AGN, it consistently leans toward the raster scan strategy under Poisson noise, irrespective of the initialization matrices. The challenge arises from the non-convex nature of this optimization problem, making it difficult to converge perfectly to the identity matrix. Nevertheless, this deviation underscores fundamental distinctions in optimizing masks under these distinct noise models.
}}
\end{figure}


\Xhide{
\begin{figure}[ht]
\caption*{First 6 Optimized Masks}
\centering
\begin{tabular}{>{\centering\arraybackslash}p{0.15\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}|>{\centering\arraybackslash}m{0.35\linewidth}}
\Xhide{Initial matrix} &  Gaussian & Poisson\\
\hline
Identity & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.pdf} \\
\hline
Hadamard & \includegraphics[width=1 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks_Hadamard.pdf} & 
\includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks_Hadamard.pdf} \\
\end{tabular}
\caption{\Xpolish{Optimizations on $\B{M}$ initialized with identity and Hadamard matrices are studied under the AGN and Poisson noise. $\B{M}$ prefers coding strategies under the AGN but favors the raster scan strategy under the Poisson noise regardless of the initialized matrices.}
{
Optimizations on the matrix $\B{M}$, initialized with identity and Hadamard matrices, are explored under both AGN and Poisson noise. While $\B{M}$ demonstrates a preference for strategies with coding under AGN, it consistently leans toward the raster scan strategy under Poisson noise, irrespective of the initialization matrices.
}
}
\label{fig:recon_masks}
\end{figure}
}

\iffalse
\begin{figure}[h]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{ONN optimized masks under Gaussian noise. Left: initialized with the identity matrix. Right: initialized with the Hadamard matrix.}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.svg}
        \includegraphics[width=0.49 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.pdf}
        \includegraphics[width=0.49 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks_Hadamard.pdf}
        \label{fig:gaussian_recon_masks}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering        
        \caption{ONN optimized masks under Poisson noise. Left: initialized with the identity matrix. Right: initialized with the Hadamard matrix.}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.svg}
        \includegraphics[width=0.49\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.pdf}
        \includegraphics[width=0.49\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks_Hadamard.pdf}
        \label{fig:poisson_recon_masks}
    \end{subfigure}
    \caption{First 6 optimized masks}
    \label{fig:recon_masks}
\end{figure}
\fi

\Xhide{
\begin{figure}[h]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Value distribution of the optimal masks under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian.pdf}
        \label{fig:gaussian_recon_masks_dist}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Value distribution of the optimal masks under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_poisson.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_poisson.pdf}
        \label{fig:poisson_recon_masks_dist}
    \end{subfigure}
    \caption{Masks values distribution (x-axis: mask values; y-axis: counts). (\subref{fig:gaussian_recon_masks_dist}) Given a Raster scan mask family, ONN returns a different mask family under the AGN, indicating that Raster scan is always suboptimal. (\subref{fig:poisson_recon_masks_dist}) ONN adheres to the Raster scan, suggesting it is optimal under Poisson noise.
    textcolor{red}{these can be much smaller}
    }
    \label{fig:masks_value_dist}
\end{figure}
}





\Xhide{\begin{figure}[h]  
\caption*{Distributions of ONN reconstructed masks}
    % \begin{subfigure}{0.49\linewidth}
    % \centering  
    % \caption{$\B{M}_G^I$ VS $\B{M}_P^I$}
    % \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist.pdf}    
    % \end{subfigure}    
    % \begin{subfigure}{0.49\linewidth}
    % \centering  
    % \caption{$\B{M}_G^H$ VS $\B{M}_P^H$}
    % \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_Hadamard.pdf}
    % \end{subfigure}   
    \centering
    \includegraphics[width=.8\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist.pdf}
        \caption{\Xpolish{Denote masks initialized with the identity matrix and optimized under the AGN as $\B{M}_G^I$, masks initialized with the identity matrix and optimized under the Poisson noise as $\B{M}_P^I$, masks initialized with the Hadamard matrix and optimized under the AGN as $\B{M}_G^H$, masks initialized with the Hadamard matrix and optimized under the Poisson noise as $\B{M}_P^H$.  
        $\B{M}_G^I$ is going to increase the light throughput by openning more pixels, but $\B{M}_P^I$ is fixed as it is already an ideal choice. $\B{M}_P^H$ is approaching the identity matrix, differently from the $\B{M}_G^H$. Due to the fact that this optimization problem is not perfectly convex, it is difficult to optimize $\B{M}_P^H$ to the perfect identity matrix, but it shows essential differences between the optimization questions under these two distinct noise models.}{ The Poisson noise data is displayed topside-down by negating its counts. Let $\B{M}_G^I$ represent masks initialized with the identity matrix and optimized under the AGN, and $\B{M}_P^I$ denote masks initialized with the identity matrix and optimized under Poisson noise. Additionally, $\B{M}_G^H$ and $\B{M}_P^H$ represent masks initialized with the Hadamard matrix and optimized under AGN and Poisson noise, respectively. While $\B{M}_G^I$ dynamically enhances light throughput by opening more pixels, $\B{M}_P^I$ remains fixed, representing an already ideal choice. Notably, $\B{M}_P^H$ tends to approach the identity matrix, in contrast to the behavior of $\B{M}_G^H$. The challenge arises from the non-convex nature of this optimization problem, making it difficult for $\B{M}_P^H$ to converge perfectly to the identity matrix. Nevertheless, this deviation underscores fundamental distinctions in optimizing masks under these distinct noise models.
        }
    }
    \label{fig:masks_value_dist}
\end{figure}
}


\Xhide{\bnote{talk about onn first in the last section and then show the reconstruction reuslts before the classifiction}}

\Xhide{
\Xpolish{The different results of the optimal masks suggest the masks optimized under the AGN model may not have the same performance under the Poisson noise. If the measured data is Poisson distributed, then the methods proposed under the AGN assumption are problematic.}
{The results from optimizing the masks indicate that the optimal masks under the AGN model may not perform similarly under Poisson noise. Specifically, methods developed under the AGN assumption may not be effective when the measured data follows a Poisson distribution. \YLnote{For instance, coding optimization based on minimizing the mutual coherence in compressed sensing \cite{mordechay2014matrixRIP} may be defective.} The inherent differences in the underlying noise models of the two distributions can lead to suboptimal performance of AGN-optimized masks in Poisson noise scenarios. Therefore, it is crucial to consider Poisson noise when designing coding schemes and algorithms for imaging applications, especially when working with state-of-the-art sensors.}
}

==> hardware_pca_onn/sections/4_methods/sensing_matrices_by_prior.tex <==
\subsection{Sensing Matrices by Priors}

\Xpolish{In the last section, we mentioned the masks $\B{M}$ can be generated by different coding strategies. 
In order to effectively determine the appropriate coding strategies for a given scenario, it is necessary to evaluate the various strategies based on their priors. Image priors, which can vary in type, can enhance the robustness of models in the presence of noise and improve overall image quality \cite{cossairt2012does, levin2007coded}. It should be noted that all of the strategies discussed in this paper possess three distinct prior levels. }
{In the preceding section, we discussed the generation of masks $\B{M}$ using different coding strategies. Evaluating the efficacy of these strategies for a given scenario requires a systematic assessment of their respective priors. Image priors come in varying types and can enhance model robustness in noisy environments and improve overall image quality \cite{cossairt2012does, levin2007coded}. It is important to note that all the strategies outlined in this paper possess three distinct prior levels.}
% \bnote{suggest bolding the priors}
\begin{itemize}
    \item \textbf{Null prior} (data is not compressible or needs to be reconstructed without priors). \Xpolish{Coding strategies in this category require no information about the data. They usually generate full rank matrices as $\B{M}$. In this project, we chose Raster Scan (RS) and Hadamard Basis (HB) for performance evaluation. $\B{M}$ for RS is an identity matrix while it is a Hadamard matrix for HB. On top of these two stratgies, we also include Impulse Imaging (II) which is the optimal measurement that can only be achieved with a sensor array. In our toy example this would be achieved by a camera sensor that captures the image so no coding is necessary. Mathematically, the sensing matrix $\B{M}$ of II is also an identity matrix, but each mask in II has $N$ times longer exposure time compared with RS.}
    {Coding strategies in this category require no information about the data. They usually generate full rank matrices as $\B{M}$. In this project, we chose Raster Scan (RS), Binary Random Basis (BR), and Hadamard Basis (HB) for performance evaluation. $\B{M}$ for RS is an identity matrix while it is a Hadamard matrix for HB. BR employs random values for each pixel in the mask, i.e  $\B{M} \in \{0,1\}^{N\times N}$. On top of these strategies, we also include Impulse Imaging (II) which works as a golden standard in this project. II is an ideal case assuming it can capture the whole data spectrum simultaneously. Mathematically, the sensing matrix $\B{M}$ of II is also an identity matrix, but each mask in II has $N$ times longer exposure time compared with RS.}
    \item \textbf{Reconstruction prior} (data is moderately compressible). \Xpolish{Coding strategies in this category are based on the fact that noise has greater influence on the high-frequency components in any images. We used Low-Frequency-Hadamard Basis which only keeps the low frequency vectors in a Hadamard matrix to study this prior. In this paper, it is labeled as Truncated Hadamard (TH).}
    {One common strategy in coding for images is to take advantage of the fact that noise tends to have a greater impact on high-frequency components. To investigate this phenomenon, we utilized a Low-Frequency-Hadamard Basis approach, in which only the low-frequency vectors of a Hadamard matrix are retained. This approach is referred to as Truncated Hadamard (TH) in this paper.}
    \item \textbf{Task-Specific prior or Selective Sensing prior} (data is extremely compressible). \Xpolish{Coding strategies requires much information from the data and tasks, and their corresponding sensing matrices $\B{M}$ vary from task to task. One strategy in this category is called Hardware PCA (Principal Components Analysis). It computes the most principal components in the training data, and constructs the masks with these components. Another interesting strategy is Selective Sensing (SS) whose sensing matrix $\B{M}$ is not pre-defined nor fixed, but is optimized within a Neural Networks model during the training. This optimization method is called Optical Neural Networks (ONN) in this project.}
    {Coding strategies are an essential component of signal processing that involve gathering task-specific information from data. In order to design these strategies, sensing matrices $\B{M}$ are developed, which can vary depending on the task at hand. One such approach is the Hardware Principal Components Analysis (PCA) technique, which identifies the most principal components in the training data and uses them to construct masks. Another strategy\Xhide{ is the Selective Sensing (SS), which} uses a sensing matrix $\B{M}$ that is not pre-defined or fixed, but rather is optimized using a Neural Networks model during training. In this project, this optimization method is referred to as Optical Neural Networks (ONN).}
\end{itemize}

\Xpolish{In this study, we examined the impact of various priors on a single-pixel imaging system in terms of\Xhide{ both \textbf{reconstruction}} and classification. Firstly, we explained our the methods for imeplementing the constraints in the single-pixel imaging model. Then, we simulated the effect of different prior types on classification performance using the MNIST dataset. Subsequently, we tested the feasibility of these strategies by experiments. \Xhide{Specifically, we first conducted a theoretical analysis to compare the reconstruction capabilities of the HB and RS in the presence of noise. Subsequently, we simulated the effect of different prior types on classification performance using the MNIST dataset. \bnote{is our theoretical analysis novel?} \rnote{I thought it was novel before read the hadamard book}}}
{In this study, we examine the impact of various priors on a single-pixel imaging system in terms of classification. Firstly, we explain our methods for implementing constraints in the single-pixel imaging model. Then, we simulate the effect of different prior types on classification performance using the MNIST dataset. Finally, we test the feasibility of these strategies through experiments.}



\Xhide{\bnote{The first and second sentences here are somewhat confusing due to the "Proposed model" language. We have not proposed a model yet, so unclear if it is our model or someone else's.} \rnote{This model is proposed by Rebecca, but I believe there is some error on the negative entries} In equation \ref{eqn:NoiselessMeasurement}, the parameter regarding the number of photons is an integral part of the mathematical representation of $\B{x}$. To further examine the mask basis under varied light levels, we propose a revised photon-counting model that decouples $\B{M}$ from the number of photons. In the following sections, we detail the development of this new model and provide insights into its practical implementation to avoid violating these constraints.} 

==> hardware_pca_onn/sections/5_results_theory.tex <==
In this section, we start with a theoretical investigation on the reconstruction performances of null-prior strategies. Then the reconstruction and classification performances of all strategies and fairly compared by simulations and experiments. 

\subsection{Theoretical treatment for Null-Prior Reconstruction }

\YLnote{The dual branch section is removed and the ref link doesn't work}
% \textcolor{blue}{This section could be taken out.}
Define $\B{I}$ as the identity matrix and $\totphoton = \rho \tau$ as the total number of photons from the source. Given the noisy photon counts $\tilde{\B{y}}$ and the full-rank mask basis $\B{M}$, we can reconstruct the field of view $\tilde{\B{x}} = \B{M}^{-1} \tilde{\B{y}}$.
Based on Parseval's identity, the covariance matrix of a vector $\B{b}$ is $\B{\Sigma}_{\B{b}\B{b}} = c^2 \sigma^2 \B{I}$ if $\B{b} = \B{W a}$ where $\B{\Sigma}_{\B{a}\B{a}} = \sigma^2 \B{I}$ and 
% $\B{W}$ is $c$ times an orthonormal matrix
$\B{W} \B{W}^\top = c^2 \B{I}$
. For RS, we have $\lambda = \frac{\totphoton}{N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{I}\B{x}, \sigma^2 \B{I})$. Thus, the reconstructed field of view is 
\begin{equation}
    \label{eqn:RS_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{\sigma^2 N^4}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
For HB, we have $\lambda = \frac{\totphoton}{2N^2}$  and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{H}\B{x}, 2\sigma^2 \B{I})$ due to the dual branch trick mentioned in section \Xpolish{\ref{sssection:DualBranch}}{\ref{ssection:constraints}}. For $\B{H}^{-1}$, $c = \sqrt{\frac{1}{N}}$. The reconstructed field of view is 
\begin{equation}
    \label{eqn:HB_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{8 \sigma^2 N^3}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
% Therefore, when considering the AWGN model, using the Hadamard matrix can improve the SNR of the reconstructed field of view when $N$ is large.
Therefore, using the Hadamard matrix in the AWGN model can improve the signal-to-noise ratio (SNR) of the reconstructed field of view when the number of elements, $N$, is large. 

When the noise is Poisson distributed, the covariance matrix of the noisy photon counts depends on the choice of $\B{M}$. Suppose $\sigma_j$ is the standard deviation of $\lambda \tilde{y}_j$, the $j_\text{th}$ measured noisy photon counts. For the RS, we have $\sigma_j^2 = \lambda x_j$ and $\lambda = \frac{\totphoton}{N^2}$. The covariance matrix of the reconstructed field of view is thus 
\begin{equation}
    \label{eqn:RS_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{N^2}{\totphoton}\diag\{x_1, x_2, \cdots, x_N\}
    \end{aligned}.
\end{equation}
% For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$ by the Skellam Distribution in section \ref{sssection:DualBranch}. Since Hadamard matrices only includes $\pm 1$ entries, we further have $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$ and the covariance matrix  

In the case of the HB, we can express the rate parameter $\lambda$ as $\lambda = \frac{\totphoton}{2N^2}$, as demonstrated in section \ref{ssection:constraints} using the Skellam Distribution. Additionally, we can express the variance of each element in the sum as $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$. As Hadamard matrices only contain entries of $\pm 1$, this reduces to $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$. Using this information, we can construct the covariance matrix
\begin{equation}
    \label{eqn:HB_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{2N \sum_{k=1}^N x_k}{\totphoton}  \B{I}
    \end{aligned}.
\end{equation}
% Therefore, the mean squared error (MSE) of HB is 2 times that of RS under Poisson noise. This factor of 2 arises from the dual branch trick. In other words, HB can never exceed RS in reconstruction error even when measuring with 2 PMTs simultaneously.
The results of our analysis reveal that the mean squared error (MSE) of the HB method is twice that of the RS method when the noise is Poisson distributed. This difference is attributed to the dual branch trick utilized in the HB method. Despite the use of two PMTs in the HB method, it is unable to surpass the reconstruction error of the RS method. These findings demonstrate the limitations of the HB method in comparison to the RS method under Poisson noise conditions.




==> hardware_pca_onn/sections/biography.tex <==



\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{\homedir/figures/biography/yizhou_lu_300ppi.jpg}}]{Yizhou Lu}
\Xhide{Biography text here.}
obtained his B.S. degree in Geochemistry from Nanjing University, China, in 2017, followed by M.S. degrees in Materials Science and Engineering and Computer Sciences from the University of Wisconsin-Madison, WI, USA, in 2019 and 2023, respectively. Currently pursuing a Ph.D. degree with the Electrical and Computer Engineering Department at the University of Wisconsin-Madison, his research interests encompass computational imaging and information theory.
\end{IEEEbiography}




\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{\homedir/figures/biography/Trevor_Seets_Headshot.png}}]{Trevor Seets}
\Xhide{Biography text here.}
received his B.S. and M.S. degree in electrical engineering from the University of Wisconsin-Madison in 2019 and 2023, respectively. He is now a Ph.D. student under Professor Andreas Velten at UW-Madison. His research interests include computational optics, statistical signal processing, and imaging.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{\homedir/figures/biography/2022-04_FGB_300dpi.png}}]{Felipe Gutierrez Barragan}
\Xhide{Biography text here.}
is a Senior Software Engineer at Ubicept. He received his B.S. (2016), M.S. (2019), and Ph.D. (2022) in Computer Sciences from the University of Wisconsin-Madison.  His Ph.D. research focused on practical modifications to SPAD-based and time-of-flight 3D cameras to reduce power consumption and data bandwidth while preserving or increasing their precision. His research interests include computational imaging, computer vision, and machine learning.
\end{IEEEbiography}

% \begin{IEEEbiographynophoto}{Ehsan Ahmadi} earned his B.S. in Computer Software Engineering from Iran University of Science and Technology, Tehran, Iran, and his M.S. in Electrical and Electronics Engineering from Southern Illinois University, Carbondale, Illinois. Currently, he is pursuing a Ph.D. in Computer Engineering at UW-Madison, focusing on Fluorescence Lifetime Imaging Microscopy (FLIM).
% \end{IEEEbiographynophoto}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{\homedir/figures/biography/ehsan_ahmadi300.png}}]{Ehsan Ahmadi}
\Xhide{Biography text here.}
earned his B.S. in Computer Software Engineering from Iran University of Science and Technology, Tehran, Iran, and his M.S. in Electrical and Electronics Engineering from Southern Illinois University, Carbondale, Illinois. Currently, he is pursuing an M.S. in Computer Engineering at UW-Madison, focusing on Fluorescence Lifetime Imaging Microscopy (FLIM).
\end{IEEEbiography}



    




\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{\homedir/figures/biography/andreas_velten300.jpeg}}]{Andreas Velten}
\Xhide{Biography text here.}
received the B.A. degree in physics from the Julius Maximilian University of Wurzburg, Wurzburg, Germany, in 2003, and the Ph.D. degree in physics from the University of New Mexico, Albuquerque, NM, in 2009. From 2010 to 2012, he was a postdoctoral research associate with the Massachusetts Institute of Technology, Cambridge, MA, USA, where he was working on high speed imaging systems that can look around
a corner using scattered light. From 2013 to 2016, he was an associate scientist with the Laboratory for Optical and Computational Instrumentation, University of Wisconsin–-Madison, Madison WI, USA, working in optics, computational imaging, and medical devices. Since 2016, he has been an associate professor with the Biostatistics and Medical Informatics, Electrical and Computer Engineering Department, University of Wisconsin–-Madison. His research focuses on performing multidisciplinary work in applied computational optics and imaging.
\end{IEEEbiography}


==> hardware_pca_onn/sections/title.tex <==
Selective Sensing

==> hardware_pca_onn/sections_2022_Dec_OLD/0_abstract.tex <==
Abstract Single-pixel computer vision under poisson noise

==> hardware_pca_onn/sections_2022_Dec_OLD/1_intro.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

% Coding is a fundamental technique used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance. For applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging, coding enables a low dimensional sensor to sample in a \textbf{complete} measurement space.
% %an $n$-dimension measurement space.
% Due to its range of applications, coding schemes have been investigated thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise. It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under the AGN. This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 

% In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.

% Coding is a widely-used technique in computational imaging (CI) that aims to improve image quality and reduce the dimensionality of the measurement space \cite{cossairt2012does}. It has been shown to be effective in a variety of applications, including single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging. These techniques rely on coding to allow low-dimensional sensors to sample a complete measurement space. While coding schemes have been widely studied, most research has focused on low noise scenarios or additive Gaussian noise models. This is due to the fact that additive Gaussian noise, which is introduced by imperfections in cameras and sensors, is easy to model both analytically and computationally as it is a signal-independent linear noise.



\IEEEPARstart{C}{oding} or multiplexing is a widely used technique in computational imaging (CI) for improving image quality \cite{cossairt2012does}. In addition to increasing light throughput, coding can reduce the dimensionality of the measurement space, which is a common metric for the performance if a CI method. Coding allows low-dimensional sensors to sample a complete measurement space in applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging.

While coding schemes have been extensively researched, the mathematical foundation is based on low noise scenarios or Additive Gaussian Noise (AGN) models. This is because the AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurements in cameras and sensors, and is easy to analyze and compute analytically as it is signal-independent and linearly additive.

However, as optical imaging technologies improve, readout noise is decreasing and Poisson noise, due to the quantized nature of light, is becoming more dominant in measured imaging data. Poisson noise is a fundamental physical property of light and arises from the discrete nature of light. An optical signal is composed of discrete photons that can not be arbitrarily divided across codes. Therefore, in state-of-the-art and future sensors measuring visible light, it is important to consider measurement and processing techniques under Poisson noise.

Previous research has shown that coding behaves substantially different under Poisson noise compared to the AGN \cite{duarte2008CS}, which is particularly significant in emerging single-photon sensors that only experience Poisson noise. This means that existing coding and computational imaging techniques may not be applicable to single-photon or "few-photon" sensitive sensors (such as most state-of-the-art CMOS and machine vision cameras) where readout noise is on the order of just a few photons.

In this paper, we analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. Similar to the conclusion of Cossairt et al., we find that coding provides little benefit in unbiased prior free image reconstruction tasks, but can provide significant performance gains \cite{cossairt2012does} when codes are optimized specifically for downstream vision tasks.


\iffalse
\textbf{New paper story:}
\begin{enumerate}
    \item Coding is one of the fundamental techniques used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance.\bnote{Insert definition of computational imaging, probably similar to the one of \cite{cossairt2012does}}.
    \item 
    Coding is important in any application where an n dimensional measurement space is sampled with a sensor or dimensionality $<$ n. It is relevant in single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, polarization imaging, compultational imaging, and compressed sensing.
    \item Due to its range of applications coding schemes have been explored thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. 
    \item As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. \item In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise.
    \item It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under AGN.
    % \item For example, recent work explored the regimes where coding/computational imaging can lead to improved performance \cite{cossairt2012does}. The conclusion of their analysis was that coding/computational imaging can improve performance in scenarios where the dominant noise source is due to Gaussian noise often associated to read-out noise. However, when the dominant noise source is Poisson noise, due to the random arrival of photons, the performance gains are negligible. In other words: In a Poisson noise limited measurement, the best "code" is the trivial "pinhole" code, where each sample is scanned on it's own. 
    % \item Beccas paper.
    \item This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 
    \item In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. 
    \item Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.
\end{enumerate}
\fi

\section{Outline (for planning only)}
Definition of coding, sensor dimensionality, measurement dimensionality

definition of signal reconstruction, imaging, and pattern recognition

\bnote{Single-pixel imaging.} 

\bnote{Compressive sensing} Compressive sensing has enabled the design of single-pixel imaging systems that are able to reconstruct images from very few measurements. 
These systems are useful in applications where it is expensive to have pixel arrays that sample the full image in parallel. 
For example in low-light applications, PMTs are commonly used, and it is expensive to build arrays of PMTs.

Additionally, compressive sensing can also be applied to other imaging modalities such as hyper-spectral imaging,  fluorescence imaging etc... 

\bnote{Signal reconstruction under Poisson noise.} The most efficient compressive sensing systems have been implemented for signal reconstruction under Gaussaian noise. 
Unfortunately, compressive sensing in the presence of Poisson noise does not benefit from the same low-sample complexity \cite{raginsky2011performance}.
This is due to XXX

\bnote{Signal reconstruction amplifies noise so we should skip it.} 
Signal reconstruction, however, is often an intermediate step. 
The final goal is often to execute a high-level task such as classification or segmentation.
To this end, current computer vision systems extract features from the reconstructed signal and use these features to accomplish the task at hand.
In this paper, we find that in a single-pixel imaging system under Poisson noise, it is sub-optimal to reconstruct from compressive measurements and then extract features.
This is because the signal reconstruction step amplifies noise.

\bnote{Task Specific Masks vs General Masks}
Should we adapt our masks based on our objective (pattern recognition task, image reconstruction domain, different types of signals)? The conventional wisdom for AGN is that that doesn't help much. 

Now we need to do analysis:
define toy problems, discuss performance for simple adaptive masks
conclusion: with Poisson noise signal reconstruction makes no sense. But pattern recognition works with an adapted mask set.

How do we find the masks:
PCA, ONN

\bnote{Optical neural nets to the rescue.} 
Inspired by recent trends in optical neural networks, we propose a single-pixel vision system for low-light applications. 
By capturing image features directly we avoid amplifying noise

\bnote{How to design these masks.} 

Discussion:
end to end computational imaging with adaptive asks works under Poisson noise.

This provides an additional motivation for proposed optical ANNs or ANNs with optical layers. Such an architecture allows me to choose where in the design I want to add the Poisson noise.

Possibly: Quantum mechanics interpretation.

==> hardware_pca_onn/sections_2022_Dec_OLD/3_background.tex <==
% \IEEEPARstart{A}{} single-pixel sensor such as a photonmultiplier tube (PMT) can only count the total number of photons in measurements. A Digital Micromirror Device (DMD) consisting of millions of mirror chips tunable by $\pm 12$ degrees is necessary for the spatial information. When the photons from the whole field of view arrive at the DMD, the chips split and reflect them as two branches. In each measurement, the sensor counts the photons from those chips, or pixels, in other words, facing it. 

\IEEEPARstart{A}{} single-pixel sensor, such as a photon multiplier tube (PMT), is capable of detecting the total number of photons in a measurement, but lacks the ability to provide spatial information. In order to obtain this information, a Digital Micromirror Device (DMD) must be used. The DMD consists of millions of mirror chips that are tunable by $\pm 12$ degrees and can split and reflect photons from the field of view into two separate branches. During a measurement, the sensor counts the photons from the chips, or pixels, that are facing it, providing spatial information about the distribution of photons within the field of view.


\subsection{Model Formulation}

% introduce the Poisson noise
% start from noiseless model

% \subsubsection{Ideal Model}



% The single-pixel-sensing process, if ignoring noise, can be expressed as the following equation 
% \begin{equation*}
%     \begin{aligned}
%         n_{\gamma} &=  j \sum_{k=1}^N x_k \sum_{l=1}^L m^B_{kl}  \tau_l \\
%             &= \lambda \sum_{k=1}^N x_k m_k
%     \end{aligned},
% \end{equation*}
% where $n_\gamma$ is the total number counted by the sensor, $N$ is the total number of pixels, $m^B_{kl} \in \{-1, 1\}$ and $\tau_l$ are the binary status of the $k_\text{th}$ DMD chip and the exposure time for the $l_\text{th}$ physical measurement respectively, $x_k$ is the the reflection coefficient of the $k_\text{th}$ subarea of the field of view measured as one pixel, and $j$ is the photon flux cast on each $x_k \in [0,1]$. Suppose the field of view is illuminated uniformly, $x_k=1$ stands for a white pixel while $x_k=0$ represents a black pixel. The $m_k \in \IR$ is introduced for simplicity, which physically stands for the fact that we can obtain a real-number mask by combining multiple binary masks with different exposure periods. The scaling factor $\lambda$ is related to the photon distribution among all the masks and will be discussed later. Thus, for the $t_\text{th}$ measurement, we have 
% \begin{equation*}
%     \begin{aligned}
%         {n_\gamma}_t &= \lambda \sum_{k=1}^N M_{tk} x_k 
%     \end{aligned}.
% \end{equation*} 
% Here, we introduce the normalized measurement $y = \frac{n_\gamma}{\lambda}$ as the optical nature of the objects.
% The corresponding matrix expression for the single-pixel imaging is 
% \begin{equation}
%     \label{eqn:NoiselessMeasurement}
%     \begin{aligned}
%         \B{y} &=  \B{M} \B{x}
%     \end{aligned}.
% \end{equation} 

% Two noise models were investigated in this project. The first one is the popular Additive White Gaussian Noise (AWGN) with the following form
% % \subsubsection{Gaussian Noise Model}

% \begin{equation}
%     \begin{aligned}
%         \lambda\tilde{\B{y}} &\sim \mathcal{N}(\lambda \B{M} \B{x} , \sigma \B{I})
%     \end{aligned}.
% \end{equation} 
% % \subsubsection{Poisson Noise Model}
% The $\sigma$ is the standard deviation. The other is the Poisson Noise model for photon-counting systems \cite{willet2009CSPoisson} with the following form
% \begin{equation}
%     \begin{aligned}
%         \lambda\tilde{\B{y}} &\sim \mathcal{P}(\lambda \B{M} \B{x})
%     \end{aligned}.
% \end{equation} 

Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ masks, the single-pixel-sensing process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{Mx}
    \end{aligned},
\end{equation}
where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is the sensing masks linearly projecting the field of view , and $\B{y} \in \IR^{m \times 1}$ is the corresponding photon counts \cite{willet2009CSPoisson}. There are two main physical constraints when optically implementing equation \ref{eqn:NoiselessMeasurement} \cite{neifeld2003dual}. 
% \begin{enumerate}    
%     \item\label{constraint:photonNumber} The single-pixel imaging model concerns the re-distribution of available photons among masks \cite{neifeld2003dual}. No photons should be created by improper entries in the mask basis $\B{M}$.
%     \item\label{constraint:negativeEntry}Negative values of the masks $\B{M}$ cannot be implemented directly \cite{neifeld2003dual}. 
% \end{enumerate}

\begin{enumerate}
    \item\label{constraint:photonNumber}The single-pixel imaging model involves the allocation of available photons among masks, as discussed in \cite{neifeld2003dual}. It is important to ensure that the mask basis $\B{M}$ does not produce additional photons through improper entries. 
    \item\label{constraint:negativeEntry}It is not possible to physically implement negative values for the masks $\B{M}$, as demonstrated in \cite{neifeld2003dual}. 
\end{enumerate}

% This concise model, however, is not convenient for us to investigate the same mask basis under different light levels. So it is necessary to reformulate this photon-counting model where $\B{M}$ and $\B{x}$ are not related to the number of photons. The new photon-counting model and some tricks for the implementation are discussed in the following sections.

To further examine the mask basis under varied light levels, we propose a revised photon-counting model that decouples $\B{M}$ and $\B{x}$ from the number of photons. In the following sections, we detail the development of this new model and provide insights on its practical implementation.


\subsubsection{Photon Distribution Factor} \label{sssection:PDF}

Suppose the total number of available photons is $\totphoton$. Instead of constraining the mask basis $\B{M}$, we define a Photon Distribution Factor $\lambda$ in the single-pixel imaging model. In our hypothesis, ${\totphoton_j}$ photons are distributed to the $j_\text{th}$ mask, $\B{x} \in [0,1]^{N \times 1}$ is the unit image representation of the field of view, and there is no idle time between masks. In other word, each mask is re-scaled to have the maximum abstract value equal to $1$. The measured photon counts in the $j_\text{th}$ measurement $\photon_j = \frac{\totphoton_j}{N} \sum_{k=1}^N \frac{M_{jk}}{v_j} x_k$ where $v_j$ is the maximum abstract value of the $j_\text{th}$ mask. It is not necessary to have $\photon_j = \totphoton_j$ as some entries in masks block photons. If $\totphoton_j$ is proportional to $v_j$, it is obvious that $\totphoton_j = \frac{v_j \totphoton}{N \sum_{k=1}^m v_k}$. Let $\lambda = \frac{\totphoton}{N \sum_{k=1}^m v_k}$, and we have $\photon_j = \lambda \sum_{k=1}^N M_{jk} x_k$. Though $\photon_j$ is what is measured by the sensor and also what is contaminated by noise, it is convenient to let $\tilde{y}_j = \frac{\photon_j}{\lambda}$ to resemble the noiseless model above. Here, we name $\B{y}$ the normalized photon counts.

% Thus, we have the general noisy model
%  \begin{equation}
%     \label{eqn:GeneralNoisyMeasurement}
%     \begin{aligned}
%         \lambda \tilde{\B{y}} &\sim  \mathcal{D}(\lambda\B{Mx}, \cdot)
%     \end{aligned},
% \end{equation}
% where $\mathcal{D}$ is the distribution of the interested noise model, $\tilde{\B{y}}$ is the noisy photon counts, and $\cdot$ is the optional parameter of the covariance.

Two noise models were investigated in this project. The first one is the Additive White Gaussian Noise (AWGN) stemming from the imperfectness of sensors \cite{boyat2015review} with the following form
% \subsubsection{Gaussian Noise Model}

\begin{equation}
    \begin{aligned}
        \lambda\tilde{\B{y}} &\sim \mathcal{N}(\lambda \B{M} \B{x} , \sigma^2 \B{I})
    \end{aligned}
\end{equation} 
% \subsubsection{Poisson Noise Model}
where the $\sigma$ is the standard deviation. The other is the Poisson Noise model for photon-counting systems \cite{willet2009CSPoisson} originating from the statistical nature of photons \cite{boyat2015review} with the following form
\begin{equation}
    \begin{aligned}
        \lambda\tilde{\B{y}} &\sim \mathcal{P}(\lambda \B{M} \B{x})
    \end{aligned}.
\end{equation} 

By introducing the Photon Distribution Factor, the mask basis $\B{M}$ is freed from constraint \ref{constraint:photonNumber}.


\subsubsection{Dual-Branch Trick for Negative Entries}\label{sssection:DualBranch}

Although we can obtain a negative number of photons from the difference between the two measurements, the Poisson noise cannot be directly applied to these values. Otherwise, it violates the nature of Poisson distributions and the fact that Poisson noise appears in the sensors. On the contrary, noise should be considered in both branches independently. 

To create the two branches, the mask $\B{M}$ should be split into $\B{M}^+ = \text{ReLU}(\B{M})$ and $\B{M}^- = \text{ReLU}(-\B{M})$. The superscripts of the parameters indicate the branches they belong to. Intuitively, we have $\lambda \tilde{\B{y}} = \lambda \tilde{\B{y}}^+ - \lambda \tilde{\B{y}}^-$ where $\tilde{\B{y}}^+$ and $\tilde{\B{y}}^-$ are noisy photon counts measured by $\B{M}^+$ and $\B{M}^-$ respectively. In this case, it is worth noting that the Photon Distribution Factor $\lambda = \frac{\totphoton}{N (\sum_{k=1}^m v_k^+ + \sum_{k=1}^m v_k^-)}$ where all the parameters are of the same meaning as in section \ref{sssection:PDF}.

In the AWGN model, the measurement $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{Mx}, 2\sigma^2 \B{I})$ with the dual-branch trick. But in the Poisson noise model, the measurement $\lambda \tilde{\B{y}} \sim \text{Skellam}(\lambda \B{M^+ x}, \lambda \B{M^- x})$. 

\subsection{Noise models}

\subsection{Scan Strategies with Different Priors}

% In general, single-pixel imaging involves computational and non-computational methods. Their essential difference is that computational imaging requires optical coding and computational decoding steps \cite{cossairt2012does}. A typical non-computational strategy is the raster scan by which the sensor measures each pixel sequentially \cite{duarte2008CS}. Correspondingly, computational strategies measure a combination of pixels simultaneously. The computational strategies can be further classified by their masks. The following is a natural arrangement of the strategies based on mask generations.  

Single-pixel imaging is a technique that involves both computational and non-computational methods. The primary difference between the two is that computational imaging requires additional steps of optical coding and computational decoding in order to capture and process the image \cite{cossairt2012does}. Non-computational methods, such as raster scanning, involve measuring each pixel sequentially \cite{duarte2008CS}. On the other hand, computational methods measure a combination of pixels simultaneously and can be further classified based on the type of mask used. In this paper, we will arrange the various computational strategies based on their mask generation techniques.
\begin{figure}[h]
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.711\linewidth]{\homedir/figures/RasterScan.png}
        \caption{Non-computational Imaging}
        \label{fig:RasterScan}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=1\linewidth]{\homedir/figures/BasisScan.png}
        \caption{Computational Imaging}
        \label{fig:BasisScan}
    \end{subfigure}
    \caption{Single-Pixel Imaging Methods}
    \label{fig:SinglePixelImaging}
\end{figure}
 
\begin{enumerate}
    \item Static strategies: 
    Masks are predetermined and fixed.
    \begin{enumerate}
        \item Non-compressible strategies
        \begin{enumerate}
            \item Raster Scan (RS). In this strategy, only one pixel will be scanned in each measurement. Thus, $\B{M} = \B{I}$.
            \item Impulse Imaging (II). II captures the field of view by a pixel array. In this case, each pixel gets $N$ times as much as the exposure time of RS. Mathematically, $\B{M} = N\B{I}$. Alternatively, we can treat it as another RS with $N$ times as many photons. The II works as the baseline for the comparisons with other strategies.
            \item Hadamard Basis (HB). In this strategy, we choose the 2-D Walsh-Hadamard matrix $\B{H}$ as the mask basis.
        \end{enumerate}
        
        \item Compressible strategies
        \begin{enumerate}
            \item Randomly Truncated Hadamard (RTH). Given a default Walsh-Hadamard matrix $\B{H}$ and randomly pick several rows as $\B{M}$.
            \item Low-Frequency-Truncated Hadamard (LFTH). Given a default Walsh-Hadamard matrix $\B{H}$ and only keep the first several rows as $\B{M}$.
            \item Sorted-Truncated Hadamard (STH). Re-order the rows according to their correlation coefficients with the mean of training images. More relevant ones are picked first.
            \item Hardware Principal Components Analysis (HPCA). The DMD displays the PCA components calculated from the training images.
        \end{enumerate}
    \end{enumerate}
    
    \item Dynamic strategies: Masks can be optimized based on the tasks.
    \begin{itemize}
        \item Optical Neural Networks (ONN).
    \end{itemize}
\end{enumerate}
% This classification is intuitive but not conducive in deciding proper mask basis. A more sensible way is to evaluate these strategies by their priors. Image priors, depending on their types, can strengthen models' robustness to noise and improve the quality \cite{cossairt2012does, levin2007coded}. Conspicuously, All the strategies mentioned above have the following three prior levels.
In order to effectively determine the appropriate mask basis for a given scenario, it is necessary to evaluate the various strategies based on their priors. Image priors, which can vary in type, can enhance the robustness of models in the presence of noise and improve overall image quality \cite{cossairt2012does, levin2007coded}. It should be noted that all of the strategies discussed in this paper possess three distinct prior levels.
% Thus, these strategies can be re-grouped as follows. 
% For example, the RS doesn't need  , the LFTH is based on the fact that low-frequency components are more robust, and the HPCA learns information from training data. 

\begin{enumerate}
    \item Null-Prior: RS, II, and HB. It requires no information before measurements.
    \item Reconstruction-Prior: RTH and LFTH. This prior is from the inductive bias for signal reconstruction regardless of the data.
    \item Task-Specific-Prior: STH, HPCA, and ONN. This prior requires the features from training data of a specific task.
    % make plots based on the groups
\end{enumerate}



% \subsection{Illumination determination}




==> hardware_pca_onn/sections_2022_Dec_OLD/4_methods.tex <==
% \IEEEPARstart{I}{n} this project, we analyzed the influence of different priors on a single-pixel imaging system regarding both reconstruction and classification and propose the inductive bias for single-pixel imaging. The first step was a theoretical investigation to compare the reconstruction performances of HB and RS in both noise models. Then, we investigated the roles of different prior types in classification on the MNIST dataset by simulations.

\IEEEPARstart{I}{n} this study, we examined the impact of various priors on a single-pixel imaging system in terms of both reconstruction and classification. Specifically, we first conducted a theoretical analysis to compare the reconstruction capabilities of the HB and RS in the presence of noise. Subsequently, we simulated the effect of different prior types on classification performance using the MNIST dataset.

% if have experiment, list here

% \subsection{Physical Constraints and Solutions}

% There are two main physical constraints for the implementation of equation \ref{eqn:NoiselessMeasurement} optically \cite{neifeld2003dual}. Firstly, negative values of the masks $\B{M}$ cannot be implemented directly \cite{neifeld2003dual}. Secondly, the single-pixel imaging model concerns the re-distribution of available photons among masks \cite{neifeld2003dual}. When optimizing $\B{M}$, no photons should be created by improper entries.

% \subsubsection{Dual-Branch Trick for Negative Entries}

% Although we can obtain a negative number of photons from the difference between the two measurements, the Poisson noise cannot be directly applied to these values. Otherwise, it violates the nature of Poisson distributions and the fact that Poisson noise appears in the sensors. On the contrary, noise should be considered in both measurements.

% Supposing we split the masks $\B{M}$ into the positive part $\B{M}^+$ and the negative part $\B{M}^-$, the final measurement $\lambda \tilde{\B{y}} = \lambda  \B{M}^+\B{x} - \lambda (1 - \B{c})\odot  \tilde{\B{y}}^-$. The positive and negative measurement obeys two independent distributions and the coefficient $\B{c}$ is not necessarily to be $\frac{1}{2}$. The determination of $\B{c}$ will be discussed in the next section.

% In the AWGN model, the measurement $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{Mx}, 2\sigma \B{I})$ with the dual-branch trick. But in the Poisson noise model, the measurement $\lambda \tilde{\B{y}} \sim \text{Skellam}(\lambda \B{Mx}, \diag\{\lambda \B{M}^{|\cdot|}\B{x}\})$. The superscript $|\cdot|$ represents taking the elementwise absolute values of the matrix.


% \subsubsection{Photon Distribution on Masks}








% In the derivation, we decided to use a Gaussian noise $\mathcal{N}(x,x)$ to approximate $\mathcal{P}(x)$.

\subsection{Simulations}

% To interpret the roles of the different priors in reconstruction and classification, we conducted a bunch of simulations on the MNIST dataset. The model for all the simulations consists of a homemade scanner module mimicking the single-pixel imaging and an Artificial Neural Networks (ANN) classifier. Notably, the ONN's scanner and classifier are optimized together. 

% A noise layer is implemented at the end of the scanner to generate noise photon counts $\tilde{\B{y}}$. The random number functions, in principle, do not have gradients. Studies on the \textit{score function estimator method} suggest that their gradients can be restored by \textit{Monte Carlo gradient estimation} \cite{shakir2020scorefunction}.

To understand the impact of different priors on reconstruction and classification, we conducted a series of simulations using the MNIST dataset. Our model included a custom scanner module that simulated single-pixel imaging and an Artificial Neural Network (ANN) classifier. The scanner and classifier were optimized together using the ONN approach.

To simulate noise, we included a noise layer at the end of the scanner that generated photon count estimates $\tilde{\B{y}}$. While random number functions typically do not have gradients, we utilized the score function estimator method and Monte Carlo gradient estimation to restore these gradients, as demonstrated in previous research by Shakir et al. \cite{shakir2020scorefunction}.


\subsubsection{MNIST Data Pre-processing}

% The MNIST dataset includes handwritten numbers from 0 to 9 with default size of 28 by 28. To reconcile the data to the Hadamard matrices, we padded black pixels at the edges of each image to resize it into 32 by 32. Afterward, we adjusted the range of all the pixel values from $[0,1]$ to $[0.3, 1]$. Since the black pixels never invoke Poisson noise of which the variance is proportional to the expected photon counts, this operation renders the dataset more persuasive for different noise models.

The MNIST dataset consists of handwritten digits from 0 to 9, with a default size of 28 by 28 pixels. In order to align the data with the Hadamard matrices, we padded the images with black pixels at the edges to resize them to 32 by 32 pixels. We also transformed the range of all pixel values from $[0,1]$ to $[0.3, 1]$. This operation enhanced the persuasiveness of the dataset for various noise models, as the added black pixels do not generate Poisson noise, whose variance is proportional to the expected photon counts.

% training details, how to evaluate the classification
\subsubsection{Scanner}

% The scanner module is modified from the \textit{Linear} module in PyTorch. In addition to the input and mask matrix, it also requires the total number of available photons and noise models as the arguments. The tricks mentioned in section \ref{sec:3_background} are implemented inside. Photon Distribution Factor $\lambda$ is updated whenever the mask is changed. The last sub-module takes the noiseless photon counts and returns its noisy version. The scanner can also reconstruct the field of view when the measurement is finished. 

In order to improve the performance of our scanner module, we have modified the \textit{Linear} module from PyTorch. The modified module takes in three primary arguments: the input and mask matrix, as well as the total number of available photons. Additionally, it requires the implementation of certain tricks, as described in Section \ref{sec:3_background}, in order to optimize its performance.

One key aspect of our modified module is the incorporation of the Photon Distribution Factor $\lambda$, which is dynamically updated whenever the mask is altered. This ensures that the scanner can accurately simulate the photon distribution throughout the measurement process.

Finally, the modified module also includes a sub-module that takes in the noiseless photon counts and returns a noisy version, replicating the effects of real-world measurement noise. Upon completion of the measurement, the scanner is also able to reconstruct the field of view with high accuracy.

\subsubsection{Classifier}

% The classifier is an ANN model including two hidden layers with 40 and 128 nodes. It takes the re-centered normalized noisy photon counts as the input and predicts its corresponding number. The re-centered normalized noisy photon counts is calculated by $\tilde{\B{y}} - \B{M} \B{\bar{x}}_T$ where $\B{\bar{x}}_T$ is the average of the training data. After each hidden layer, there is a dropout layer followed by a ReLU activation layer.
In this study, we employed a two-hidden layer artificial neural network (ANN) classifier with 40 and 128 nodes as the main model for predicting the corresponding number of re-centered, normalized, and noisy photon counts. The input data for the classifier was obtained by subtracting the average of the training data, represented by $\B{\bar{x}}_T$, from the re-centered normalized noisy photon counts, denoted by $\tilde{\B{y}}$. To prevent overfitting and improve the generalizability of the model, dropout layers were inserted after each hidden layer, followed by a ReLU activation layer.

% run a comparison show that number of parameters doesn't change a lot? use reconstructed and compare with the direct ones

\subsubsection{Performance Evaluation}

% The models' performances were evaluated by their average classification rates. For each strategy, the model was assessed 5 times independently. After randomly splitting the dataset into training and validation sets in each assessment, the scanner of each model engendered the noisy photon counts. The classifier was trained on the corresponding re-centered normalized photon counts until the validation rate grew insignificantly or dropped. The best validation rate throughout all epochs was chosen as the representative performance for this assessment. Eventually, the model's overall performance referred to the average of all 5 representatives.

The performances of the models were evaluated through their average classification rates. To ensure a thorough assessment, the model was tested five times independently, each time with a randomly split dataset for training and validation. During each assessment, the scanner generated noisy photon counts, which were then used to train the classifier until the validation rate reached a plateau or declined. The best validation rate achieved during the training process was chosen as the representative performance for each assessment. The overall performance of the model was determined by averaging the results of all five assessments.

\subsubsection{Reparameterization Trick for Poisson Noise}

% include a figure
% Unlike the static strategies, the ONN can optimize the masks by the back-propagation during the training. This method has several advantages.
% \begin{enumerate}
%     \item The model can find the most optimal scanner for the classifier.
%     \item The model can be more robust to the noise since the noise in each epoch is different. 
% \end{enumerate}
% % include the gradient method
% As the main problem of this strategy, it is crucial to determine a proper gradient for the stochastic process. In our observation, the score function estimator method was worse than the method in which the gradient of the noise layer was always 1. Though no proof shows the latter is the optimal, it can be considered a lower bound for the ONN's performance.

One key advantage of the ONN is its ability to optimize the masks through back-propagation during training. This dynamic approach allows the model to identify the optimal scanner for the classifier and to become more resilient to noise, as the noise in each epoch is distinct. However, determining a suitable gradient for the stochastic process remains a challenge. In our experiments, we found that using the score function estimator method resulted in inferior performance compared to using a constant gradient of 1 for the noise layer. While we cannot definitively prove that this latter approach is optimal, it serves as a lower bound for the ONN's performance.

% It is observed that the score function estimator method is unstable.

\subsection{Experiments}

==> hardware_pca_onn/sections_2022_Dec_OLD/5_results.tex <==

\subsection{Theoretical Investigation for Null-Prior Reconstruction }

Suppose $\B{I}$ is the identity matrix. Given the noisy photon counts $\tilde{\B{y}}$ and the full-rank mask basis $\B{M}$, we can reconstruct the field of view $\tilde{\B{x}} = \B{M}^{-1} \tilde{\B{y}}$.
Based on Parseval's identity, the covariance matrix of a vector $\B{b}$ is $\B{\Sigma}_{\B{b}\B{b}} = c^2 \sigma^2 \B{I}$ if $\B{b} = \B{W a}$ where $\B{\Sigma}_{\B{a}\B{a}} = \sigma^2 \B{I}$ and 
% $\B{W}$ is $c$ times an orthonormal matrix
$\B{W} \B{W}^\top = c^2 \B{I}$
. For RS, we have $\lambda = \frac{\totphoton}{N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{I}\B{x}, \sigma^2 \B{I})$. Thus, the reconstructed field of view is 
\begin{equation}
    \label{eqn:RS_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{\sigma^2 N^4}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
For HB, we have $\lambda = \frac{\totphoton}{2N^2}$  and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{H}\B{x}, 2\sigma^2 \B{I})$ due to the dual branch trick mentioned in section \ref{sssection:DualBranch}. For $\B{H}^{-1}$, $c = \sqrt{\frac{1}{N}}$. The reconstructed field of view is 
\begin{equation}
    \label{eqn:HB_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{8 \sigma^2 N^3}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
% Therefore, when considering the AWGN model, using the Hadamard matrix can improve the SNR of the reconstructed field of view when $N$ is large.
Therefore, using the Hadamard matrix in the AWGN model can improve the signal-to-noise ratio (SNR) of the reconstructed field of view when the number of elements, $N$, is large. 

When the noise is Poisson distributed, the covariance matrix of the noisy photon counts depends on the choice of $\B{M}$. Suppose $\sigma_j$ is the standard deviation of $\lambda \tilde{y}_j$, the $j_\text{th}$ measured noisy photon counts. For the RS, we have $\sigma_j^2 = \lambda x_j$ and $\lambda = \frac{\totphoton}{N^2}$. The covariance matrix of the reconstructed field of view is thus 
\begin{equation}
    \label{eqn:RS_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{N^2}{\totphoton}\diag\{x_1, x_2, \cdots, x_N\}
    \end{aligned}.
\end{equation}
% For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$ by the Skellam Distribution in section \ref{sssection:DualBranch}. Since Hadamard matrices only includes $\pm 1$ entries, we further have $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$ and the covariance matrix  

In the case of the HB, we can express the rate parameter $\lambda$ as $\lambda = \frac{\totphoton}{2N^2}$, as demonstrated in section \ref{sssection:DualBranch} using the Skellam Distribution. Additionally, we can express the variance of each element in the sum as $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$. As Hadamard matrices only contain entries of $\pm 1$, this reduces to $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$. Using this information, we can construct the covariance matrix
\begin{equation}
    \label{eqn:HB_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{2N \sum_{k=1}^N x_k}{\totphoton}  \B{I}
    \end{aligned}.
\end{equation}
% Therefore, the mean squared error (MSE) of HB is 2 times that of RS under Poisson noise. This factor of 2 arises from the dual branch trick. In other words, HB can never exceed RS in reconstruction error even when measuring with 2 PMTs simultaneously.
The results of our analysis reveal that the mean squared error (MSE) of the HB method is twice that of the RS method when the noise is Poisson distributed. This difference is attributed to the dual branch trick utilized in the HB method. Despite the use of two PMTs in the HB method, it is unable to surpass the reconstruction error of the RS method. These findings demonstrate the limitations of the HB method in comparison to the RS method under Poisson noise conditions.

\subsection{Simulated Results}


==> hardware_pca_onn/sections_2022_Dec_OLD/custom_sty.tex <==
% re-define the equation environment
\let\oldequation\equation%
\let\endoldequation\endequation%
\renewenvironment{equation}%
  {\linenomath\oldequation}{\endoldequation\endlinenomath}%
\expandafter\let\expandafter\oldequationstar\csname equation*\endcsname%
\expandafter\let\expandafter\endoldequationstar\csname endequation*\endcsname%
\renewenvironment{equation*}%
  {\linenomath\oldequationstar}{\endoldequationstar\endlinenomath}%

\newcommand{\B}{\mathbf}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IZ}{\mathbb{Z}}

\newcommand{\diag}{\text{diag}}

\usepackage{subcaption}

\newcommand{\totphoton}{\mathfrak{N}}
\newcommand{\photon}{\mathfrak{n}}

\newcommand{\totexposure]}{\mathfrak{T}} %total expo time
\newcommand{\exposure}{\mathfrak{t}} %expo time for each mask

==> hardware_pca_onn/sections_2022_Dec_OLD/include.tex <==
%% SET PAPER TITLE HERE
% \newcommand{\papertitle}{Single-Pixel Computer Vision in Low-Light}
% \newcommand{\papertitle}{Single-Pixel Computer Vision under Poisson Noise}
% \newcommand{\papertitle}{Single-Pixel Inference under Poisson Noise}
% \newcommand{\papertitle}{When does optical coding improve performance of single-photon cameras?}

\newcommand{\papertitle}{Coded Imaging under Poisson Noise}

%% Additional packages included, and also any commands defined
\usepackage{enumitem,kantlipsum}

\usepackage{siunitx}

% Fun colors to use: https://en.wikibooks.org/wiki/LaTeX/Colors
\usepackage[dvipsnames]{xcolor} 
% \hypersetup{colorlinks,linkcolor={blue},citecolor={RoyalBlue},urlcolor={red}} 
\newcommand{\rnote}[1]{\textcolor{red}{#1}}
\newcommand{\bnote}[1]{\textcolor{blue}{#1}}
%\newcommand{\rnote}[1]{{\begin{color}{red}#1\end{color}}}
%\newcommand{\bnote}[1]{{\begin{color}{blue}#1\end{color}}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newenvironment{myenum}
{ \begin{enumerate}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}     }
{ \end{enumerate}                } 

\newenvironment{myitem}
{ \begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}     }
{ \end{itemize}                } 


\def\E{\mathsf{E}}
\def\Var{\mathsf{Var}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

\newcommand{\taud}{\tau_\text{d}}

\newcommand*{\nolink}[1]{%
  {\protect\NoHyper#1\protect\endNoHyper}%
}

% customized styles
\input{\homedir/sections/custom_sty}

==> hardware_pca_onn/sections_2023_Dec_OLD/0_abstract.tex <==
% Abstract Single-pixel computer vision under poisson noise

 Optical coding is widely used in the design of computational imaging systems. While most coding approaches are developed with additive Gaussian noise models, most real optical imaging systems noise is dominated by Poisson noise due to light quantization. It has been observed in previous studies that code performance varies significantly between these two noise models. Therefore the design of an imaging approach, including the derivation of suitable codes, lenses, or cameras should take into account Poisson noise. In this work, we use the single pixel camera as a toy model to derive \Xpolish{capture strategies}{coding scheme} that are feasible in Poisson noise limited environments. While our work has implications for all optical vision systems, we focus on a system designed for highly compressive tasks like character recognition where the effect of Poisson noise is most apparent. We show that in such a case, our optimized capture approach can approach the performance of an ideal full resolution camera.

==> hardware_pca_onn/sections_2023_Dec_OLD/1_intro.tex <==
\input{\homedir/sections/1_intro/1_intro_2024_01_03.tex}

==> hardware_pca_onn/sections_2023_Dec_OLD/1_intro/1_intro.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

% Coding is a fundamental technique used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance. For applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging, coding enables a low dimensional sensor to sample in a \textbf{complete} measurement space.
% %an $n$-dimension measurement space.
% Due to its range of applications, coding schemes have been investigated thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise. It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under the AGN. This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 

% In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.

% Coding is a widely-used technique in computational imaging (CI) that aims to improve image quality and reduce the dimensionality of the measurement space \cite{cossairt2012does}. It has been shown to be effective in a variety of applications, including single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging. These techniques rely on coding to allow low-dimensional sensors to sample a complete measurement space. While coding schemes have been widely studied, most research has focused on low noise scenarios or additive Gaussian noise models. This is due to the fact that additive Gaussian noise, which is introduced by imperfections in cameras and sensors, is easy to model both analytically and computationally as it is a signal-independent linear noise.

\IEEEPARstart{A}{}n imaging device performs a projection from a high-dimensional scene space onto a lower-dimensional reconstruction space. The need for the projection stems partially from a need to reduce and interpret the data, either as a human-interpretable image or as some form of pattern yielding actionable information about the scene. In addition, especially when imaging with visible light, a projection reduces the information to an amount that can be digitized by a camera sensor and processed. Camera sensors are two-dimensional and capture the absolute value squared of the light wave averaged over pixels in space, time, wavelength, and polarization. The projection onto a sensor prior to digitization is thus a fundamental and essential component of any imaging and vision device for physical and computational reasons. One quite general way to model this projection process is through what is commonly referred to as coding or multiplexing. 

\Xhide{\bnote{insert an eqn about the symbols mentioned below}}

Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. \YLnote{The \textbf{single-pixel-imaging} technique is considered as a typical example of this model.} Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x}
    \end{aligned}
\end{equation}
, where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is a set of sensing masks\Xhide{or in other words, weighing design (WD) \cite{harwit1979hadamard} \bnote{not sure if language from 1979 is useful. I have not heard of weighing design},} linearly projecting the field of view onto the sensor pixels, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured \YLnote{flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts.


A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does}\Xhide{\bnote{Define coding here?}} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.

%\rnote{Coding is accomplished by blocking photons over time or space, and more details about the scene can be preserved consequently \cite{raskar2009computational}}. In addition to increasing light throughput, coding can reduce the dimensionality of the measurement space, which is a common metric for the performance of a CI method. Coding allows low-dimensional sensors to sample a complete measurement space in applications such as single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, and polarization imaging.

% \bnote{This paragraph reads choppily. Many of the sentences could be blended together/ reorganized to be smoother. Potentially combine this with the following paragraph.} While coding schemes have been extensively researched, the mathematical foundation is based on low noise scenarios or Additive Gaussian noise (AGN) models. This is because the AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurements in noisy cameras and sensors, and is easy to analyze and compute analytically as it is signal-independent and linearly additive.

Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 

Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation~\ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not effective under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson}.

\YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
%Previous research has shown that coding behaves differently under Poisson noise compared to AGN \cite{duarte2008CS, harwit1979hadamard, neifeld2003FSI}. Existing coding and computational imaging techniques may not be applicable to these sensors, which makes developing new coding techniques a crucial task. 

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{In this project, we use the popular a single pixel camera design to analyze and design effecive coding models under Poisson noise. Similar to the conclusion of Cossairt et al., Harwid et. al., and Swift et. al., and Willett et. al. we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $M$ \YLnote{\cite{cossairt2012does, harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}.
We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. We propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. 
%This is opposed to compressive sensing strategies, where data is projected into a sparse basis after capture. SS coding strategies can provide a significant improvement on downstream tasks such as correlation analysis and classification in the presence of Poisson noise.
This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of noise on downstream analyses.}

% However, as optical imaging technologies improve, readout noise is decreasing and Poisson noise, due to the quantized nature of light, is becoming more dominant in measured imaging data \bnote{Mention the sensors that make this capable here? By combining with the previous paragraph it could also be made more clear the Poisson noise breaks the underlying assumptions of coding derivations. Mention that the signal-dependent property of Poisson noise is a key factor in why these proofs break down.} \rnote{For instance, Single-photon Avalanche Diode (SPAD) and Photon Multiplier Tube (PMT) are two typical sensors}. Poisson noise is a fundamental physical property of light and arises from the discrete nature of light. An optical signal is composed of discrete photons that can not be arbitrarily divided across codes. Therefore, in state-of-the-art and future sensors measuring visible light, it is important to consider measurement and processing techniques under Poisson noise.

% Previous research has shown that coding behaves substantially differently under Poisson noise compared to the AGN \cite{duarte2008CS}, which is particularly significant in emerging single-photon sensors that only experience Poisson noise. \bnote{Talk more about why Poisson noise is hard to code here.} \rnote{Coding is challenging in this case as it is impossible to remove the Poisson noise without eliminating some of the signal \cite{harwit1979hadamard}}. This means that existing coding and computational imaging techniques may not be applicable to single-photon or "few-photon" sensitive sensors (such as most state-of-the-art CMOS and machine vision cameras) where readout noise is on the order of just a few photons \cite{harwit1979hadamard}.

Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network.
\end{itemize}

While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.

% \bnote{Should we add the example 4-pixel problem and a teaser figure here?}\ynote{I think that makes most sense in the context of compressed sensing. We could add it to the discussion or leave it for the talk.}

\iffalse
\textbf{New paper story:}
\begin{enumerate}
    \item Coding is one of the fundamental techniques used in computational imaging (CI) for image quality improvement \cite{cossairt2012does}. On top of increasing the light throughput, coding reduces the dimensionality of a measurement space where the reconstruction accuracy is a usual metric for the CI's performance.\bnote{Insert definition of computational imaging, probably similar to the one of \cite{cossairt2012does}}.
    \item 
    Coding is important in any application where an n dimensional measurement space is sampled with a sensor or dimensionality $<$ n. It is relevant in single pixel imaging, spectroscopy, structured illumination imaging, time of flight imaging, polarization imaging, computational imaging, and compressed sensing.
    \item Due to its range of applications coding schemes have been explored thoroughly. Most implementations, however, are using very low noise scenarios or additive Gaussian noise models. The rationale is that additive Gaussian noise is a good model for the readout noise introduced by the imperfect measurement of cameras and sensors. This AGN is easy to model analyticlly and computationally since it is a signal independent linear additive noise. 
    \item As optical imaging technologies improve, readout noise is decreasing and Poisson noise to to the quantized nature of light is dominating measured imaging data. While readout noise is a technical problem introduced by an imperfect measurement, quantization noise is a fundamental physical property of light. In other words, since light is actually composed of photons that hit the sensor at discrete times, the light flux property we are trying to measure and compute on exists only as an ensemble average over a Poisson distribution and is not in that sense a "real" quantity. \item In state of the art and future sensors measuring visible light, it is therefore important to consider measurement and processing techniques under Poisson noise.
    \item It has been shown in multiple foundational publications, that coding behaves fundamentally different under Poisson noise than it does under AGN.
    % \item For example, recent work explored the regimes where coding/computational imaging can lead to improved performance \cite{cossairt2012does}. The conclusion of their analysis was that coding/computational imaging can improve performance in scenarios where the dominant noise source is due to Gaussian noise often associated to read-out noise. However, when the dominant noise source is Poisson noise, due to the random arrival of photons, the performance gains are negligible. In other words: In a Poisson noise limited measurement, the best "code" is the trivial "pinhole" code, where each sample is scanned on it's own. 
    % \item Beccas paper.
    \item This problem becomes particularly pronounced in emerging single-photon sensors that only suffer from Poisson noise. Therefore, the previous conclusion would imply that existing techniques of coding/computational imaging are not applicable  single-photon or "few-photon" sensors (i.e. sensors where the readout noise is on the order of just a few photons, such as most state for the are sCMOS and machine vision cameras). 
    \item In this paper we analyze the performance of coding techniques using simple toy applications, compare the behavior of popular approaches for AGN and Poisson noise and develop coding strategies that work with Poisson noise. 
    \item Similar to \cite{cossairt2012does} we find that coding has negligible performance gains when the task is \textit{image reconstruction}. However, when performance gain is measured for downstream tasks, coding with codes that are adapted to the downstream tasks can provide non-trivial performance gains and in some cases recover the performance of an optimal measurement performed with a high dimensional sensor.
\end{enumerate}
\fi

\iffalse
\subsection{Outline (for planning only)}
Definition of coding, sensor dimensionality, measurement dimensionality

definition of signal reconstruction, imaging, and pattern recognition

\bnote{Single-pixel imaging.} 

\bnote{Compressive sensing} Compressive sensing has enabled the design of single-pixel imaging systems that are able to reconstruct images from very few measurements. 
These systems are useful in applications where it is expensive to have pixel arrays that sample the full image in parallel. 
For example in low-light applications, PMTs are commonly used, and it is expensive to build arrays of PMTs.

Additionally, compressive sensing can also be applied to other imaging modalities such as hyper-spectral imaging,  fluorescence imaging etc... 

\bnote{Signal reconstruction under Poisson noise.}\ynote{same as before. Shouldn't talk about comprehensive sensing here. Everything we have talked about before is about signal reconstruction} The most efficient compressive sensing systems have been implemented for signal reconstruction under Gaussaian noise. 
Unfortunately, compressive sensing in the presence of Poisson noise does not benefit from the same low-sample complexity \cite{raginsky2011performance}.
This is due to XXX


\bnote{Signal reconstruction amplifies (\rnote{may not necessarily}) noise so we should skip it.} 
Signal reconstruction, however, is often an intermediate step. 
The final goal is often to execute a high-level task such as classification or segmentation.
To this end, current computer vision systems extract features from the reconstructed signal and use these features to accomplish the task at hand.
In this paper, we find that in a single-pixel imaging system under Poisson noise, it is sub-optimal to reconstruct from compressive measurements and then extract features.
This is because the signal reconstruction step amplifies noise.

\bnote{Task Specific Masks vs General Masks}
Should we adapt our masks based on our objective (pattern recognition task, image reconstruction domain, different types of signals)? The conventional wisdom for AGN is that that doesn't help much. 

Now we need to do analysis:
define toy problems, discuss performance for simple adaptive masks
conclusion: with Poisson noise signal reconstruction makes no sense. But pattern recognition works with an adapted mask set.

How do we find the masks:
PCA, ONN

\bnote{Optical neural nets to the rescue.} 
Inspired by recent trends in optical neural networks, we propose a single-pixel vision system for low-light applications. 
By capturing image features directly we avoid amplifying noise

\bnote{How to design these masks.} 

Discussion:
end to end computational imaging with adaptive asks works under Poisson noise.

This provides an additional motivation for proposed optical ANNs or ANNs with optical layers. Such an architecture allows me to choose where in the design I want to add the Poisson noise.

Possibly: Quantum mechanics interpretation.
\fi

==> hardware_pca_onn/sections_2023_Dec_OLD/1_intro/1_intro_2023_11_30.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi



\IEEEPARstart{I}{}n imaging devices, a crucial step involves projecting information from a high-dimensional scene space onto a lower-dimensional reconstruction space. This projection serves the dual purpose of data reduction for human interpretation and the extraction of actionable patterns pertaining to the scene. Information from a 3D scene involving color, timing, polarization, and phase has to be encoded on a 2 dimensional image sensor. This process, often termed coding or multiplexing, is a fundamental and essential aspect of both physical and computational considerations in imaging and vision devices.

Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. The \textbf{single-pixel-camera} is considered as a typical example of this model. Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view (FOV), $\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts.

In this work we will study the performance of this camera for different choices of $\B{M}$ under different noise models. The single pixel camera is intended specifically as a toy model that exhibits the more general dimensional reduction problem experienced by all imaging devices. Our goal is to design $\B{M}$ such that it allows us to extract desired information from the scene when combined with digital processing. In other words, we seek to design an end to end vision system and consider both the physical and the digital part of the design. While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.


%A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.



% Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 
Coding schemes, often developed under signal independent Additive Gaussian Noise (AGN), provide a mathematically tractable framework. While AGN is suitable to model certain types of noise introduced by the measurement device, it does not correctly model Poisson noise which is signal-dependent. In almost all modern cameras and sensors, however, Poisson noise is predominant, especially in advanced sensors like Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}.  This necessitates a reevaluation of coding strategies tailored to this noise type.

% Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation \ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not recommended under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Poisson noise, a fundamental property of light, arises due to the discrete nature of light measurements. Unlike the assumptions of the linear model in Eq.  \ref{eqn:NoiselessMeasurement}, it's impossible to distribute a photon measurement across all open pixels in a mask. Consequently, the measurements $\B{y}$ called for by the equation are unattainable by linear reconstruction approaches. This renders coding and compressed sensing approaches, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. The optimal code, denoted as $\B{M}_P$, for measurements limited by real Poisson noise must converge to $\B{M}_G$ applicable to the optimal code under Additive Gaussian Noise (AGN) or under no noise as the number of measured photons tends toward infinity. However, it is crucial to highlight that, as demonstrated below, $\B{M}_P$ does not necessarily exhibit similarity to $\B{M}_G$ for any finite number of photons.

\AVnote{\checkednote{The optimal code $\B{M}_P$ for a real Poisson noise limited measurement has to approach the $\B{M}_G$ for a noise-less measurement or one under AGN as the number of measured photons goes to infinity. Crucially, however, as we will show below $\B{M}_P$ does not become similar to $\B{M}_G$ for any finite number of photons.}}

% \YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
\Xhide{
\Xpolish{In most of the papers, people optimize the algorithms on reconstruction but keep using random coding \cite{goyal2016performance}. Some other work, such as Feature Specific Imaging (FSI) does optimize the sensing matrices based on some learn-able priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, but how to optimize masks under Poisson noise remains an unsolved problem \cite{neifeld2014optimizing}. Meanwhile, some attempts on matrix optimization based on minimal mutual coherence are not based on Poisson noise model itself \cite{mordechay2014matrixRIP} and is proved defective in this paper.}
{
\AVnote{this seems like it belongs into related work}
In many papers, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}  \YLnote{need more here}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methids explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}
}

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{In this project, we use the popular single pixel camera design to analyze and design effective coding models under Poisson noise. Similar to the conclusion of Cossairt et al., Harwid et. al., and Swift et. al., and Willett et. al. we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $\B{M}$ \YLnote{\cite{cossairt2012does, harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}.
We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. We propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of noise on downstream analyses.}



Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel cameras.}
\end{itemize}

\Xpolish{While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.}
{
Our work, although rooted in compressed sensing principles applicable to regularized image reconstruction, specifically addresses two extreme scenarios. The first involves non-compressible data with full-rank measurements, reconstructed without regularization. Conversely, we examine highly compressible data in image classification, projecting images into a minimal feature space where the impact of Poisson noise becomes particularly evident.}
\AVnote{\checkednote{Add a figure showing different vision tasks with different compressibilities}}





==> hardware_pca_onn/sections_2023_Dec_OLD/1_intro/1_intro_2024_01_03.tex <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi



\IEEEPARstart{I}{}n imaging devices, a crucial step involves projecting information from a high-dimensional scene space involving color, timing, polarization, and phase onto a lower-dimensional reconstruction space. This projection serves the dual purpose of data reduction for human interpretation and the extraction of actionable patterns pertaining to the scene. This process, often termed coding or multiplexing, is a fundamental and essential aspect of both physical and computational considerations in imaging and vision devices. 
In this project, the primary objective is to optimize coding schemes, with a particular emphasis on selecting the appropriate noise model.

\Xhide{Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. }The \textbf{single-pixel-camera} demonstrated in Fig.\ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}. Supposing the image of the field of view (FOV) consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ projections, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts \cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-ranked, this model accurately characterizes conventional single-pixel imaging scenarios. However, even when $m < N$, the model remains effective through the integration of regularization techniques, specifically compressed sensing.

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct measurement strategy (Raster scan)}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational imaging strategy (Basis scan)}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

In this work we will study the performance of this camera for different choices of $\B{M}$ under different noise models. \Xhide{The single pixel camera is intended specifically as a toy model that exhibits the more general dimensional reduction problem experienced by all imaging devices. Our goal is to design $\B{M}$ such that it allows us to extract desired information from the scene when combined with digital processing. In other words, we seek to design an end to end vision system and consider both the physical and the digital part of the design. }While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.


%A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.



% Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 
Coding schemes, often developed under signal independent Additive Gaussian Noise (AGN), provide a mathematically tractable framework. While AGN is suitable to model certain types of noise introduced by the measurement device, it does not correctly model Poisson noise which is signal-dependent and not avoidable via better sensor fabrication techniques. \Xhide{In almost all modern cameras and sensors, however, Poisson noise is predominant, especially in advanced sensors like Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}.  }This necessitates a reevaluation of coding strategies tailored to this noise type.

% Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation \ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not recommended under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Poisson noise, a fundamental property of light, arises due to the discrete and random nature of light measurements. Unlike the assumptions of the linear model in Eq.  \ref{eqn:NoiselessMeasurement}, it's impossible to distribute a photon measurement across all open pixels in a mask. Consequently, linear reconstruction approaches based on the measurements $\B{y}$ called for by the equation are \Xpolish{unattainable}{unsatisfactory}\Xhide{ by linear reconstruction approaches}. This renders coding and compressed sensing approaches\YLnote{\checkednote{more about  compressed sensing}}, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. \Xhide{The optimal code, denoted as $\B{M}_P$, for measurements limited by real Poisson noise must converge to $\B{M}_G$ applicable to the optimal code under Additive Gaussian Noise (AGN) or under no noise as the number of measured photons tends toward infinity. However, it is crucial to highlight that, as demonstrated below, $\B{M}_P$ does not necessarily exhibit similarity to $\B{M}_G$ for any finite number of photons.}

\AVnote{\checkednote{The optimal code $\B{M}_P$ for a real Poisson noise limited measurement has to approach the $\B{M}_G$ for a noise-less measurement or one under AGN as the number of measured photons goes to infinity. Crucially, however, as we will show below $\B{M}_P$ does not become similar to $\B{M}_G$ for any finite number of photons.}}

% \YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
\Xhide{
\Xpolish{In most of the papers, people optimize the algorithms on reconstruction but keep using random coding \cite{goyal2016performance}. Some other work, such as Feature Specific Imaging (FSI) does optimize the sensing matrices based on some learn-able priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, but how to optimize masks under Poisson noise remains an unsolved problem \cite{neifeld2014optimizing}. Meanwhile, some attempts on matrix optimization based on minimal mutual coherence are not based on Poisson noise model itself \cite{mordechay2014matrixRIP} and is proved defective in this paper.}
{
\AVnote{this seems like it belongs into related work}
In many papers, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}  \YLnote{need more here}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methids explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}
}

\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{\Xhide{In this project, we use the popular single pixel camera design to analyze and design effective coding models under Poisson noise. } Therefore, we propose a coding methodology called \textbf{Selective Sensing} (SS) that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time. This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of Poisson noise on downstream analyses.}



Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Harwit et. al. \cite{harwit1979hadamard}, and Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $\B{M}$ {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extract the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel cameras.}
\end{itemize}

\Xhide{\Xpolish{While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.}
{
Our work, although rooted in compressed sensing principles applicable to regularized image reconstruction, specifically addresses two extreme scenarios. The first involves non-compressible data with full-rank measurements, reconstructed without regularization. Conversely, we examine highly compressible data in image classification, projecting images into a minimal feature space where the impact of Poisson noise becomes particularly evident.}
\AVnote{\checkednote{Add a figure showing different vision tasks with different compressibilities}}}





==> hardware_pca_onn/sections_2023_Dec_OLD/2_related.tex <==
\input{\homedir/sections/2_related/2_related_revised_2}

==> hardware_pca_onn/sections_2023_Dec_OLD/2_related/2_related.tex <==
% \bnote{Don't use the paper start unless it is the large first letter unless it the paper start.... }Multiplexing \bnote{multiplexing has not been mentioned yet. stick with either coding or multiplexing.} %is a method that 

\bnote{Few projects optimize masks for Poisson noise}
\bnote{list how they find the masks for Poisson}


In single-pixel imaging, coding allows the capture of a two-dimensional image with a single-pixel sensor. \bnote{\checkednote{ not constrained to single independent noise just probed for that case.}} Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal} in systems with only additive gaussian noise.
\Xhide{ \bnote{Combine these two sentences?} However, under Poisson noise a trivial raster scan, where one pixel of the mask opens at a time provides the best performance even though it transmits only a small fraction of the light \cite{wuttig2005optimal, harwit1979hadamard, cossairt2012does}.} \checkednote{Previous studies have shown that there is an upper limit to the performance gain of Hadamard multiplexing when Poisson noise is present.} However, incorporating task-specific priors can be beneficial for reconstructions \cite{cossairt2012does, harwit1979hadamard}. \ynote{do these papers really show this? That seems like it is our contribution} \Xhide{\bnote{We are citing mostly just the cossairt2012 paper for all these claims, can we add more citations to the different claims?}. \ynote{Cossairt takes these results from the hadamard transform optics book. We should cite that.}}

% but it is still unclear how to surpass this limit on photon counting systems where Poisson noise is predominant. 



Priors are usually used to enhance the image quality \cite{cossairt2012does, nayer2009prior, Levin2007prior} but the extent of this improvement depends on prior types and masks\Xhide{\ynote{what is imaging coding??}}\cite{cossairt2012does}. Compressed sensing, which utilizes sparsity priors, is a proposed method for improving the reconstruction performance \Xhide{of photon counting systems~\rnote{Is this true?? This seems to be contradicting beccas paper.}}\cite{duarte2008CS}. Nevertheless, the performance attainable under Poisson noise is bounded, significantly lower than under additive gaussina noise, and is heavily influenced by the number of measurements taken and thereby the resolution of the reconstructed image\cite{willet2009CSPoisson}. As such, compressed sensing is a far more challenging task when the measured data are Poisson distributed \cite{willet2009CSPoisson}. Coding strategies and theoretical frameworks developed for additive Gaussian noise are not necessarily usable under Poisson noise.

\Xpolish{While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}. \Xhide{\ynote}{In many cases the most meaningful way to quantify the quality of the collected imaging data is to apply it to a downstream vision task.} Therefore, we explore 
% alternative metrics that better capture the perceptual features and 
optimal masks for feature specific imaging \cite{neifeld2003dual}. \Xhide{\rnote{FSI doesn't work under Poisson \cite{neifeld2003dual}}}
One inspiring solution is the task-specific imaging via Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training}. Wang et al. \cite{nature2022ONN}\Xhide{\ynote{citation}} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. }
{While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation \cite{davenport2007smashed}. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}. Therefore, we explore 
% alternative metrics that better capture the perceptual features and 
optimal masks for feature specific imaging \cite{neifeld2003dual}. The principal component analysis (PCA) is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. Another inspiring solution is the task-specific imaging via end-to-end optimization such as Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training}. 
\YLnote{This idea was usually implemented without considering Poisson noise \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training} or training under Poisson noise \cite{tseng2021differentiable, diamond2021dirty, rego2022deep}. Rego et. al froze the sensing matrix as a pinhole without optimizing it.}
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. }
% Wang et al. reported a successful implementation of a neural networks model on optical device for handwritten numbers classification with limited photon budget \cite{nature2022ONN}, which gives a inspiring example in searching task-specific optimal coding scheme for the CI with the assistance of AI .
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked from a set of hyper-parameter combinations \cite{nature2022ONN}. } 


% \rnote{Our contribution}





% Raginsky et al proved the 

%see
%http://vigir.missouri.edu/~gdesouza/Research/Conference_CDs/IEEE_CVPR_2007/data/papers/0194.pdf

==> hardware_pca_onn/sections_2023_Dec_OLD/2_related/2_related_revised.tex <==
\textbf{Single Pixel Imaging}. In single-pixel imaging, coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal} in systems with only additive gaussian noise.

\textbf{Imaging Priors}. Priors are usually used to enhance the image quality \cite{cossairt2012does, nayer2009prior, Levin2007prior} but the extent of this improvement depends on prior types and masks \cite{cossairt2012does}. 

\textbf{Compressed Sensing}. Compressed sensing, which utilizes sparsity priors, is a proposed method for improving the reconstruction performance \Xhide{of photon counting systems~\rnote{Is this true?? This seems to be contradicting beccas paper.}}\cite{duarte2008CS}. Nevertheless, the performance attainable under Poisson noise is bounded, significantly lower than under additive gaussina noise, and is heavily influenced by the number of measurements taken and thereby the resolution of the reconstructed image\cite{willet2009CSPoisson}. As such, compressed sensing is a far more challenging task when the measured data are Poisson distributed \cite{willet2009CSPoisson}. Coding strategies and theoretical frameworks developed for additive Gaussian noise are not necessarily usable under Poisson noise.

\textbf{Non-reconstruction classification}. While image reconstruction is a common task performed by an optical imaging system, it is often an intermediate step for performing downstream computer vision tasks such as classification or segmentation \cite{davenport2007smashed}. Extracting features from reconstructed signals is sub-optimal compared to direct linear feature extraction during measurements \cite{neifeld2003FSI}, and the extracted features hardly improve the reconstruction \cite{neifeld2003dual}. Notably, the Mean Squared Error (MSE) is a common metric for evaluating image reconstruction but may not necessarily reflect visual image quality \cite{cossairt2012does, wang2004MSEmetric}.

% \textbf{Metric for imaging}. \YLnote{MSE is not a good metric}

\textbf{Principal Component Analysis}. The principal component analysis (PCA) aims to extract significant features in another orthogonal space \cite{abdi2010PCA}. It is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}.

\textbf{End-to-End optimization}. This method refers to training hardware and software networks for image processing pipelines \cite{diamond2021dirty, zhang2021deep}. \Xhide{One typical archetecture is Optical Neural Networks \cite{nature2022ONN, spall22hybrid_training, caulfield1989ONN}.} \YLnote{In many previous projects, this idea was usually implemented without considering Poisson noise \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training} or without optimizing masks under Poisson noise \cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN}. Rego et al. froze the sensing matrix as a pinhole without optimizing it \cite{rego2022deep}}
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. 
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked from a set of hyper-parameter combinations \cite{nature2022ONN}. } 

==> hardware_pca_onn/sections_2023_Dec_OLD/2_related/2_related_revised_2.tex <==
\textbf{Coding under Poisson noise}. In single-pixel imaging, coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal} in systems with only additive gaussian noise. \Xhide{However, when Poisson noise is predominant, we should not use any coding \cite{harwit1979hadamard, cossairt2012does}. When the noise is Poisson distributed, coding with sparse priors such as compresses sensing are not recommended \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}.}
{In many recent projects, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}\YLnote{\checkednote{need more here}}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson,  willett2011poisson, vanden2019various}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methods explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}



% \textbf{Task Specific Imaging}

\textbf{End-to-end optimization}. This method refers to training hardware and software networks for image processing pipelines \cite{diamond2021dirty, zhang2021deep, jacome2023middle}. \YLnote{In many previous projects, this idea was usually implemented without considering Poisson noise \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training, jacome2023middle} or without optimizing masks under Poisson noise during training \cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN}. Rego et. al froze the sensing matrix as a pinhole without optimizing it \cite{rego2022deep}}
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes in CI. 
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked from a set of hyper-parameter combinations \cite{nature2022ONN}. } Our contribution is developing a noise-included training approach within a neural network model to find the optimal masks under Poisson noise.

% \textcolor{blue}{Add section on feature specific imaging}

\textbf{Feature Specific Imaging}. Feature-specific imaging is a type of imaging system that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it \cite{neifeld2003FSI, neifeld2003dual}. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}. This technique can be viewed as a variant of compressed sensing, wherein the sensing matrix is determined based on prior information \cite{neifeld2014optimizing}. Nevertheless, its performance and implications under Poisson noise conditions remain relatively unexplored in the existing literature, warranting further discussion and investigation.


\iffalse

\YLnote{For the feature specific imaging, here are some paper to cite}

\YLnote{yizhou notes start}
\textbf{Mark A. Neifeld and Premchandra Shankar, "Feature-specific imaging," Appl. Opt. 42, 3379-3389 (2003)} Feature-specific imaging is a type of imaging system that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features.  Poisson noise when the mean and variance of the photon count are equal. The paper shows that feature-specific imaging does not provide any advantage over conventional imaging in the presence of shot noise, because the shot-noise-limited SNR is inherent in the irradiance collected by the instrument and does not depend on the energy incident on any particular detector. Therefore, we can infer that feature-specific imaging would not work well with Poisson noise either, unless the mean and variance of the photon count are very different. \YLnote{However, that is where we come up with hardware PCA. We can then further reduce the text by citing Neifeld for the PCA part. }

\textbf{Abhijit Mahalanobis and Mark Neifeld, "Optimizing measurements for feature-specific compressive sensing," Appl. Opt. 53, 6108-6118 (2014)} "Although our analysis assumes that the noise is independent of the signal, this is not the case when Poisson noise is present. While a formal treatment of the effects of signal-dependent noise is beyond the scope of the paper, we compare the behavior of optimized masks to the normalized PCA in signal-dependent noise." It also has imcomplete future work "Other types of noise models will also be considered, such as signal-dependent shot noise." It seems it hasn't been studied after this paper. We could say that our contribution is designing a method to extend feature specific imaging in poisson noise model.

\YLnote{Interesting conclusions listed below}  

"FSI is a form of CS in which the measurement kernels are not random, but are based on prior knowledge of the information we are interested in sensing. Working in this FSI framework, we have developed a methodology for designing a set of masks that satisfy the photon constraint and are optimum for making measurements that minimize the reconstruction MSE in the presence of noise. "

"Of course, the primary reason for CS is to make fewer measurements than the number of pixels in the reconstructed image, and to collect the information more efficiently than a conventional image. One might intuitively expect that utilizing more features (or measurements) in the reconstruction process will yield a smaller reconstruction error. We demonstrated, however, that the photon constraint limits the number of masks that can be used at a particular SNR to reduce the reconstruction MSE. In noisy conditions, the MSE initially decreases as the number of measurements is increased, but then increases when measurements that contain more noise than signal information are included." \YLnote{It aligns with Rebecca's work.}

\textbf{W. Van den Broek, B. W. Reed, A. Béché, A. Velazco, J. Verbeeck and C. T. Koch, "Various Compressed Sensing Setups Evaluated Against Shannon Sampling Under Constraint of Constant Illumination," in IEEE Transactions on Computational Imaging, vol. 5, no. 3, pp. 502-514, Sept. 2019, doi: 10.1109/TCI.2019.2894950.}  show that for the investigated sensing matrices and in the absence of read-out noise, i.e. with only Poisson noise present, compressed sensing does not raise the amount of Fisher information in the recordings above that of a Shannon sampled signal.





\YLnote{yizhou notes end}

\ynote{andreas notes start}
Other refrerences:
M. Mordechay and Y. Y. Schechner, "Matrix optimization for poisson compressed sensing," 2014 IEEE Global Conference on Signal and Information Processing (GlobalSIP), Atlanta, GA, USA, 2014, pp. 684-688, doi: 10.1109/GlobalSIP.2014.7032205.
“Considering that the measurements are noisy, it is important to
avoid energy loss, since measurements with low energy have low
signal-to-noise ratio (SNR).”
We prove this assumption wrong in this paper ... \YLnote{ONN reconstruction}

Photon-noise: is a single-pixel camera better than point scanning? A signal-to-noise ratio analysis for Hadamard and Cosine positive modulation, Camille Scotté, Frédéric Galland1 and Hervé Rigneault
Published 7 June 2023 • © 2023 The Author(s). Published by IOP Publishing Ltd
Journal of Physics: Photonics, Volume 5, Number 3 Citation Camille Scotté et al 2023 J. Phys. Photonics 5 035003 DOI 10.1088/2515-7647/acc70b
Looking at SNR for different codes. Mostly confirms prior results. Finds that snr is improved for brightest pixels, but degraded for others. \YLnote{Only $x_i \ge k \bar{x} = \frac{k\sum_{j=1}^N x_j}{N}$ can get improved. $k$ is usually $2, 4, 16$, which means only bright pixels get reconstruction gain. E.g. cosmophotography. For normal images, that usually means the general performance degrades!}

D. Shin, J. H. Shapiro and V. K. Goyal, "Performance Analysis of Low-Flux Least-Squares Single-Pixel Imaging," in IEEE Signal Processing Letters, vol. 23, no. 12, pp. 1756-1760, Dec. 2016, doi: 10.1109/LSP.2016.2617329.
Finds bounds for noise. Probably agrees with paper above.
This is very interesting. AT very low rates the non negativity constraint can improve our estimate for multiplexing so it may become better than poisson. The paper doesn’t prove that it is better. Just says the proof for the general case is not valid and shows an experiment where an improvement is shown. Could we use the same constraint in convex optimization? What does this say about other constrained or regularized optimizations?
\ynote{andreas notes end}


\iffalse
better arrangement
coding under Poisson: mention hadamard book, ollie and becca's paper show that coding under Poiss is not ideal
mask optimization: people optimize the masks under wrong noise model, we proposed a better way for Poiss 

\fi


\YLnote{In summary, we can have a list of literature by their category
\begin{enumerate}
    \item Open more pixels doesn't help under Poisson noise (no compression): \cite{harwit1979hadamard, neifeld2003FSI, cossairt2012does, scotte2022photon_noise}
    \item Regularization doesn't help (usually comes with compression):
    \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}. Their suggestion is to use fewer measurements as more measurements give rise to a greater reconstruction error upper bound. BTW, ONN are can have many measurements with low rank, which doesn't contradict to this conclusion.
    \item Feature specific imaging is designed for gaussian noise especially. It is a good way for feature preserving and reconstruction. No follow-up about the poisson. That is why we start this project.
    \item When doing a classification task, we give some higher compression by labelling. E.g, gender recognition. We only need one mask to tell the gender in the most ideal case. \textbf{It will be good to find some paper directly saying this.} As the data can be highly compressible, we can avoid dense measurements, and thus have lower error bound. Reconstruction is just a linear operation, so it doesn't matter a lot if we use Rebecca's conclusion about the upper bound, even though it is for reconstruction. 
        \begin{itemize}
        \item Think about reconstructing an image about the night sky. After using TV \textbf{re-binning}, we have two colors, black for background, and white for stars. It can be treated as a classification task as well! That is why rebecca proposed some algorithms with TV stuff: to minimize the possible amount of measurements.
    \end{itemize}
    Neifeld uses features learned from training data to do reocnstruction, that is how our idea of directly classification comes from. If we want to apply the ONN for reconstruction, it may be useful to read "RecDNN: deep neural network for image reconstruction from limited view projection data"
\end{enumerate}
}
\fi


\AVnote{\checkednote{Regularization, CS, might help but noise bounds are very unfavorable (cite becca). \\ In most of the papers, people optimize the algorithm. In only very few people try to optimize the masks. No paper where masks are optimize with poisson noise. \\ In this paper we are looking at how to optimize the measurement under poisson noise. \\ We find that optimizing the measurement can have profound improvements to the performance of single pixel vision approaching the perfonance of ideal mutipixel cameras in particular for Poisson noise dominated signals like visible light. }}




==> hardware_pca_onn/sections_2023_Dec_OLD/3_background.tex <==
\AVnote{\checkednote{this paragraph has no new information. probaply can be removed}}
\Xhide{\Xpolish{In this work we study the coding problem by considering the single pixel camera as a specific implementation. This system provides a well studied example of coding and is therefore a good toy model to work with. Our findings, however are general and should apply to any form of coding. In this section, we describe some implementation details in our work\ynote{can mention spectral simulations if they are included}}
{In this study, we investigate the coding problem with a specific focus on the single-pixel camera as an illustrative implementation. This system serves as a well-established paradigm for coding, making it an insightful model for our research. Although our exploration is rooted in this particular example, our findings are intended to be of broader applicability, extending to diverse coding forms. In this section, we elaborate on implementation details central to our study.}}

% \Xhide{Our study on coding focuses on the single pixel camera, which serves as a specific implementation that provides a well-studied example of coding. We use this system as a toy model to investigate the problem, but our findings have broader implications and can be generalized to any form of coding.}

\Xpolish{A single-pixel sensor, such as a photon multiplier tube (PMT), is capable of detecting the total number of photons in a measurement but lacks the ability to provide spatial information. In order to obtain this information, a Digital Micromirror Device (DMD) can be used to spatially code the signal. The DMD consists of millions of small tunable mirrors placed at the image plane of the camera objective lens. Each mirror reflects photons photons from a pixel in the image one of two separate detectors. During a measurement, the sensor counts the photons from the DMD
micromirrors, or pixels, that are facing it, providing spatial information about the distribution of photons within the field of view. }
{\Xhide{While a single-pixel sensor like a photon multiplier tube (PMT) can detect the total number of photons in a measurement, it cannot provide spatial information. A single pixel camera uses a Digital Micromirror Device (DMD) located at the image plane of the camera objective lens to code the signal.}}


\subsection{Selection of Sensing Matrix}\label{ssec:selectionofsensingmatrix}

% \YLnote{1. What are sensing matrix 2. their types 3. limitations}



\input{hardware_pca_onn/sections/3_background/model_implementation}





\iffalse
\paragraph{Impulse}
\paragraph{Non-Selective Codes}
Non-selective codes are codes that are not adjusted to the specific sparsity of the dataset. Any general code not generated using the statistics of a representative training set is included in this group. This incudes many codes used in practice today, such as Hadmard patterns and Rademacher Random codes. We also include truncated Hadamard patterns that are popular in compressed sensing. A truncated Hadamard code uses a random subset of the full Hadamard basis.
\paragraph{Selective Codes}
In this work we show that for single photon cameras, codes need to be specifically selected to measure sparse representations of the data. To achieve this we employ PCA codes and ONN generated codes. ...
\fi



\iffalse
Recall the model described by Equation \ref{eqn:NoiselessMeasurement}. \Xpolish{The sensing matrix $\B{M}$ can be generated by either computational or non-computational imaging methods. Their primary difference is that computational imaging requires additional steps of optical coding and computational decoding in order to capture and process the image \cite{cossairt2012does}. Non-computational method, or Raster scan, involves measuring each pixel sequentially \cite{duarte2008CS} and $\B{M} = \B{I}$ which is an identity matrix. On the other hand, computational methods measure a combination of pixels simultaneously and can be further classified based on the type of mask used.\Xhide{ In this paper, we will arrange the various coding strategies based on their mask generation techniques.
\bnote{consistent language: maybe we should switch "Mask" to "Code" everywhere in the text}} For example, Hadamard matrices composed of $\pm 1$ have been proved as the best coding strategy for reconstruction by Hotelling in 1944 under the AGN \cite{harwit1979hadamard}. A useful feature of computational methods is the compressibility.\ynote{I wouldn't say the methods are compressible. I think what you are trying to say is that computational methods can take advantage of the compressibility of the data.} If the signal is sparse in the subspace of $\B{M}$, it is likely that we only need several vectors of $\B{M}$.}
{\ynote{\checkednote{We distinguish different types of sensing matrixes: A diagonal measurement matrix corresponds to a raster scan where the image is measured pixel by pixel. No computation is required to invert $\B{M}$ and reconstruct the image. We call a measurement with a diagonal $\B{M}$ a non-computational measurement. ...}}\bnote{\checkednote{Is non-computational/computational the best language? Maybe non-coded/coded measurements is more in line with the rest of our language.}  }The sensing matrix $\B{M}$ can be generated using either computational or non-computational imaging methods. The key difference between the two is that computational imaging involves additional steps of optical coding and computational decoding to capture and process the image \cite{cossairt2012does}, while non-computational method, i.e. Raster scan, \ynote{\checkednote{are there other non-computational methods????}}, involves measuring each pixel sequentially \cite{duarte2008CS}. In the case of Raster scan, $\B{M} = \B{I}$, which is an identity matrix. In contrast, computational methods measure a combination of pixels simultaneously and can be further classified based on the type of masks used. For example, Hadamard matrices composed of $\pm 1$ have been shown to be the optimal coding strategy for reconstruction under the AGN \cite{harwit1979hadamard}. A useful feature of computational methods is their compressibility. If the signal is sparse in the subspace of $\B{M}$, it is likely that only a few vectors of $\B{M}$ are needed.}

\fi


\Xhide{\bnote{Use direct measurement / trivial measurement}}

\Xhide{
\begin{enumerate}
    \item Static strategies: 
    Masks are predetermined and fixed. \ynote{aren't they fixed for compressive strategies as well??? Maybe you are trying to distinguish between selective and non-selective masks?}
    \begin{enumerate}
        \item Non-compressible strategies \bnote{(Full rank)}
        \begin{enumerate}
            \item Raster Scan (RS). In this strategy, only one pixel will be scanned in each measurement. Thus, $\B{M} = \B{I}$.
            \item Impulse Imaging (II). II captures the field of view by a pixel array. In this case, each pixel gets $N$ times as much as the exposure time of RS. Mathematically, $\B{M} = N\B{I}$. Alternatively, we can treat it as another RS with $N$ times as many photons. The II works as the baseline for the comparisons with other strategies. 
            \item Hadamard Basis (HB). In this strategy, we choose the 2-D Walsh-Hadamard matrix $\B{H}$ as the mask basis. Hadamard matrices composed of $\pm 1$ has been proved as the best coding strategy \bnote{WD is only mentioned once way earlier, probably better to just change this language.} for reconstruction by Hotelling in 1944 under the AGN.
            \Xhide{\bnote{next part of this sentence is confusing}
            when noise is independent from this signal 
            such as the AGN\cite{cossairt2012does,harwit1979hadamard,wuttig2005optimal}.}
        \end{enumerate}        
        \item Compressible strategies
        \begin{enumerate}
            \item Low-Frequency Truncated Hadamard (LFTH). Given a default Walsh-Hadamard matrix $\B{H}$ and  pick first several rows of it as $\B{M}$. \Xhide{\bnote{switching to low freq}}
            % \item Low-Frequency-Truncated Hadamard (LFTH). Given a default Walsh-Hadamard matrix $\B{H}$ and only keep the first several rows as $\B{M}$.
            % \item Sorted-Truncated Hadamard (STH). Re-order the rows according to their correlation coefficients with the mean of training images. More relevant ones are picked first.
            \item Hardware Principal Components Analysis (HPCA). The DMD displays the PCA components calculated from the training images. \bnote{this learns from data so should maybe go with the ONN? also we should mention this is a novel technique, and give some more explanation to what PCA is}
        \end{enumerate}
    \end{enumerate}    
    \item Selective Sensing\Xhide{Dynamic strategies \bnote{Dynamic is probably not a good name, "dynamic" makes me think the masks will be determined on the fly based on previous measurements}\ynote{Lets use the selective sensing vacabulary here that we introduce in the title.}}: Masks can be optimized based on the tasks.
    \begin{itemize}
        \item Optical Neural Networks (ONN).
    \end{itemize}
\end{enumerate}
}

  
\Xhide{
\rnote{should we ignore the LFTH and STH? And add Compressed sensing}
\ynote{is this really ne distinction we need to make? Key is wether or not we change the mask to adjust to the measurement (selective sensing), or we use a general mask.}
\begin{enumerate}
    \item Null-Prior: RS, II, and HB. It requires no information before measurements.
    % \item Reconstruction-Prior: RTH and LFTH. This prior is from the inductive bias for signal reconstruction that low frequencies components are more robust to noise regardless of the data. % it is wrong if not explaining the LFTH
    \item Reconstruction-Prior: RTH. This prior is based on the fact that the light throughput and SNR in each measurement are greater with fewer masks.
    \item Task-Specific-Prior: STH, HPCA, and ONN. This prior requires the features from training data of a specific task.
    % make plots based on the groups
\end{enumerate}  
\rnote{We now have several results: classification reconstruction plot on MNIST; freeze method; reconstruction on random patterns; what to include?}  \bnote{Reconstruction on random patterns needs to be in the section when we explain the ONN optimizer}
}


%\Xpolish{In this project, we are primarily interested in finding the most optimal one among all common coding strategies. Different from common optimization problems, there are two main physical constraints when optically implementing equation}
%{In this paper, our main objective is to identify the optimal coding strategy among various commonly used methods. However\Xhide{, unlike typical optimization problems}, we face two fundamental physical constraints when implementing the coding strategy optically, as expressed by Equation \ynote{\checkednote{I think any coding method in imaging has these constraints. Probably word it differently.}}}\bnote{\checkednote{Agree to reword. Many optimization and physical problems have constraints no need to overstate the problem, just mentioning that our physical constraints induce the following mathematical constraints may be enough.} }\ref{eqn:NoiselessMeasurement} \cite{neifeld2003dual, willet2009CSPoisson}. 

%\begin{enumerate}
%    \item\label{constraint:photonNumber} \textbf{Flux-preserving} \cite{willet2009CSPoisson}\Xhide{\bnote{Y: Should I use the same term as Rebecca?}}. The single-pixel imaging model involves the allocation of available photons among masks, as discussed in \cite{neifeld2003dual}. It is important to ensure that the mask basis $\B{M}$ does not produce additional photons through improper entries \cite{neifeld2003dual}. Mathematically, $\sup \sum_{i=1}^m M_{ij} = 1, \forall j \in \{1,2,\dots,N\}$ \cite{neifeld2003dual}.\Xhide{\bnote{Include what an improper entry is!} \bnote{A: this is not something we need to mention here. its obvious that the measurements have to be normalized correctly}}
%    \item\label{constraint:negativeEntry} \textbf{Positivity-preserving} \cite{willet2009CSPoisson}. It is not possible to physically implement negative values for the masks $\B{M}$, as demonstrated in \cite{neifeld2003dual, willet2009CSPoisson}. 
%\end{enumerate}




% \subsubsection{Photon Distribution Factor} \label{sssection:PDF}


\subsection{Constraints of sensing matrices} \label{ssection:constraints}

\input{\homedir/sections/3_background/restrictions_of_masks}

\subsection{Model under Noise}

\input{\homedir/sections/3_background/model_under_noise}




==> hardware_pca_onn/sections_2023_Dec_OLD/3_background/model_implementation.tex <==
% \YLnote{1. What are sensing matrix 2. their types 3. limitations}
\Xhide{As a representative technique in the CI, the mathematical underpinning of single-pixel camera is encapsulated by Eq. \ref{eqn:NoiselessMeasurement}. The diverse selections of the sensing matrix $\B{M}$ lead to distinct coding strategies, as elaborated upon subsequently. }

In the realm of the CI, the foundational equation for single pixel imaging is encapsulated in Eq. \ref{eqn:NoiselessMeasurement}. The diverse array of choices for the sensing matrix $\B{M}$ engenders two basic coding strategies, as expounded in Fig \ref{fig:SinglePixelImaging}. However, the process of discerning an optimal $\B{M}$, whether drawn from random matrices or Hadamard matrices, hinges on multifaceted considerations. In the present study, we advocate the notion that the selection of an ideal $\B{M}$ should be contingent upon the requisite prior information pertinent to the tasks at hand. Herein, we delineate various coding types along with their corresponding optimal applications for reference and guidance.

\iffalse
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct measurement strategy (Raster scan)}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational imaging strategy (Basis scan)}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}
\fi
% As a typical CI technique, the mathematical foundation of single pixel imaging follows the equation \ref{eqn:NoiselessMeasurement}. However, the different choices of the sensing matrix $\B{M}$ give rise to different coding types (strategies) introduced later. However, how to select a good $\B{M}$ from random matrices to Hadamard matrices for the Basis scan depends on many factors. In this project, we proposed that the optimal $\B{M}$ should be selected based on the required prior information of tasks we want to complete. The coding types and the most suitable task of each type are listed below for reference.

\subsubsection{Coding Types}

\begin{itemize}
    \item \textbf{Raster scan} entails a pixel-wise scanning approach where photon counts for all pixels are sequentially measured. Mathematically, the sensing matrix $\B{M} = \B{I}$, an identical matrix.      
    
    \item \textbf{Impulse imaging} entails an ideal camera that simultaneously captures complete hyper-spectral data. A prominent instance is a pixel array. When the field of view $\B{x}$ consists of $N$ pixels, the sensing matrix assumes the form $\B{M} = N\B{I}$ where $\B{I}$ is an identical matrix. Each pixel receives $N$ times the exposure in comparison to the raster scan scenario. This technique sets a benchmark akin to a gold standard, serving as an upper limit for the CI performance and an indicator of the noise level for comparison.
    
    \item \textbf{Non-Selective Codes} \Xpolish{are codes that are not adjusted to the specific sparsity of the dataset. Any general code not generated using the statistics of a representative training set is included in this group. This includes many codes used in practice today, such as Hadmard patterns and Rademacher Random codes. We also include truncated Hadamard patterns that are popular in compressed sensing. A truncated Hadamard code uses a random subset of the full Hadamard basis.
    }{encompass coding schemes that lack adaptation to the inherent sparsity of a given dataset. Codes falling within this category are not crafted based on the statistical attributes of a representative training set. This classification encompasses a range of widely used codes, such as Hadamard patterns and Rademacher Random codes, which do not leverage the specific characteristics of the dataset. This grouping also extends to truncated Hadamard patterns, a popular choice in compressed sensing, which employ random subsets of complete Hadamard basis.
    }
    \item \textbf{Selective Codes}.
    \Xpolish{In this work we show that for single photon cameras, codes need to be specifically selected to measure sparse representations of the data. To achieve this we employ PCA codes and ONN generated codes. The principal component analysis (PCA) is a classical method for multispectral data correspondence analysis and classification \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. In this project, the most significant components are computed from the training data and implemented as the hardware masks. Measured photon counts $\B{y}$ are then be feed to a classifier for model optimization. The optical neural networks (ONN) method is like a fully-connected neural networks model but its first layer is used to simulate the sensing matrix $\B{M}$. By properly applying the physical constraints on the first layer, it is possible for this model to find optimal sensing matrix for a given task.}
    {In this study, we elucidate the necessity for the tailored selection of codes in the context of single photon cameras to effectively capture sparse data representations. To address this, we harness both PCA codes and ONN-generated codes. Principal Component Analysis (PCA) serves as a classical technique for analyzing and classifying multispectral data correspondences \cite{rodarmel2002PCA, carr1999PCA, jensen1996PCA, gonzales1987PCA, schowengerdt2006PCA}. Specifically, we compute the most significant components from training data and implement them as hardware masks within this project. The recorded photon counts, $\B{y}$, are subsequently fed into a classifier to optimize the model. The Optical Neural Networks (ONN) approach mirrors a fully-connected neural network model, yet with its first hidden layer simulating the sensing matrix $\B{M}$. By adeptly applying physical constraints to this foundational layer, the model becomes capable of determining the optimal sensing matrix for a designated task.
    }
    
\end{itemize}

\subsubsection{Reconstruction Tasks}
% \paragraph{Null Prior Reconstruction/No Compression}
% \paragraph{Imaging: Weak Prior/Some compression}
% \paragraph{Classification: Strong Prior/Strong compression}
\iffalse
\begin{itemize}
    \item Classic imaging: null-prior/no compression. In this task, the rank of $\B{M}$ is required to be $N$, the number of pixels in the FOV. Therefore, there is no compression when conduct measurements. This case is universal and doesn't require any prior knowledge of the FOV. It can be found in some scenarios such as raster scan. When there is no noise, we can also use full rank Hadamard to reconstruct the FOV. The coding types commonly seen in this kind of tasks are raster scan and non-selective codes.
    \item Image Processing and the Computational Imaging: weak-prior/some compression. This idea comes from some prior knowledge such as signals are sparse in some linear space and noise is concentrated in high frequency domain. One example is the JPEG format of pictures. If we only measure the FOV with low frequency components of the Hadamard matrices, we are working on this task. This type can be found in scenarios such as compressed sensing and image compression. The coding type commonly seen in this kind of tasks is non-selective codes.
    \item Computer vision: strong-prior/much compression. Usually we switch to downstream computer vision tasks such as classification after reconstruct the FOV. However, it is possible to directly capture the principal features by $\B{M}$ if some of its components are similar to the FOV. In this kind of tasks, only a few measurements are needed if we have a strong prior from training data. The coding type involved in this kind of tasks is selective codes.
\end{itemize}
\fi

\begin{itemize}
    \item Classic Imaging (Null-prior/No Compression):
    In tasks involving classic imaging, a null-prior is assumed, and there is no compression during measurements. The rank of the measurement matrix $\B{M}$ is required to be equal to $N$, the number of pixels in the FOV. This scenario, such as in raster scan applications, is universal and does not necessitate prior knowledge of the FOV. Full-rank Hadamard matrices can be employed for reconstruction in noise-free situations. Common coding types for this task include raster scan and non-selective codes.
    \item Image Processing and Computational Imaging (Weak-prior/Some Compression):
    In this kind of tasks, a weak-prior assumption is made, allowing for some compression during measurements. This idea is based on prior knowledge, such as signals being sparse in some linear space, with noise concentrated in the high-frequency domain. An example is the JPEG format. If only the low-frequency components of Hadamard matrices are measured for reconstructing the FOV, this task is engaged. Non-selective codes are typically used for this purpose.    
    \item Computer Vision (Strong-prior/Much Compression):
    Tasks related to computer vision involve a strong prior, enabling substantial compression during measurements. After reconstructing the FOV, the process often transitions to downstream computer vision tasks like classification. Alternatively, direct capture of principal features by $\B{M}$ is possible if some of its components resemble the FOV. In these tasks, a few measurements are often sufficient with a strong prior derived from training data. Selective codes are commonly employed in this context.
\end{itemize}

==> hardware_pca_onn/sections_2023_Dec_OLD/3_background/model_implementation_old.tex <==
\Xhide{Supposing the image of the field of view consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ masks\Xhide{\bnote{We have not introduced the language mask yet.}}, 
  the single-pixel-sensing process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x}
    \end{aligned}
\end{equation}
, where $\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, $\B{M} \in \IR^{m \times N}$ is the sensing masks\Xhide{or in other words, weighing design (WD) \cite{harwit1979hadamard} \bnote{not sure if language from 1979 is useful. I have not heard of weighing design},} linearly projecting the field of view, and $\B{y} \in \IR^{m \times 1}$ is the corresponding photon counts \cite{willet2009CSPoisson}.}

\Xpolish{
As a typical CI technique, the mathematical foundation of single pixel imaging follows the equation \ref{eqn:NoiselessMeasurement}. However, the different choices of the sensing matrix $\B{M}$ give rise to different coding types (strategies) introduced later. However, $\B{M}$ yields to two constraints when physically implemented. 
}{
As a representative technique in the CI, the mathematical underpinning of single-pixel camera is encapsulated by Eq. \ref{eqn:NoiselessMeasurement}. The diverse selections of the sensing matrix $\B{M}$ lead to distinct coding strategies, as elaborated upon subsequently. \Xhide{Nonetheless, the physical realization of $\B{M}$ introduces two inherent constraints.}
}
\YLnote{Not a good place for this}
\begin{enumerate}
    \item\label{constraint:photonNumber} \textbf{Flux-preserving} \cite{willet2009CSPoisson}\Xhide{\bnote{Y: Should I use the same term as Rebecca?}}. The single-pixel camera model involves the allocation of available photons among masks, as discussed in \cite{neifeld2003dual}. It is important to ensure that the mask basis $\B{M}$ does not produce additional photons through improper entries \cite{neifeld2003dual}. Mathematically, $\sup \sum_{i=1}^m M_{ij} = 1, \forall j \in \{1,2,\dots,N\}$ \cite{neifeld2003dual}.\Xhide{\bnote{Include what an improper entry is!} \bnote{A: this is not something we need to mention here. its obvious that the measurements have to be normalized correctly}}
    \item\label{constraint:negativeEntry} \textbf{Positivity-preserving} \cite{willet2009CSPoisson}. It is not possible to physically implement negative values for the masks $\B{M}$, as demonstrated in \cite{neifeld2003dual, willet2009CSPoisson}. 
\end{enumerate}

\AVnote{the rest of this section can be removed. the figure should stay}
\YLnote{The sensing matrix $\B{M}$ can be generated using either computational or non-computational imaging methods (i.e. Raster scan). The key difference between the two is that computational imaging involves additional steps of optical coding and computational decoding to capture and process the image \cite{cossairt2012does}, while non-computational method, i.e. Raster scan, involves measuring each pixel sequentially \cite{duarte2008CS}. In the case of Raster scan, $\B{M} = \B{I}$, which is an identity matrix. In contrast, computational methods measure a combination of pixels simultaneously and can be further classified based on the type of masks used. For example, Hadamard matrices composed of $\pm 1$ have been shown to be the optimal coding strategy for reconstruction under the AGN \cite{harwit1979hadamard}. A useful feature of computational methods is their compressibility. If the signal is sparse in the subspace of $\B{M}$, it is likely that only a few vectors of $\B{M}$ are needed.}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct measurement scheme (Raster scan)}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {\homedir/figures/Background/RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational imaging scheme (Basis scan)}
        \includegraphics[width=1\linewidth]{\homedir/figures/Background/BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{ Single-Pixel imaging methods. $\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

\YLnote{It is better to intro this at the end of this section or \textbf{move it to methods}}
\Xpolish{
Another problem to be investigated is the noise. To compare measurements, we assume that each measurement is performed using the same amount of light at the camera aperture and over the same total time.
}{
Another critical issue for investigation is noise level. In order to establish meaningful comparisons between measurements, it is assumed that each measurement is conducted under consistent conditions, including uniform light intensity at the camera aperture and an equal duration of exposure.
}

==> hardware_pca_onn/sections_2023_Dec_OLD/3_background/model_under_noise.tex <==
\Xpolish{Two noise models were investigated in this project. The first one is the AGN, or read noise, mainly stemming from thermal vibration of atoms at sensors. In this noise model, the equation \ref{eqn:NoiselessMeasurement} turns into 
\Xequa{
    \noisy{\B{y}} = \B{Mx} + \B{\epsilon} 
},
where $\B{\epsilon} \sim \AGN(\B{0}, \sigma^2\B{I})$ and the $\sigma$ is the standard deviation. The other is the Poisson noise, or shot noise, \Xhide{model for photon-counting systems\rnote{A:shot noise doesn't just exist in photon counting systems} \cite{willet2009CSPoisson} }originating from the statistical nature of photons \cite{boyat2015review} with the following form
\Xequa{
    \noisy{\B{y}} \sim \Poisson(\B{Mx})
}. Due to the constraint \ref{constraint:negativeEntry}, no entries in $\B{M}$ can be negative.}
{This project investigates two noise models. The first one is the additive Gaussian noise (AGN) or read noise, which mainly originates from thermal vibrations of atoms at sensors. In this noise model, Eq. \ref{eqn:NoiselessMeasurement} becomes:
\Xequa{
\noisy{\B{y}} = \B{Mx} + \B{\epsilon},
}
 where $\B{\epsilon} \sim \AGN(\B{0}, \sigma^2\B{I})$, and $\sigma$ is the standard deviation. The other noise model is the Poisson noise or shot noise, which arises from the statistical nature of photons \cite{boyat2015review}. The measurement equation for this noise model is:
\Xequa{
\noisy{\B{y}} \sim \Poisson(\B{Mx}).
\label{eqn:poisson_measurement}
} It should be noted that the constraint \ref{constraint:negativeEntry} in Eq. \ref{eqn:poisson_measurement} prohibits negative entries in $\B{M}$. 
}

\Xhide{
Two noise models were investigated in this project. The first one is the 
% Additive White Gaussian Noise (AWGN)
AGN
, or read noise,  mainly stemming from thermal vibration of atoms at sensors \iffalse the imperfectness of sensors\fi \cite{boyat2015review} with the following form
% \subsubsection{Gaussian Noise Model}
\Xequa{
    \Xalign{
        \lambda\tilde{\B{y}^+} &\sim \mathcal{N}(\lambda \B{M}^+ \B{x} , \sigma^2 \B{I})\\
        \lambda\tilde{\B{y}^-} &\sim \mathcal{N}(\lambda \B{M}^- \B{x} , \sigma^2 \B{I})
    },
} 
% \subsubsection{Poisson Noise Model}
where the $\sigma$ is the standard deviation. The other is the Poisson noise, or shot noise, \Xhide{model for photon-counting systems\rnote{A:shot noise doesn't just exist in photon counting systems} \cite{willet2009CSPoisson} }originating from the statistical nature of photons \cite{boyat2015review} with the following form
\Xequa{
    \Xalign{
        \lambda\tilde{\B{y}^+} &\sim \mathcal{P}(\lambda \B{M}^+ \B{x})\\
        \lambda\tilde{\B{y}^-} &\sim \mathcal{P}(\lambda \B{M}^- \B{x})
    }.
}   
\bnote{This paragraph is somewhat confusing, and some of the ideas should maybe be before the equations.}  
Although we can obtain a negative number of photons from the difference between the two branches, the Poisson noise cannot be directly applied to these values. Otherwise, it violates the nature of Poisson distributions and the fact that Poisson noise appears in the sensors. On the contrary, noise should be considered in both branches independently.  
\bnote{Mention that this comes from the relevant equation in the dual branch section. }
Therefore, in the AGN model, the measurement $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{Mx}, 2\sigma^2 \B{I})$ with the dual-rail trick. But in the Poisson noise model, the measurement $\lambda \tilde{\B{y}} \sim \text{Skellam}(\lambda \B{M}^+ \B{x}, \lambda \B{M}^- \B{x})$ \cite{hwang2007skellam, gan2017skellam}. 
}

% \subsection{Scan Strategies with Different Priors}

% \bnote{We should maybe focus less on the term "single-pixel imaging" that is the way we show our results but maybe it obscures our main point.}

% \Xhide{\ynote{We already talked about single pixel imaging in the beginning. I think the figure could be introduced here along with the math model}
% Single-pixel imaging is a technique that involves both computational and non-computational methods. }

==> hardware_pca_onn/sections_2023_Dec_OLD/3_background/restrictions_of_masks.tex <==
\Xpolish{Though we are able to find the ideal $\B{M}$ based on the tasks we want to accomplish, the optimization problem of $\B{M}$ may not be convex due to the following two constraints.}
{While we can identify the optimal $\B{M}$ tailored to the tasks at hand, it's crucial to acknowledge that the optimization problem for $\B{M}$ might not exhibit convexity. This is attributed to the presence of two constraining factors. Consequently, achieving globally optimal masks may not be universally feasible within the scope of this problem.}

\begin{enumerate}
    \item\label{constraint:photonNumber} \textbf{Flux-preserving} \cite{willet2009CSPoisson}\Xhide{\bnote{Y: Should I use the same term as Rebecca?}}. The single-pixel camera model involves the allocation of available photons among masks, as discussed in \cite{neifeld2003dual}. It is important to ensure that the mask basis $\B{M}$ does not produce additional photons through improper entries \cite{neifeld2003dual}. Mathematically, $\sup \sum_{i=1}^m M_{ij} = 1, \forall j \in \{1,2,\dots,N\}$ \cite{neifeld2003dual}.\Xhide{\bnote{Include what an improper entry is!} \bnote{A: this is not something we need to mention here. its obvious that the measurements have to be normalized correctly}}
    \item\label{constraint:negativeEntry} \textbf{Positivity-preserving} \cite{willet2009CSPoisson}. It is not possible to physically implement negative values for the masks $\B{M}$, as demonstrated in \cite{neifeld2003dual, willet2009CSPoisson}. In this project, we employed the dual-rail approach as outlined in the work of Neifeld et al. \cite{neifeld2003dual}.
\end{enumerate}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods.tex <==
\input{\homedir/sections/4_methods/model_config.tex}


\input{\homedir/sections/4_methods/model_validation.tex}

% move this section to appendix 
%\input{\homedir/sections/4_methods/sensing_matrices_by_prior.tex}

% move this section to appendix 
% \input{\homedir/sections/4_methods/constraint_implement.tex}

\input{\homedir/sections/4_methods/simulations.tex}

% \input{\homedir/sections/4_methods/spectral_datasets.tex}

\input{\homedir/sections/4_methods/experiments.tex}

% \bnote{The ONN should be introduced here first, then show the results in reconstruction}




==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/constraint_implement.tex <==
\subsection{Constraints Implementation}

\Xpolish{This section introduces our methods for the optical implementations for the model. To construct a valid model, the Flux-preserving and Positivity-preserving constraints has been satisfied by the following techniques.}
{In this section, we outline our methods for implementing the model optically. In order to ensure that our model is valid, we have implemented techniques that satisfy both the Flux-preserving and Positivity-preserving constraints. By using these techniques, we can ensure that the model accurately represents the underlying physical processes and produces results that are both reliable and interpretable.}

\subsubsection{Photon Distribution Factor} \label{sssection:PDF}
\Xhide{\bnote{A: This section shouldn't be here}}

\Xpolish{The optimization of $\B{M}$ can be challenging, as it is subject to constraint \ref{constraint:photonNumber}.\Xhide{ Specifically, $\B{M}$ must belong to a subset $S$ of $\IR^{m \times N}$, which can vary depending on the specific case \bnote{<- not sure why this sentence is here}. To address this issue \bnote{the issue of belonging to a subset?}, } Here, we propose using a scale factor as a solution. This allows us to select any values for $\B{M}$ without being limited by the constraint \ref{constraint:photonNumber}\Xhide{\bnote{It would be nice to name the constraints}}. The Photon Distribution Factor, $\lambda$, is thus introduced to ensure compliance with constraint \ref{constraint:photonNumber}. As a scale factor, it is calculated as \Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m v_k}},\Xhide{ \bnote{this should be in an equation line}} where $\flux$ represents the number of photons per second projected onto the DMD, $\totexposure$ is the total exposure time for all masks, $N$ represents the number of pixels, and $v_k$ represents the greatest value of the $k_\text{th}$ mask. The maximum value $v_k$ is selected as its corresponding pixel is open for longer than any other one in the $k_\text{th}$ mask, and the exposure time of this mask depends solely on $v_k$. Furthermore, the total exposure time $\totexposure$ is proportional to $\sum_{k=1}^m v_k$ and the total number of photons from the field of view is $\totexposure \sum_{i=1}^N \frac{\flux}{N} x_i$.  }
{Optimizing $\B{M}$ subject to constraint \ref{constraint:photonNumber} can be challenging. To overcome this limitation, we propose the use of a scale factor, known as the Photon Distribution Factor $\lambda$, which allows us to select any values for $\B{M}$ without violating constraint \ref{constraint:photonNumber}. The Photon Distribution Factor is calculated as \Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m v_k}}, where $\flux$ is the number of photons per second projected onto the DMD, $\totexposure$ is the total exposure time for all masks, $N$ is the number of pixels, and $v_k$ is the greatest value of the $k_\text{th}$ mask. The maximum value $v_k$ is chosen as its corresponding pixel is open for longer than any other pixel in the $k_\text{th}$ mask, and the exposure time of this mask depends solely on $v_k$. Moreover, the total exposure time $\totexposure$ is proportional to $\sum_{k=1}^m v_k$, while the total number of photons from the field of view is $\totexposure \sum_{i=1}^N \frac{\flux}{N} x_i$.}

\Xhide{\rnote{Maybe in appendix} \bnote{ Could just state the first and last lines of the math and move the proof to the appendix but still state this ensures constraint one is true}
% Suppose we use an arbitrary matrix $\{\B{a}_1, \dots, \B{a}_m \} \in \IR^{N \times m}$ for measurement, the total number of photons detected is
When an arbitrary measurement matrix, $\{\B{a}_1, \dots, \B{a}_m \} \in \IR^{N \times m}$, is used, the total number of detected photons can be expressed as $\sum_{i=1}^m \lambda \B{a}_i^\top \B{x}$ and the following inequality always holds:
\begin{equation}
\begin{aligned}
    \sum_{i=1}^m \lambda \B{a}_i^\top \B{x} &\le \sum_{i=1}^m \lambda \sum_{j=1}^N v_i x_j\\
    &= \sum_{i=1}^m \sum_{j=1}^N \frac{\flux \totexposure}{N \sum_{k=1}^m v_k} v_i x_j \\
    &= \frac{\flux \totexposure}{N} \sum_{j=1}^N x_j  \frac{\sum_{i=1}^m v_i}{\sum_{k=1}^m v_k} \\
    &= \totexposure \sum_{j=1}^N \frac{\flux}{N} x_j
\end{aligned}.
\end{equation}
% Therefore, by the Photon Distribution Factor, the constraint \ref{constraint:photonNumber} is never violated.
}

\Xpolish{By utilizing the Photon Distribution Factor, constraint \ref{constraint:photonNumber} is guaranteed to be never violated. Then we can re-formulate model in Equation \ref{eqn:NoiselessMeasurement} as the following equation
 \begin{equation} \label{eqn:NoisyMeasurement}
    \begin{aligned}
        \tilde{\B{y}} &=  \frac{1}{\lambda}f_r(\lambda \B{ M x})
    \end{aligned}
\end{equation}
, where $f_r$ generates random numbers with expectation $\lambda \B{ M x}$ to simulate the noise and gives rise to the measurement with noise \bnote{Be consistent with language throughout the text. "noisy-version-measurement" is probably not the best name} $\tilde{\B{y}}$.}
{By utilizing the Photon Distribution Factor, we can guarantee that constraint \ref{constraint:photonNumber} is never violated. With this in mind, we can re-formulate the model in Equation \ref{eqn:NoiselessMeasurement} into the following equation,
\Xequa{\tilde{\B{y}} &=  \frac{1}{\lambda}f_r(\lambda \B{ M x})}.
Here, $f_r$ generates random numbers with an expected value of $\lambda \B{ M x}$ to simulate noise and produce a measurement with noise, denoted as $\tilde{\B{y}}$.}

\subsubsection{Dual-Rail Technique for Negative Entries}\label{sssection:DualBranch}
\Xpolish{\Xhide{\ynote{this could be part of a methods section later on or go to the supplement. Shouldn't be here.}\bnote{Consistent language "Rail" or "Branch" or "Path"} }
The dual-rail technique is introduced for constraint \ref{constraint:negativeEntry} \cite{neifeld2003dual}. In it\Xhide{ \bnote{ might be better to call it a "technique"}}, one measurement needs two complementary branches where one measures with all positive entries, $\B{M}^+$, and the other measures with all negative entries, $\B{M}^-$ \cite{neifeld2003dual}. }
{To satisfy constraint \ref{constraint:negativeEntry}, the dual-rail technique \cite{neifeld2003dual} employs two complementary measurement branches: one measures with all positive entries, denoted as $\B{M}^+$, while the other measures with all negative entries, denoted as $\B{M}^-$. By doing so, the dual-rail technique effectively converts the constraint on negative entries to a constraint on the difference between the measurements made by the two branches.}

\begin{figure}[h]
    \centering
    % \includesvg[width=0.9\linewidth]{\homedir/figures/Methods/Dual_rail.svg}
    \includegraphics[width=0.9\linewidth]{\homedir/figures/Methods/Dual_rail.pdf}
    \caption{Dual-Rail technique}
    \label{fig:Dual-Rail Technique}
\end{figure}


\Xpolish{\bnote{Many of these equations should be on their own line for readability and to reference them later. We have 11 pages so we can do this easily.}
To create the two branches, the mask $\B{M}$ should be split into $\B{M}^+ = \max(\B{M}, 0)$ and $\B{M}^- = \max(-\B{M}, 0)$. The superscripts of the parameters indicate the branches they belong to. Intuitively, we have $\lambda \tilde{\B{y}} = \lambda \tilde{\B{y}}^+ - \lambda \tilde{\B{y}}^-$ where $\tilde{\B{y}}^+$ and $\tilde{\B{y}}^-$ are photon counts with noise measured by $\B{M}^+$ and $\B{M}^-$ respectively. The two-rail trick also changes the expression of the  Photon Distribution Factor. In the case that each branch has a PMT, 
\Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m |v_k|}}
where $|\cdot|$ takes the absolute value. In the case of using only one PMT, it is worth noting that the Photon Distribution Factor changes to 
\Xequa{\lambda = \frac{\flux \totexposure}{N (\sum_{k=1}^m v_k^+ + \sum_{k=1}^m v_k^-)}}
as one PMT measures with $\B{M}_k^+$ and $\B{M}_k^-$ in turn to accomplish measuring $\B{M}_{k}$. \iffalse as there are approximately two times of measurements. \fi \rnote{figure}All the parameters in this updated Photon Distribution Factor are of the same meaning as in section \ref{sssection:PDF}.}{To implement the two branches, we split the mask $\B{M}$ into two components: $\B{M}^+ = \max(\B{M}, 0)$ and $\B{M}^- = \max(-\B{M}, 0)$, with the superscripts indicating the respective branches. This enables us to express $\lambda \tilde{\B{y}}$ as the difference between the photon counts with noise measured by $\B{M}^+$ and $\B{M}^-$, denoted $\lambda \tilde{\B{y}}^+$ and $\lambda \tilde{\B{y}}^-$, respectively. Notably, the two-rail approach also modifies the expression for the Photon Distribution Factor. In the case that each branch has a PMT, 
\Xequa{\lambda = \frac{\flux \totexposure}{N \sum_{k=1}^m |v_k|}}, 
where $|\cdot|$ takes the absolute value. In the case of using only one PMT, it is worth noting that the Photon Distribution Factor changes to 
\Xequa{\lambda = \frac{\flux \totexposure}{N (\sum_{k=1}^m v_k^+ + \sum_{k=1}^m v_k^-)}},
since one PMT measures with both $\B{M}_k^+$ and $\B{M}_k^-$ sequentially to obtain the measurement result for $\B{M}_{k}$. All the parameters in this updated Photon Distribution Factor are of the same meaning as in section \ref{sssection:PDF}, and $v_k^+$ and $v_k^-$ stand for the maximum values of $\B{M}^+$ and $\B{M}^-$ respectively. 
} 

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/experiments.tex <==
\subsection{Hardware Experiments}

\Xpolish{Besides the simulations, an experiment is also conducted to enhance our conclusion. The DMD we use is the DLP 7000 purchased from Texas Instruments and the PMT is the PMA Series from PicoQuant. This experiment consisted of a hardware-end data capture and a software-end classifier training. \Xhide{The steps are introduced in the following sections.}}
{To further support our conclusions, we conducted an experiment in addition to simulations. The experiment utilized a DMD (digital micromirror device), specifically the DLP 7000 model from Texas Instruments, and a PMT (photomultiplier tube) from PicoQuant, specifically the PMA Series. The experimental setup involved both hardware-end data acquisition and software-end classifier training.}

% \subsubsection{Data preparation}

\Xpolish{Before data acquisition, we transformed and re-calibrated the MNIST images into what the PMT exactly "observed", and trained the classifier with this new data. This step is important if we don't use the hardware-end data for training.}
{To ensure that the classifier was accurately trained using the PMT data, we performed a transformation and re-calibration of the MNIST images to match what the PMT would actually "observe" during data acquisition. This step is crucial when training the classifier without the use of hardware-end data. By implementing this transformation and re-calibration process, we were able to accurately simulate the imaging conditions that the PMT would encounter during actual data acquisition, allowing for more reliable and robust classification results.}

\Xpolish{First, we conducted a Raster scan on a sample from MNIST data and each mask in this scan was exposed for 1 second. The light level had been adjusted and the brightest pixel in this experiment generated about 1000 photon records per second. The captured data vector was then reshaped into a 32 by 32 image, which can be treated as a linearly transformed version of the raw image.}
{First, we performed a Raster scan of a sample from the MNIST dataset, with each mask exposed for 1 second. The light intensity was adjusted to ensure that the brightest pixel generated approximately 1000 photon counts per second. The data captured during this experiment was then reshaped into a 32 by 32 image, which can be regarded as a linearly transformed version of the original raw image.}

\begin{figure}[h]
    \centering
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=0.4\linewidth]       {\homedir/figures/Methods/sensor_perception_raw.png}
        \includegraphics[width=0.4\linewidth]{\homedir/figures/Methods/sensor_perception_crop2.pdf}
        % crop2 is better one
        \label{fig:sensor_perception}
    \end{subfigure}
    \caption{Raw image (left) VS measured image}
\end{figure}

\Xpolish{Then, we estimated the linear transformation between the digital data and exprimental data, and then transformed all digital data in the same way so that the new data are similar to the sensor's observation. This transformed data was then input into the code modules used for simulation to train the software-end classifier. For the selective sensing, the masks were also trained in this step.}
{Then, we estimated the linear transformation between the digital and experimental data to ensure that the digital data closely matched the sensor's observations. After applying this transformation to all digital data, we used it to train the software-end classifier through simulation. Additionally, in this step, the masks used for Selective Sensing were also trained.} \YLnote{The masks with decimals use the fraction of a super pixel \cite{spall22hybrid_training} The ONN training is called \textit{in silico} method (Wright et al) \cite{spall22hybrid_training, wright2021backprop}}

\Xpolish{Finally, we uploaded the masks as the pattern sequences onto the DMD to acquire the data $\noisy{\B{y}}$. The testset consisted of ten images and each handwritten number appeared exactly once. The exposure time for each mask was 1 second. Since all photon records preserved the arrival time, we could change the noise level by choosing random intervals during the whole exposure time and counting the photons within it. }
{After generating the mask pattern sequences, we uploaded them onto the DMD to acquire the data, denoted as $\noisy{\B{y}}$. Our test set consisted of ten handwritten images, each of which appeared exactly once during the experiment. To control the noise level in the data, we varied 
% the number of photons recorded within 
lengths of random intervals throughout the 1-second exposure time for each mask. By preserving the arrival times of all photons, we were able to systematically adjust the level of noise in the acquired data.}


\begin{figure}[h]
    \centering    
        \includegraphics[width=\linewidth]       {\homedir/figures/Methods/HardwareSetup.jpg}        
        % crop2 is better one
        \label{fig:hardware_setup}
    \caption{Experimental Configuration of the Single-Pixel Camera: The light path is illustrated by the blue arrows in the diagram. Specifically, our setup utilizes only one branch reflected by the DMD.}
\end{figure}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/model_config.tex <==
\subsection{Model Configuration \ynote{\checkednote{this is just the ONN. We probably also want to say something about PCA}}} 
\Xpolish{Although coding strategies are different, they essentially share the same model structure shown in figure \ref{fig:model_config} for classification tasks. In this study, we built a classification pipeline consisting of a scanner module and a classifier in PyTorch. This model consists of a \textit{scanner} module and a \textit{classifier} module.\Xhide{The scanner is simulating the measurement process described in equation \ref{eqn:NoisyMeasurement} and the classifier is a neural networks model.} The scanner simulates the operations to count the photons, following the techniques\Xhide{ \bnote{"tricks" -> "techniques"}} mentioned in section \ref{ssec:ModelFormulation}. We\Xhide{ also \bnote{"Also" could mean we have two different models.}} employed a two-hidden layer artificial neural network (ANN) classifier with 40 and 128 nodes as the main model for predicting which number the object is.
%by the corresponding  number of re-centered, normalized, and noisy photon counts. 
% The input data for the classifier was obtained by subtracting the average of the training data, represented by $\B{\bar{x}}_T$, from the re-centered normalized noisy photon counts, denoted by $\tilde{\B{y}}$. 
To prevent overfitting and improve the generalizability of the model, dropout  was applied after each hidden layer, followed by a ReLU activation layer.  }
{All coding strategies for classification tasks share the same fundamental model structure, as illustrated in Fig. \ref{fig:model_config}. To classify handwritten numbers using optical devices with limited photon budget, we built a PyTorch-based pipeline consisting of a \textit{scanner} module and a \textit{classifier} module. The scanner module simulates the photon counting process using the techniques described in section \ref{ssec:selectionofsensingmatrix}. For the classification task, we utilized a two-hidden layer artificial neural network (ANN) with 40 and 128 nodes, serving as the primary model. To prevent overfitting and enhance generalizability, we applied dropout after each hidden layer, followed by a rectified linear unit (ReLU) activation layer.}

\Xpolish{When training this model, the scanner computes the photon counts with noise, and feeds it to the classifier. The noise is sampled from a predefined noise distribution, and is different in different epochs. After the loss is computed, parameters in the classifier are optimized by gradient descent. The ONN is different from the others as the back-propagation is extended into the scanner so that the masks are optimized together with the classifier.}
{During the training of the model, the scanner computes the photon counts with noise and then transmits this data to the classifier. The noise is sampled from a pre-defined noise distribution and varies across epochs. Once the loss has been computed, gradient descent is used to optimize the parameters of the classifier. \textbf{What sets the ONN apart from other models is that back-propagation is extended into the scanner, allowing for the simultaneous optimization of the masks and the classifier {under different noise models}}. This approach offers distinct advantages compared to traditional methods, which typically optimize the classifier independently of the scanner {or optimize the scanner without the appropriate noise model}.}

\begin{figure}[ht]
    \centering
    % \includesvg[width=0.9\linewidth]{\homedir/figures/Methods/Model_Structure.svg}
    \includegraphics[width=0.9\linewidth]{\homedir/figures/Methods/Model_Structure.pdf}
    \caption{Model configuration}
    \label{fig:model_config}
\end{figure}

ONN can also be used for reconstruction. \YLnote{To address this, we propose a simple approach of optimizing the ONN masks for a reconstruction task under different noise models. To achieve this, we developed a new ONN model with $m = N$ masks. The scanner takes raw image vectors $\B{x}$ and outputs $N$-element measured photon count vectors under a chosen noise model, $\noisy{\B{y}}$. The classifier is a single-layer network that takes $\noisy{\B{y}}$ as input and outputs $\noisy{\B{x}}$, also an $N$-element vector. The objective is to minimize the MSE between the input images and the output vectors, $\|\noisy{\B{x}} - \B{x}\|_2^2$. In noiseless cases, the classifier is equivalent to $\B{M}^{-1}$, where $\B{M}$ is the masks used in the scanner.}


\subsubsection*{ONN Optimization under Poisson Noise} 

\Xpolish{Since the Poisson noise generating function has no gradient, it is challenging to optimize the scanner. The reparameterization trick is a useful method for the AGN instead of the Poisson noise. Our method is using a normal distribution whose variance equals its expectation to approximate the Poisson distribution in training, and therefore, the reprameterization trick can be employed.}
{Optimizing the scanner can be challenging as the Poisson noise generating function typically lacks a gradient. While reparameterization is a useful method for addressing AGN, it is not as effective for addressing Poisson noise. To address this limitation, we employ a method mentioned by Cossairt et al. that utilizes a normal distribution with a variance equal to its expectation to approximate the Poisson distribution during training \cite{cossairt2012does}.\ynote{\checkednote{we need more details on this and how it is implemented in the network. Probably a figure of the entire network structure and the equation for the gradient (i think we also have references to cite here)}} This approximation enables us to employ PyTorch builtin reparameterization method, i.e. \texttt{rsample}, and optimize the scanner more effectively under Poisson noise.}

% \YLnote{
% A seperate section? And mention that Ollie did that as well.  \\
% Similar to corssairt et al, we use a normal dist to approximate poisson
% }

% \YLnote{
% Transform $\B{y} \sim \mathcal{P}(\B{Mx})$ to $\B{y} \sim \mathcal{N}(\B{Mx}, (\B{Mx})^\frac{1}{2})$ to use the reparamaterization trick. The variance will also play a role in computing the gradient.
% } 

To approximate the Poisson noise by the AGN, we can re-write the measurement with noise $\noisy{\B{y}} = \B{Mx} + \B{J}$ where $\B{J} =  (\B{Mx})^{\frac{1}{2}} \odot \B{\epsilon}, \B{\epsilon} \sim \mathcal{N}(0, \B{I})$. During the training under Poisson noise, $\B{J}$ also plays a role in gradient computation, which is the most significant difference compared with training under the AGN. 

\textcolor{blue}{\checkednote{I think we can remove sections 4.2 and 4.3. They mostly repeat waht we already said and add too much detail for a paper.}}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/model_validation.tex <==
\subsection{Model Validation}

% In this section, we start with a theoretical investigation on the reconstruction performances of null-prior strategies. Then the reconstruction and classification performances of all strategies and fairly compared by simulations and experiments. 

\Xpolish{To validate the ONN model is correct, we begin with a theoretical derivation of the null-prior reconstruction. Afterwards, we test our ONN model by reconstructing random signals under two noise models and see what the optimized masks converge to at last.}
{
To affirm the correctness of the ONN model, we initiate the validation process with a theoretical derivation of the null-prior reconstruction. Subsequently, we conduct empirical testing of the ONN model by reconstructing random signals under two distinct noise models. This experimental approach allows us to observe the convergence of optimized masks, providing empirical evidence for the validity and efficacy of the ONN model.}

\subsubsection{Theoretical Treatment for Null-Prior Reconstruction }


% \textcolor{blue}{This section could be taken out.}
Define $\B{I}$ as the identity matrix and $\totphoton = \rho \tau$ as the total number of photons from the source. Given the noisy photon counts $\tilde{\B{y}}$ and the full-rank mask basis $\B{M}$, we can reconstruct the field of view $\tilde{\B{x}} = \B{M}^{-1} \tilde{\B{y}}$.
Based on Parseval's identity, the covariance matrix of a vector $\B{b}$ is $\B{\Sigma}_{\B{b}\B{b}} = c^2 \sigma^2 \B{I}$ if $\B{b} = \B{W a}$ where $\B{\Sigma}_{\B{a}\B{a}} = \sigma^2 \B{I}$ and 
% $\B{W}$ is $c$ times an orthonormal matrix
$\B{W} \B{W}^\top = c^2 \B{I}$
. For RS, we have $\lambda = \frac{\totphoton}{N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{I}\B{x}, \sigma^2 \B{I})$. Thus, the reconstructed field of view is 
\begin{equation}
    \label{eqn:RS_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{\sigma^2 N^4}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
For HB, we have $\lambda = \frac{\totphoton}{2N^2}$  and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{H}\B{x}, 2\sigma^2 \B{I})$ due to the dual branch trick mentioned in section \Xpolish{\ref{sssection:DualBranch}}{\ref{ssection:constraints}}. For $\B{H}^{-1}$, $c = \sqrt{\frac{1}{N}}$. The reconstructed field of view is 
\begin{equation}
    \label{eqn:HB_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{8 \sigma^2 N^3}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
% Therefore, when considering the AWGN model, using the Hadamard matrix can improve the SNR of the reconstructed field of view when $N$ is large.
Therefore, using the Hadamard matrix in the AWGN model can improve the signal-to-noise ratio (SNR) of the reconstructed field of view when the number of elements, $N$, is large. 

When the noise is Poisson distributed, the covariance matrix of the noisy photon counts depends on the choice of $\B{M}$. Suppose $\sigma_j$ is the standard deviation of $\lambda \tilde{y}_j$, the $j_\text{th}$ measured noisy photon counts. For the RS, we have $\sigma_j^2 = \lambda x_j$ and $\lambda = \frac{\totphoton}{N^2}$. The covariance matrix of the reconstructed field of view is thus 
\begin{equation}
    \label{eqn:RS_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{N^2}{\totphoton}\diag\{x_1, x_2, \cdots, x_N\}
    \end{aligned}.
\end{equation}
% For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$ by the Skellam Distribution in section \ref{sssection:DualBranch}. Since Hadamard matrices only includes $\pm 1$ entries, we further have $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$ and the covariance matrix  

In the case of the HB, we can express the rate parameter $\lambda$ as $\lambda = \frac{\totphoton}{2N^2}$, as demonstrated in section \ref{ssection:constraints} using the Skellam Distribution. Additionally, we can express the variance of each element in the sum as $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$. As Hadamard matrices only contain entries of $\pm 1$, this reduces to $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$. Using this information, we can construct the covariance matrix
\begin{equation}
    \label{eqn:HB_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{2N \sum_{k=1}^N x_k}{\totphoton}  \B{I}
    \end{aligned}.
\end{equation}
% Therefore, the mean squared error (MSE) of HB is 2 times that of RS under Poisson noise. This factor of 2 arises from the dual branch trick. In other words, HB can never exceed RS in reconstruction error even when measuring with 2 PMTs simultaneously.
The results of our analysis reveal that the mean squared error (MSE) of the HB method is twice that of the RS method when the noise is Poisson distributed. This difference is attributed to the dual branch trick utilized in the HB method. Despite the use of two PMTs in the HB method, it is unable to surpass the reconstruction error of the RS method. These findings demonstrate the limitations of the HB method in comparison to the RS method under Poisson noise conditions.


\begin{figure}[ht]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Reconstruction under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_reconstruction.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_reconstruction.pdf}
        \label{fig:gaussian_reconstruction}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering        
        \caption{Reconstruction under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_reconstruction.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_reconstruction.pdf}
        \label{fig:poisson_reconstruction}
    \end{subfigure}
    \caption{Reconstruction errors on simulated data. RS: Raster basis. HB: Hadamard basis. II: Impulse imaging. BR: Binary random basis. (\subref{fig:gaussian_reconstruction}) RS is always worse than HB for all noise levels under Gaussian noise. (\subref{fig:gaussian_reconstruction}) HB is no better than RS under Poisson noise.
    }
    \label{fig:simulated_reconstruction}
\end{figure}




\subsubsection{Mask optimized with ONN for Reconstruction}

\Xhide{The first question to be answered is if the ONN can find the (approximately) optimal masks. To get the benchmark, we compared the reconstruction performance w.r.t the mean squared error between the raw and reconstructed images $\|\noisy{\B{x}} - \B{x}\|_2^2$ where $\noisy{\B{x}} = \B{M}^{-1} \noisy{\B{y}}$. Fig. \ref{fig:simulated_reconstruction} shows that Hadamard Basis is less preferred under Poisson noise but more optimal under the AGN compared with the Raster Basis.}

\Xpolish{We already saw the ONN had the best classification performance on the simulated data and its masks are optimal, it is still unclear if the ONN masks under the AGN and Poisson noise are similar. Since many algorithms are based on the AGN model, the conclusions drawn from them may be problematic if the optimal masks are different under the Poisson noise model. One simple approach is to let the ONN optimize the masks for a reconstruction task under different noise models. Therefore, we built a new ONN model which has $m = N$ masks. Its scanner took the raw images vectors $\B{x}$, and output $N$-element measured photon count vectors under some noise model, $\noisy{\B{y}}$. Its classifier is a single-layer network taking $N$-element vectors $\noisy{\B{y}}$ and outputting $N$-element vectors $\noisy{\B{x}}$. The objective is to minimize the MSE between the input images and the output vectors, or $\|\noisy{\B{x}} - \B{x}\|_2^2$. In noiseless cases, the classifier is equivalent to $\B{M}^{-1}$ if $\B{M}$ is the masks in the scanner.}
{\Xhide{The ONN demonstrated superior classification performance on simulated data with optimal masks; however, it remains unclear whether these masks are optimal under different noise models, specifically AGN and Poisson noise.} 
The primary question to address is whether the ONN has the ability to identify noise specific optimized masks. We established a benchmark by comparing the reconstruction performance in terms of mean squared error (MSE) between the original and reconstructed images, denoted by $\|\noisy{\B{x}} - \B{x}\|_2^2$, where $\noisy{\B{x}} = \B{M}^{-1} \noisy{\B{y}}$. The reconstructed images were obtained using the Hadamard basis and Raster basis under Poisson noise and AGN models respectively. The outcomes, depicted in Fig. \ref{fig:simulated_reconstruction} where the x-axis is the log-scaled MSE of impulse imaging with different exposure times, indicate that the Hadamard basis is less effective in the presence of Poisson noise, while it is more effective under the AGN model when compared to the Raster basis. Given that many algorithms rely on the AGN model, their conclusions may not hold if the optimal masks differ under Poisson noise. \ynote{\checkednote{the following text does not belong in the results section}}\Xhide{ To address this, we propose a simple approach of optimizing the ONN masks for a reconstruction task under different noise models. To achieve this, we developed a new ONN model with $m = N$ masks. The scanner takes raw image vectors $\B{x}$ and outputs $N$-element measured photon count vectors under a chosen noise model, $\noisy{\B{y}}$. The classifier is a single-layer network that takes $\noisy{\B{y}}$ as input and outputs $\noisy{\B{x}}$, also an $N$-element vector. The objective is to minimize the MSE between the input images and the output vectors, $\|\noisy{\B{x}} - \B{x}\|_2^2$. In noiseless cases, the classifier is equivalent to $\B{M}^{-1}$, where $\B{M}$ is the masks used in the scanner.}
}

\Xpolish{To make this reconstruction task less specific and more general, the input data vectors $\B{x}$ were reshaped from 8 by 8 random patterns. In different epochs of training, the $\B{x}$ was re-generated randomly. This simulation is conducted with a great noise level as the total number of photons is about $1 \times 10^3$. The masks $\B{M}$ were initialized with an $N \times N$ identical matrix and were optimized until this model reported constant losses.}
{To make this reconstruction task less specific and more general, we reshaped the input data vectors $\B{x}$ from $10^5$ random 8 by 8 patterns, increasing their generality. We randomly re-generated $\B{x}$ for 10 times during the training, introducing additional variability. The simulations were conducted under significant noise, with a total of $1 \times 10^2$ photons. We initialized the masks $\B{M}$ with an $N \times N$ identical matrix and a $\{0,1\}$ Hadamard matrix respectively, and optimized them until the model reported constant losses.}

\Xpolish{The first 6 masks optimized by the ONN is shown in figure \ref{fig:recon_masks}. From it, we can see that the ONN model has very different behaviors under the AGN and the Poisson noise. For the AGN, it tended to open more pixels to increase the light throughput, while it adhered to the RS mode for the Poisson noise. The figure \ref{fig:masks_value_dist} gives a more thorough visualization of the optimized masks by showing their entries' distributions. The x-axis is the values in the masks and the y-axis is the total number of entries in a certain range. This result is consistent with the classification results in the last section, where the RS is mediocre under the AGN but much better under the Poisson noise.}
{Fig. \ref{fig:recon_masks} displays the first 6 optimized masks generated by the ONN model. A notable observation is that the model exhibits distinct behavior patterns under the AGN and Poisson noise. Specifically, it tends to open more pixels to enhance light throughput under the AGN, but adheres to the RS mode under the Poisson noise. Fig. \ref{fig:masks_value_dist} provides a more detailed visualization of the optimized masks by presenting the distribution of their entries. The x-axis represents the values in the masks, while the y-axis shows the total number of entries within a specific range. This observation aligns with the reconstruction results\Xhide{classification results presented in the previous section}, where the RS performed modestly under the AGN but considerably better under the Poisson noise. The rationale behind this is that re-projection from a captured basis into a basis of sparsity does not yield the same recovery quality under Poisson noise that is provides for AGN. To obtain a performance benefit over the trivial point scanning method, or RS, it is essential that the data is sparse and is captured in a sparse basis. Since random patterns are not sparse, the best scanning strategy is the point scanning, which matches our results.}

\begin{figure}[h]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{ONN optimized masks under Gaussian noise. Left: initialized with the identity matrix. Right: initialized with the Hadamard matrix.}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.svg}
        \includegraphics[width=0.49 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks.pdf}
        \includegraphics[width=0.49 \linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_gaussian_masks_Hadamard.pdf}
        \label{fig:gaussian_recon_masks}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering        
        \caption{ONN optimized masks under Poisson noise. Left: initialized with the identity matrix. Right: initialized with the Hadamard matrix.}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.svg}
        \includegraphics[width=0.49\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks.pdf}
        \includegraphics[width=0.49\linewidth]{\homedir/figures/Results/ONN_recon/ONN_recon_poisson_masks_Hadamard.pdf}
        \label{fig:poisson_recon_masks}
    \end{subfigure}
    \caption{First 6 optimized masks}
    \label{fig:recon_masks}
\end{figure}

\Xhide{
\begin{figure}[h]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Value distribution of the optimal masks under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_gaussian.pdf}
        \label{fig:gaussian_recon_masks_dist}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Value distribution of the optimal masks under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_poisson.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_poisson.pdf}
        \label{fig:poisson_recon_masks_dist}
    \end{subfigure}
    \caption{Masks values distribution (x-axis: mask values; y-axis: counts). (\subref{fig:gaussian_recon_masks_dist}) Given a Raster scan mask family, ONN returns a different mask family under the AGN, indicating that Raster scan is always suboptimal. (\subref{fig:poisson_recon_masks_dist}) ONN adheres to the Raster scan, suggesting it is optimal under Poisson noise.
    textcolor{red}{these can be much smaller}
    }
    \label{fig:masks_value_dist}
\end{figure}
}

\begin{figure}[h]  
    % \begin{subfigure}{0.49\linewidth}
    % \centering  
    % \caption{$\B{M}_G^I$ VS $\B{M}_P^I$}
    % \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist.pdf}    
    % \end{subfigure}    
    % \begin{subfigure}{0.49\linewidth}
    % \centering  
    % \caption{$\B{M}_G^H$ VS $\B{M}_P^H$}
    % \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist_Hadamard.pdf}
    % \end{subfigure}    
    \includegraphics[width=1\linewidth]{\homedir/figures/Results/ONN_recon/Mask_value_dist.pdf}
        \caption{\Xpolish{Denote masks initialized with the identity matrix and optimized under the AGN as $\B{M}_G^I$, masks initialized with the identity matrix and optimized under the Poisson noise as $\B{M}_P^I$, masks initialized with the Hadamard matrix and optimized under the AGN as $\B{M}_G^H$, masks initialized with the Hadamard matrix and optimized under the Poisson noise as $\B{M}_P^H$.  
        $\B{M}_G^I$ is going to increase the light throughput by openning more pixels, but $\B{M}_P^I$ is fixed as it is already an ideal choice. $\B{M}_P^H$ is approaching the identity matrix, differently from the $\B{M}_G^H$. Due to the fact that this optimization problem is not perfectly convex, it is difficult to optimize $\B{M}_P^H$ to the perfect identity matrix, but it shows essential differences between the optimization questions under these two distinct noise models.}{
        The Poisson noise data is displayed topside-down by negating its counts. Let $\B{M}_G^I$ represent masks initialized with the identity matrix and optimized under the AGN, and $\B{M}_P^I$ denote masks initialized with the identity matrix and optimized under Poisson noise. Additionally, $\B{M}_G^H$ and $\B{M}_P^H$ represent masks initialized with the Hadamard matrix and optimized under AGN and Poisson noise, respectively. While $\B{M}_G^I$ dynamically enhances light throughput by opening more pixels, $\B{M}_P^I$ remains fixed, representing an already ideal choice. Notably, $\B{M}_P^H$ tends to approach the identity matrix, in contrast to the behavior of $\B{M}_G^H$. The challenge arises from the non-convex nature of this optimization problem, making it difficult for $\B{M}_P^H$ to converge perfectly to the identity matrix. Nevertheless, this deviation underscores fundamental distinctions in optimizing masks under these distinct noise models.
        }
    }
    \label{fig:masks_value_dist}
\end{figure}


\Xhide{\bnote{talk about onn first in the last section and then show the reconstruction reuslts before the classifiction}}

\Xpolish{The different results of the optimal masks suggest the masks optimized under the AGN model may not have the same performance under the Poisson noise. If the measured data is Poisson distributed, then the methods proposed under the AGN assumption are problematic.}
{The results from optimizing the masks indicate that the optimal masks under the AGN model may not perform similarly under Poisson noise. Specifically, methods developed under the AGN assumption may not be effective when the measured data follows a Poisson distribution. \YLnote{For instance, coding optimization based on minimizing the mutual coherence in compressed sensing \cite{mordechay2014matrixRIP} may be defective.} The inherent differences in the underlying noise models of the two distributions can lead to suboptimal performance of AGN-optimized masks in Poisson noise scenarios. Therefore, it is crucial to consider Poisson noise when designing coding schemes and algorithms for imaging applications, especially when working with state-of-the-art sensors.}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/sensing_matrices_by_prior.tex <==
\subsection{Sensing Matrices by Priors}

\Xpolish{In the last section, we mentioned the masks $\B{M}$ can be generated by different coding strategies. 
In order to effectively determine the appropriate coding strategies for a given scenario, it is necessary to evaluate the various strategies based on their priors. Image priors, which can vary in type, can enhance the robustness of models in the presence of noise and improve overall image quality \cite{cossairt2012does, levin2007coded}. It should be noted that all of the strategies discussed in this paper possess three distinct prior levels. }
{In the preceding section, we discussed the generation of masks $\B{M}$ using different coding strategies. Evaluating the efficacy of these strategies for a given scenario requires a systematic assessment of their respective priors. Image priors come in varying types and can enhance model robustness in noisy environments and improve overall image quality \cite{cossairt2012does, levin2007coded}. It is important to note that all the strategies outlined in this paper possess three distinct prior levels.}
% \bnote{suggest bolding the priors}
\begin{itemize}
    \item \textbf{Null prior} (data is not compressible or needs to be reconstructed without priors). \Xpolish{Coding strategies in this category require no information about the data. They usually generate full rank matrices as $\B{M}$. In this project, we chose Raster Scan (RS) and Hadamard Basis (HB) for performance evaluation. $\B{M}$ for RS is an identity matrix while it is a Hadamard matrix for HB. On top of these two stratgies, we also include Impulse Imaging (II) which is the optimal measurement that can only be achieved with a sensor array. In our toy example this would be achieved by a camera sensor that captures the image so no coding is necessary. Mathematically, the sensing matrix $\B{M}$ of II is also an identity matrix, but each mask in II has $N$ times longer exposure time compared with RS.}
    {Coding strategies in this category require no information about the data. They usually generate full rank matrices as $\B{M}$. In this project, we chose Raster Scan (RS), Binary Random Basis (BR), and Hadamard Basis (HB) for performance evaluation. $\B{M}$ for RS is an identity matrix while it is a Hadamard matrix for HB. BR employs random values for each pixel in the mask, i.e  $\B{M} \in \{0,1\}^{N\times N}$. On top of these strategies, we also include Impulse Imaging (II) which works as a golden standard in this project. II is an ideal case assuming it can capture the whole data spectrum simultaneously. Mathematically, the sensing matrix $\B{M}$ of II is also an identity matrix, but each mask in II has $N$ times longer exposure time compared with RS.}
    \item \textbf{Reconstruction prior} (data is moderately compressible). \Xpolish{Coding strategies in this category are based on the fact that noise has greater influence on the high-frequency components in any images. We used Low-Frequency-Hadamard Basis which only keeps the low frequency vectors in a Hadamard matrix to study this prior. In this paper, it is labeled as Truncated Hadamard (TH).}
    {One common strategy in coding for images is to take advantage of the fact that noise tends to have a greater impact on high-frequency components. To investigate this phenomenon, we utilized a Low-Frequency-Hadamard Basis approach, in which only the low-frequency vectors of a Hadamard matrix are retained. This approach is referred to as Truncated Hadamard (TH) in this paper.}
    \item \textbf{Task-Specific prior or Selective Sensing prior} (data is extremely compressible). \Xpolish{Coding strategies requires much information from the data and tasks, and their corresponding sensing matrices $\B{M}$ vary from task to task. One strategy in this category is called Hardware PCA (Principal Components Analysis). It computes the most principal components in the training data, and constructs the masks with these components. Another interesting strategy is Selective Sensing (SS) whose sensing matrix $\B{M}$ is not pre-defined nor fixed, but is optimized within a Neural Networks model during the training. This optimization method is called Optical Neural Networks (ONN) in this project.}
    {Coding strategies are an essential component of signal processing that involve gathering task-specific information from data. In order to design these strategies, sensing matrices $\B{M}$ are developed, which can vary depending on the task at hand. One such approach is the Hardware Principal Components Analysis (PCA) technique, which identifies the most principal components in the training data and uses them to construct masks. Another strategy\Xhide{ is the Selective Sensing (SS), which} uses a sensing matrix $\B{M}$ that is not pre-defined or fixed, but rather is optimized using a Neural Networks model during training. In this project, this optimization method is referred to as Optical Neural Networks (ONN).}
\end{itemize}

\Xpolish{In this study, we examined the impact of various priors on a single-pixel imaging system in terms of\Xhide{ both \textbf{reconstruction}} and classification. Firstly, we explained our the methods for imeplementing the constraints in the single-pixel imaging model. Then, we simulated the effect of different prior types on classification performance using the MNIST dataset. Subsequently, we tested the feasibility of these strategies by experiments. \Xhide{Specifically, we first conducted a theoretical analysis to compare the reconstruction capabilities of the HB and RS in the presence of noise. Subsequently, we simulated the effect of different prior types on classification performance using the MNIST dataset. \bnote{is our theoretical analysis novel?} \rnote{I thought it was novel before read the hadamard book}}}
{In this study, we examine the impact of various priors on a single-pixel imaging system in terms of classification. Firstly, we explain our methods for implementing constraints in the single-pixel imaging model. Then, we simulate the effect of different prior types on classification performance using the MNIST dataset. Finally, we test the feasibility of these strategies through experiments.}



\Xhide{\bnote{The first and second sentences here are somewhat confusing due to the "Proposed model" language. We have not proposed a model yet, so unclear if it is our model or someone else's.} \rnote{This model is proposed by Rebecca, but I believe there is some error on the negative entries} In equation \ref{eqn:NoiselessMeasurement}, the parameter regarding the number of photons is an integral part of the mathematical representation of $\B{x}$. To further examine the mask basis under varied light levels, we propose a revised photon-counting model that decouples $\B{M}$ from the number of photons. In the following sections, we detail the development of this new model and provide insights into its practical implementation to avoid violating these constraints.} 

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/simulations.tex <==
\subsection{Computer Simulated Experiments}

\input{\homedir/sections/4_methods/simulations/simulated_data_generation.tex}

\input{\homedir/sections/4_methods/simulations/spectral_datasets.tex}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/simulations/simulated_data_generation.tex <==
\subsubsection{MNIST Simulated Data Preparation}

% \subsubsection{MNIST Data Pre-processing}

\Xpolish{The MNIST dataset consists of handwritten digits from 0 to 9, with a default size of 28 by 28 pixels \cite{lecun1998MNIST}. In order to align the data with the Hadamard matrices, we padded the images with black pixels at the edges to resize them to 32 by 32 pixels \cite{lecun1998MNIST}. We then transformed the range of all pixel values from $[0,1]$ to $[0.3, 1]$. This operation enhanced the persuasiveness of the dataset for various noise models, as the added black pixels do not generate Poisson noise, whose variance is proportional to the expected photon counts. \bnote{did we ever vary the dark level (0.3)/ have results showing its effect?}}
{The MNIST dataset, which comprises handwritten digits ranging from 0 to 9, has a default size of 28 by 28 pixels \cite{lecun1998MNIST}. To align the data with Hadamard matrices, we added black pixels to the edges of the images and resized them to 32 by 32 pixels \cite{lecun1998MNIST}. Subsequently, we rescaled the pixel values from the original range of $[0,1]$ to $[0.3, 1]$. This rescaling was aimed at improving the dataset's suitability for different noise models, as the initial black backgrounds do not introduce Poisson noise, which is typically proportional to the expected photon counts.}

==> hardware_pca_onn/sections_2023_Dec_OLD/4_methods/simulations/spectral_datasets.tex <==
\subsubsection{Spectral Datasets and Performance Evaluation}


% \rnote{How well this model can work w/o noise}

% \subsubsection{Performance Evaluation}


\Xpolish{The performances of the models were evaluated through their average classification rates. To ensure a thorough assessment, the model was tested five times independently, each time with a randomly split dataset for 70\% training and 30\% validation. During each assessment, the model generated noisy photon counts, which were then used to train the classifier until the validation rate reached a plateau or declined. The best validation rate achieved during the training process was chosen as the representative performance upper bound for each assessment. The overall performance of the model was determined by averaging the results of all five assessments.}
{The model performances were assessed based on their average classification rates, which were calculated after five independent tests. In each test, the dataset was randomly split into 70\% for training and 30\% for validation. The model generated noisy photon counts during each assessment, and the training continued until the validation rate reached a plateau or declined. The highest validation rate obtained during the training process was considered as the representative upper bound for each assessment. The overall model performance was determined by averaging the results from all five assessments. This comprehensive evaluation ensured the reliability and accuracy of the model performance.}



==> hardware_pca_onn/sections_2023_Dec_OLD/5_results.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{\homedir/sections/5_results_theory}


% \subsection{Mask optimization using PCA}
% \ynote{Describe
% Show image created wit PCA vs raster for noise levels
% }

% \YLnote{The images of PCA and raster doesn't depend on noise levels}








\subsection{Classification Rates on Simulated Experiment Data}

\Xpolish{In simulations, both the AGN and Poisson noise models were tested with the model we proposed. The results were generated under different noise levels by changing the exposure time. In addition, all compressible strategies were tested while changing the total number of masks. We defined a metric called compression ratio which is the ratio of the number of masks over the number of pixels. For the RS and HB, this ratio is constrained to be $1.00$. And for the rest, all values in $\mathcal{C}_R = \{0.01, 0.04, 0.09, 0.16, 0.25, 0.36, 0.49, 0.64, 0.81, 1.00\}$ were evaluated. Different from other strategies whose masks were pre-defined, the initial masks for ONN can affect the performances when noise exists. In this project, we initialized its masks by the PCA components from the training data as it usually has the best performances.}
{We evaluated our proposed model through simulations that tested both AGN and Poisson noise models, using varying exposure times to generate results at different noise levels. We also tested all {compressible} strategies, varying the total number of masks, and defined a metric called compression ratio as the ratio of the number of masks to the number of pixels \cite{stojek2022define_compression_ratio}. For RS and HB, this ratio was constrained to be 1.00, while the rest were evaluated over values in $\mathcal{C}_R = \{0.01, 0.04, 0.09, 0.16, 0.25, 0.36, 0.49, 0.64, 0.81, 1.00\}$. Unlike pre-defined masks used by other strategies, the initial masks for ONN can affect performance in the presence of noise. We therefore initialized its masks with the PCA components from the training data, which typically yield better performance.}

\Xpolish{The figure \ref{fig:simulated_classification} shows the classification performances with different parameters. The x-axis is the log-scaled mean square error (MSE) of impulse imaging (II) for some exposure time. The measured impulse imaging data requires no reconstruction and can be directly used to compute the noise level via $\|\noisy{\B{y}}_{II} - \B{x}\|_2^2$. As the golden standard in this project, this MSE can work as a metric showing the noise level for both AGN and Poisson noise models. The y-axis is the classification rate on the validation set. The compression ratio can affect the classification performances, so in this figure, we tried all the values in $\mathcal{C}_R$ and picked the best one for TH, PCA and ONN.}
{Figure \ref{fig:simulated_classification} displays the classification performance of different parameters. The x-axis is the log-scaled MSE of impulse imaging (II) with varying exposure times. \Xhide{Since the measured impulse imaging data requires no reconstruction, the noise level can be directly computed by $\|\noisy{\B{y}}_\mathrm{II} - \B{x}\|_2^2$. }This MSE is the gold standard in this project and serves as a metric to measure the noise level for both AGN and Poisson noise models. The y-axis represents the validation set's classification rate. We explored all the values in $\mathcal{C}_R$ to determine the best compression ratio for TH, PCA, and ONN since compression ratio affects classification performance. The figure shows the best results among all compression ratios for each strategy.}

\begin{figure}[ht]
    \begin{subfigure}{1\linewidth}
        \centering
        \caption{Classification under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_classification.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/gaussian_classification.pdf}
        \label{fig:gaussian_classification}
    \end{subfigure}
    \begin{subfigure}{1\linewidth}
        \centering
        \caption{Classification under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_classification.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Simulated/poisson_classification.pdf}
        \label{fig:poisson_classification}
    \end{subfigure}
    \caption{Classification rates on simulated data. RS: Raster basis. HB: Hadamard basis. II: Impulse imaging. BR: Binary random basis. TH: Truncated Hadamard basis. PCA: PCA basis. ONN: Optical Neural Networks. CG: control group. Selective strategies are marked by $\square$ and non-selective strategies are marked by $\blacktriangle$.(\subref{fig:gaussian_classification}) RS is the worst but using other non-selective coding strategies can improve the performance under the AGN. (\subref{fig:poisson_classification}) Among all non-selective strategies, only selective strategies can significantly improve the performance under Poisson noise. The CG employs the optimized masks under the AGN and trains the software classifier under Poisson noise. Its performance is worse than the ONN.}
    \label{fig:simulated_classification}
\end{figure}

\Xhide{\bnote{color compressible and non-compressible differently}}


\Xpolish{In this figure, we can see the II always has the best performance, which meets our expectation. When the noise is AGN, using any coding gives rise to a significant improvement compared with RS. For this classification task, using low-rank measurement (HB, PCA, ONN) can further improve this model's classification performances. Notably, the ONN has a performance close enough to the II with only 0.1\% number of photons.}
{The results presented in the figure demonstrate that II consistently achieves the highest performance, which is in line with our expectations. In the presence of AGN, all coding schemes exhibit significant improvements over RS and in many cases provide adequate performance. This is because under Gaussian noise, projected from a captured basis into a basis of sparsity where the classifier operates can be done without a significant noise penalty. Moreover, for the classification task at hand, low-rank measurement techniques such as HB, PCA, and ONN, can yield further improvements in classification performance. Notably, the ONN approach produces results that are nearly as good as the II approach, while using only 0.1\% of the photons.}

\Xpolish{However, when the measured data is Poisson distributed, HB is no better than RS any more, which agrees the conclusions of Harwit et al. \cite{harwit1979hadamard} that we should not adopt coding for Poisson noise. Though Hadamard coding is not promising, we can still have extra performance gain by using low-rank methods. Among all low-rank methods, the ONN is still the best, suggesting Selective Sensing is the most optimal method for both noise models.}
{However, when dealing with Poisson-distributed measured data, the effectiveness of Hadamard-based (HB) coding is no longer superior to that of RS. This aligns with the findings of Harwit et al. \cite{harwit1979hadamard}, which discourage the adoption of coding for Poisson noise. Despite this, there is still potential for performance improvement by utilizing low-rank methods such as TH, PCA and ONN. This is likely due to the fact that the images with analyze do in fact have sparsity in the Hadamard basis. Selective Sensing where capture patterns are optimized to capture sparsity directly like the ONN can retain their performance under poisson noise making them viable replacements for simple point scanners. This indicates that Selective Sensing is the most optimal approach for both noise models. }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Classification Performances on Hardware Experiment Data}

\Xpolish{In the experiments, we used a DMD and a PMT to measure 10 handwritten numbers from the MNIST dataset. The models were trained with $10^5$ photons, which is a greater noise level compared with the experimental environment. The collected data was in the form of a series of timestamps recording the arrival time of the photons. When collecting data, both RS and HB used 1024 masks. The TH and the HB shares the same measured data but the TH only uses the first 92 measured data. The PCA and ONN used 92 masks, which is the same as the TH. The physical measurements took 1 second per mask for all strategies. To create data of greater noise level from the raw data, we randomly picked intervals during the 1 second span, and counted the total numbers in it. Since the ONN and PCA only have 92 masks, the maximum exposure time was set as 92 seconds. In a fair comparison, the interval length of each strategy was cpmputed as $\frac{\tau}{m}$ where $\tau$ is the total exposure time we want to investigate and $m$ is number of masks for this strategy.}
{In our experiments, we utilized a DMD and a PMT to measure ten handwritten digits from the MNIST dataset. To train the models, we employed $10^5$ photons, which constituted a higher noise level in comparison to the experimental setup. The collected data took the form of a series of timestamps recording the photons' arrival time. During data collection, both RS and HB used 1024 masks, while the TH and HB employed the same measured data, but the TH used only the first 92 measurements. Similarly, PCA and ONN utilized 92 masks. Physical measurements took one second per mask for all strategies. To generate data with higher noise levels from the raw data, we randomly selected intervals within the 1-second span and counted the total number of photons within them. Since the ONN and PCA had only 92 masks, the maximum exposure time was set to 92 seconds. To ensure a fair comparison, we computed the interval length for each strategy as $\frac{\tau}{m}$, where $\tau$ represents the total exposure time under investigation, and $m$ denotes the number of masks used for each strategy.}

\Xhide{\bnote{consistent color on figures}}

\begin{figure}[ht]
    \centering
    % \includesvg[width=1\linewidth]{\homedir/figures/Results/Experimental_results.svg}
    \includegraphics[width=1\linewidth]{\homedir/figures/Results/Experimental_results.pdf}
    \caption{Classification rates on experiment data.  RS: Raster basis. HB: Hadamard basis. TH: Truncated Hadamard basis. PCA: PCA basis. ONN: Optical Neural Networks. ONN is in general the best strategies given the experimental data.}
    \label{fig:Exp_classification}
\end{figure}

\Xhide{\bnote{change the x tick labels}}

\Xpolish{However, we still saw some unexpected phenomena in the figure. Firstly, the HB strategy was better than the RS when the exposure was short, which was not observed in the simulation. This phenomenon might arise from the dark photon in the PMT. The dark photon is a signal-independent noise which has about 40-80 counts per second and could usually be observed before the experiments started. When the exposure was short, this noise would be more significant and gave rise to a better performance of the HB. Secondly, the TH achieved better classification performances than the PCA when the exposure time is short. It was the consequence of using unneeded PCA masks. To verify, we fixed the toal number of photons at $10^5$, change the compression ratio, and made figure \ref{fig:classification_ratio} by simulation. This figure shows that the PCA method can be worse than the TH when it has more masks than needed. In other words, the PCA strategy requires an careful estimation of the noise level to avoid using extra masks. Notably, the ONN looks more stable when includes extra masks. That can be seen as another advantage of the Selective Sensing. After the models are trained, they may be applied in unknown noise levels. Different from the PCA strategy whose optimal number of masks is noise level sensitive, the ONN can have a better and robust performance even when the number of masks is not optimal.}
 {Fig. \ref{fig:Exp_classification} displays the classification rates achieved on the experimental data. The x-axis shows the exposure time, and the y-axis represents the classification rates of the models. Although there may be discrepancies between software training and hardware data acquisition, the ONN models performed excellently. However, the figure reveals some unexpected phenomena. Firstly, the HB strategy outperformed the RS for short exposure times, which was not observed in the simulations. This phenomenon may have arisen due to the dark photon in the PMT, a signal-independent noise that has about 40-80 counts per second, and was more pronounced in short exposures. Secondly, the TH achieved better classification performances than the PCA when the exposure time was short. This result was due to the use of unneeded PCA masks. To verify, we conducted simulations and made Fig. \ref{fig:2d_classification_plots} by fixing the total number of photons at $10^5$ and varying the compression ratio under the Poisson noise. This figure showed that the PCA method could perform worse than the TH if extra masks were used. Hence, the PCA strategy requires careful estimation of the noise level to avoid using extra masks. Notably, the ONN appeared more stable when including extra masks, which is another advantage of the ONN. The ONN can perform robustly even with suboptimal numbers of masks, unlike the PCA strategy, which is noise-level sensitive. While it is possible to set the noise level during training, the effectiveness of the ONN can be evaluated for other levels of noise as well. This flexibility in application allows for broader use of the ONN beyond its specific training conditions, increasing its potential impact and utility in real-world scenarios.}




\Xhide{
\begin{figure}[ht]
    \centering
    \includesvg[width=1\linewidth]{\homedir/figures/Results/classification_vs_compression.svg}
    \caption{Classification rates VS compression ratio under Poisson noise. TH: Truncated Hadamard basis. PCA: PCA basis. ONN: Optical Neural Networks. Given a certain noise level, PCA is required to be accurate in the mask numbers or it can be worse than TH. ONN doesn't have such requirement.}
    \label{fig:classification_ratio}
\end{figure}
}


\Xhide{\YLnote{2D plot. \& Don't re-train the model. For training, choose a fixed noise (1e5) level, and for testing, use multiple noise levels}.}

\Xhide{
\begin{figure}[ht]
    \centering
    \includesvg[width=1\linewidth]{\homedir/figures/Results/classification_vs_light_level.svg}
    \caption{Classification rates VS light level under Poisson noise. TH: Truncated Hadamard basis. PCA: PCA basis. ONN: Optical Neural Networks. Given a certain noise level, PCA is required to be accurate in the mask numbers or it can be worse than TH. ONN doesn't have such requirement.}
    \label{fig:classification_light_level}
\end{figure}
}

\begin{figure*}[h]
    \begin{subfigure}{0.32\linewidth}
        \centering
        \caption{Truncated Hadamard classification rate}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/2d_contours/low_freq_truncated_hadamard_2d_classification.svg}
        \includegraphics[width=\linewidth]{\homedir/figures/Results/2d_contours/low_freq_truncated_hadamard_2d_classification.pdf}
        \label{fig:truncated_hadamard_2d_classification}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \caption{Hardware PCA classification rate}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/2d_contours/hardware_pca_2d_classification.svg}
        \includegraphics[width=\linewidth]{\homedir/figures/Results/2d_contours/hardware_pca_2d_classification.pdf}
        \label{fig:hardware_pca_2d_classification}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \caption{ONN classification rate}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/2d_contours/onn_2d_classification.svg}
        \includegraphics[width=\linewidth]{\homedir/figures/Results/2d_contours/onn_2d_classification.pdf}
        \label{fig:onn_2d_classification}
    \end{subfigure}
    \caption{Classification rates on simulated data w.r.t compression ratios and light levels.  The models were trained using a light level of $10^5$ and subsequently tested under different light levels. It was observed that hardware PCA performance deteriorates when the compression ratio is not properly chosen, whereas the Truncated Hadamard and ONN models exhibit greater robustness in such scenarios.}
    \label{fig:2d_classification_plots}
\end{figure*}

\Xhide{\YLnote{Show: fixed CR and change the noise level}}

\Xhide{\bnote{use $C_R$ on x axis}}

\Xhide{\YLnote{Add how to adjust the experimental data to be classified by simulated model}}



\input{\homedir/sections/5_results_hyperspectral}

==> hardware_pca_onn/sections_2023_Dec_OLD/5_results_hyperspectral.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulated Experiment on Hyper-Spectral Data}

\Xpolish{For this experiment, we use the Indian Pines dataset \cite{PURR1947}, which was acquired by employing Airborne Visible / Infrared Imaging Spectrometer (AVIRIS) on June 12, 1992 over the Purdue University Agronomy farm northwest of West Lafayette and the surrounding area.
This dataset is composed of $145 \times 145$ pixels and 224 spectral reflectance bands in the wavelength range 0.4 to 2.5  $\mu m$
In Fig. \ref{fig:pines_dataset}, the classes of the Indian Pines dataset are depicted, along with the respective counts within the dataset. The figure showcases an illustration of one channel (band 12) for all pixels, along with the ground truth of semantic labeling.}
{
In this experiment, we utilized the Indian Pines dataset \cite{PURR1947}, which was acquired through the Airborne Visible/Infrared Imaging Spectrometer (AVIRIS) on June 12, 1992, covering the Purdue University Agronomy farm northwest of West Lafayette and its surrounding area. Comprising $145 \times 145$ pixels and 224 spectral reflectance bands in the wavelength range of 0.4 to 2.5 $\mu m$, this dataset provides a comprehensive view of the study area. Fig. \ref{fig:pines_dataset} illustrates the classes within the Indian Pines dataset, presenting the counts associated with each class. The figure further features a representation of one channel (band 12) for all pixels, along with the ground truth of semantic labeling.
}

\Xpolish{In this experiment, we zero-padded each spectrum from 224 to 256 to align with the Hadamard mask. Spectral data are normalized within the range of $[0,1]$. The scanner-classifier module from Fig. \ref{fig:model_config} was utilized, with modifications made to the ONN classification layers to match the sizes of the new dataset. Each classification was performed for 2000 epochs, with a learning rate of $5 \times 10^{-3}$ and batch size of 5000.
Figure \ref{fig:pines_result} shows the classification rates for the Indian Pines dataset varying light level from $10^{1}$ to $10^{10}$.
% $10^-1$ to $10e^10$.
% To ensure accuracy, each classification was repeated 5 times, and the average was computed as the final result. 
}
{
In this experiment, spectral data were zero-padded from 224 to 256 to align with the Hadamard mask and \YLnote{\Xpolish{normalized}{re-scaled}} to the range $[0,1]$. We utilized the scanner-classifier module from Fig. \ref{fig:model_config}, adapting the ONN classification layers to the new dataset sizes. Each classification ran for 2000 epochs, with a learning rate of $5 \times 10^{-3}$ and a batch size of 5000. Figure \ref{fig:pines_result} illustrates the classification rates for the Indian Pines dataset across varying light levels from $10^1$ to $10^{10}$.
}


% by employing an 80-megapixel RGB camera and a hyperspectral CMOS sensor from a height of approximately 5,000 feet above the Rochester Institute of Technology’s university campus as shown in figure \ref{fig:aerorit_dataset}. The dataset includes a hyperspectral dataset with almost seven-million-pixel annotations. We utilized surface reflectance as our dataset, which was calculated from the calibrated radiance image. Each pixel in the dataset contains a spectrum of size 51, and it is labeled for different categories including cars, vegetation, buildings, water, and roads as shown in figure \ref{fig:AeroRIT_dataset_labels }. It is worth noting that the cars category is notably under-represented compared to the other classes. Based on the observations depicted in figure \ref{fig:AeroRIT_Histogram}, it is evident that spectral data corresponding to certain labels, such as water, exhibit minimal scattering, and demonstrate a uniform distribution pattern. Conversely, labels such as buildings, which possess varying colors, exhibit a greater degree of scattering in their spectra.



% \printinunitsof{in}\prntlen{\textwidth}



\begin{figure}[h]

    \centering
    \includegraphics[width=1\linewidth]{hardware_pca_onn/figures/Results/Hyperspectra/IndianPines_dataset.pdf}
    \caption{Indian Pines dataset \cite{PURR1947}}
    \label{fig:pines_dataset}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/IndianPines_histogram.pdf}
%     \caption{Spectrum for each class in the Indian Pines dataset \YLnote{is it better to use png images?}}
%     \label{fig:AeroRIT_Histogram}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=.8\linewidth]{\homedir/figures/Results/Hyperspectra/IndianPines_histogram.png}
    \caption{Spectrum for each class in the Indian Pines dataset}
    \label{fig:AeroRIT_Histogram}
\end{figure}


% \begin{figure*}
%     \centering
%     \includesvg[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/spectra.svg}
%     \caption{TODO}
%     \label{fig:AeroRIT_spectra}
% \end{figure*}

% \begin{figure}[h]
%     \centerline{\includegraphics[width=1\linewidth]{hardware_pca_onn/figures/Results/Hyperspectra/AeroRIT_results.pdf}}
%     \caption{AeroRIT results(TODO: ONN, TH and BR will be added, caption will be changed) {\YLnote{II for reconstruction? The font should be larger. Ask me for plot style codes.}}}
%     \label{fig:AeroRIT_restlts}
% \end{figure}


\begin{figure}[h]
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Classification under Gaussian noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/classification_vs_light_level_gaussian.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/classification_vs_light_level_gaussian.pdf}
        \label{fig:pines_gaussian_classification}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \caption{Classification under Poisson noise}
        % \includesvg[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/classification_vs_light_level_poisson.svg}
        \includegraphics[width=1\linewidth]{\homedir/figures/Results/Hyperspectra/classification_vs_light_level_poisson.pdf}
        \label{fig:pines_poisson_classification}
    \end{subfigure}
    \caption{Classification rates of Indian Pines dataset varying light level. RS: Raster basis. HB: Hadamard basis. II: Impulse imaging. BR: Binary random basis. TH: Truncated Hadamard basis. PCA: PCA basis. ONN: Optical Neural Networks. }
    \label{fig:pines_result}
\end{figure}

==> hardware_pca_onn/sections_2023_Dec_OLD/5_results_theory.tex <==
In this section, we start with a theoretical investigation on the reconstruction performances of null-prior strategies. Then the reconstruction and classification performances of all strategies and fairly compared by simulations and experiments. 

\subsection{Theoretical treatment for Null-Prior Reconstruction }

\YLnote{The dual branch section is removed and the ref link doesn't work}
% \textcolor{blue}{This section could be taken out.}
Define $\B{I}$ as the identity matrix and $\totphoton = \rho \tau$ as the total number of photons from the source. Given the noisy photon counts $\tilde{\B{y}}$ and the full-rank mask basis $\B{M}$, we can reconstruct the field of view $\tilde{\B{x}} = \B{M}^{-1} \tilde{\B{y}}$.
Based on Parseval's identity, the covariance matrix of a vector $\B{b}$ is $\B{\Sigma}_{\B{b}\B{b}} = c^2 \sigma^2 \B{I}$ if $\B{b} = \B{W a}$ where $\B{\Sigma}_{\B{a}\B{a}} = \sigma^2 \B{I}$ and 
% $\B{W}$ is $c$ times an orthonormal matrix
$\B{W} \B{W}^\top = c^2 \B{I}$
. For RS, we have $\lambda = \frac{\totphoton}{N^2}$ and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{I}\B{x}, \sigma^2 \B{I})$. Thus, the reconstructed field of view is 
\begin{equation}
    \label{eqn:RS_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{\sigma^2 N^4}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
For HB, we have $\lambda = \frac{\totphoton}{2N^2}$  and $\lambda \tilde{\B{y}} \sim \mathcal{N}(\lambda \B{H}\B{x}, 2\sigma^2 \B{I})$ due to the dual branch trick mentioned in section \Xpolish{\ref{sssection:DualBranch}}{\ref{ssection:constraints}}. For $\B{H}^{-1}$, $c = \sqrt{\frac{1}{N}}$. The reconstructed field of view is 
\begin{equation}
    \label{eqn:HB_G_reconstruction}
    \begin{aligned}
        \tilde{\B{x}} &\sim \mathcal{N}\left(\B{x}, \frac{8 \sigma^2 N^3}{{\totphoton}^2} \B{I}\right)
    \end{aligned}.
\end{equation}
% Therefore, when considering the AWGN model, using the Hadamard matrix can improve the SNR of the reconstructed field of view when $N$ is large.
Therefore, using the Hadamard matrix in the AWGN model can improve the signal-to-noise ratio (SNR) of the reconstructed field of view when the number of elements, $N$, is large. 

When the noise is Poisson distributed, the covariance matrix of the noisy photon counts depends on the choice of $\B{M}$. Suppose $\sigma_j$ is the standard deviation of $\lambda \tilde{y}_j$, the $j_\text{th}$ measured noisy photon counts. For the RS, we have $\sigma_j^2 = \lambda x_j$ and $\lambda = \frac{\totphoton}{N^2}$. The covariance matrix of the reconstructed field of view is thus 
\begin{equation}
    \label{eqn:RS_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{N^2}{\totphoton}\diag\{x_1, x_2, \cdots, x_N\}
    \end{aligned}.
\end{equation}
% For HB, we have $\lambda = \frac{\totphoton}{2N^2}$ and $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$ by the Skellam Distribution in section \ref{sssection:DualBranch}. Since Hadamard matrices only includes $\pm 1$ entries, we further have $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$ and the covariance matrix  

In the case of the HB, we can express the rate parameter $\lambda$ as $\lambda = \frac{\totphoton}{2N^2}$, as demonstrated in section \ref{ssection:constraints} using the Skellam Distribution. Additionally, we can express the variance of each element in the sum as $\sigma_j^2 = \lambda \sum_{k=1}^N |H_{jk}| x_k$. As Hadamard matrices only contain entries of $\pm 1$, this reduces to $\sigma_j^2 = \lambda \sum_{k=1}^N x_k$. Using this information, we can construct the covariance matrix
\begin{equation}
    \label{eqn:HB_P_reconstruction}
    \begin{aligned}
        \B{\Sigma}_{\tilde{\B{x}} \tilde{\B{x}}} &= \frac{2N \sum_{k=1}^N x_k}{\totphoton}  \B{I}
    \end{aligned}.
\end{equation}
% Therefore, the mean squared error (MSE) of HB is 2 times that of RS under Poisson noise. This factor of 2 arises from the dual branch trick. In other words, HB can never exceed RS in reconstruction error even when measuring with 2 PMTs simultaneously.
The results of our analysis reveal that the mean squared error (MSE) of the HB method is twice that of the RS method when the noise is Poisson distributed. This difference is attributed to the dual branch trick utilized in the HB method. Despite the use of two PMTs in the HB method, it is unable to surpass the reconstruction error of the RS method. These findings demonstrate the limitations of the HB method in comparison to the RS method under Poisson noise conditions.




==> hardware_pca_onn/sections_2023_Dec_OLD/6_discussion.tex <==
\subsection*{\checkednote{Definition of a measurement}}

\iffalse
In \Xpolish{compressed sensing and }{computational imaging}, coding is typically defined as a measurement of an analog flux through some type of coding projection or in our example a mask. As has been shown by multiple works, this analog model of light does not account for the poisson noise inherent in any real measurements and leads to counter intuitive behavior of coding approaches.

If we instead think of our system as measuring photons through different codes, the code behavior makes intuitive sense. A photon measured through a mask with many open pixels carries less information about the scene than one captured through a raster mask because our measurement is ambiguous regarding which pixel in the mask was the origin of the photon. In a raster mask every photon can be uniquely assigned to one pixel. In essence, more photons do not equal more information.

The implication of this well documented problem become ever more important in the age of low noise and photon counting cameras where Poisson noise dominates all measurements. It is wide reaching since the projection process we study here in a specific coding experiment is part of the design of any camera. In other words: Any camera or vision system has to project data from a high dimensional scene space down into a lower dimensional sensor space where it encounters Poisson noise and then uses those noisy measurements to make inferences about the scene. 
\fi 
% replaced by the below
In computational imaging, coding typically involves measuring analog flux through a coding projection such as mask in our case. However, this analog model neglects inherent Poisson noise in real measurements, leading to counterintuitive coding behaviors. Viewing the system as measuring photons through different codes provides more intuitive insights. For instance, a photon measured through a mask with open pixels carries less scene information than one through a raster mask, where each photon can be uniquely assigned to a pixel. This challenge becomes critical in the era of low-noise, photon-counting cameras dominated by Poisson noise. This issue is significant as the projection process studied in specific coding experiments is integral to the design of any camera, where high-dimensional scene data is projected into a lower-dimensional sensor space encountering Poisson noise for subsequent scene inferences.


\Xpolish{This paper has shown that the challenges for computational imaging under Poisson noise. Algorithms based on the AGN noise assumption are problematic on the modern sensors. However, if the task requires no reconstruction but direct feature extraction, the Selective Sensing using the Optical Neural Networks model can find the optimal coding methods. We have shown the feasibility of the Selective Sensing via simulations and experiments, and it demonstrated a promising classification performance on the MNIST handwritten number dataset. Also, it is robust in the application scenarios where their noise level is hard to estimate. Furthermore, the Selective Sensing provides an motivation for proposed optical ANNs or ANNs with optical layers which allow us to optimize the coding schemes wherever the Poisson noise happens. }
{Our paper highlights the challenges of computational imaging under Poisson noise and its impact on algorithms based on the AGN noise assumption. We find that for compressible measurements, and especially tasks that involve direct feature extraction instead of signal reconstruction, a Selective Sensing approach using task-based optimized codes provides a viable coding solution. Through simulations and experiments, we demonstrate the feasibility of Selective Sensing and its promising classification performance on the MNIST handwritten number dataset. It is also robust in application scenarios with difficult-to-estimate noise levels. Our ONN method represents a method that can generate these selective measurements. Furthermore, Selective Sensing motivates the development of optical ANNs or ANNs with optical layers to globally optimize imaging systems.}

\Xpolish{On the other hand, there are some limitations in our project. First, we employed the AGN model and reparameterization trick for the model training, which is only an approximation to the noise at the sensor. Second, our test set in the experiments only contains 10 numbers, which may not be representative enough. There is also an inconsistency as the model was trained by simulated data but tested with experimental data. Last but not the least, the Photon Distribution Factor rescales the masks $\B{M}$, but its value changes during the training and it is not evolved in the back-propagation. In general, the optimization of the ONN model still has some defects and we still need to improve the results by using better optimization methods and more experimental data.}
{Despite the promising results of our project, there are some limitations that must be acknowledged. First, we used a Gaussian noise model with reparameterization to train our model, which is only an approximation of the actual quantization noise at the sensor. Second, our test set consisted of only 10 numbers, which may not provide a comprehensive evaluation of the model's performance. Additionally, we noted an inconsistency in that the model was trained using simulated data but tested with experimental data. \Xpolish{Lastly, the \YLnote{Photon Distribution Factor \#no referrence before\#} rescales the masks $\B{M}$}{Lastly, we employ a weighted re-distribution method to satisfy the constraint \ref{constraint:photonNumber} for sensing matrices}, but its value changes during training and is not evolved during back-propagation. These limitations highlight the need for further improvements in the optimization of the ONN model, such as using more advanced optimization methods and larger sets of experimental data. Our work highlights the importance of the integration of imaging hardware and signal processing. In single photon accurate imaging systems, comprehensibility and sparsity of the data can be exploited to far greater effect during the measurement, as opposed to post processing.}



==> hardware_pca_onn/sections_2023_Dec_OLD/title.tex <==
Selective Sensing
